The Data Minimization Principle in Machine Learning

The principle of data minimization aims to reduce the amount of data collected, processed or retained to minimize the potential for misuse, unauthorized access, or data breaches. Rooted in privacy-by-design principles, data minimization has been endorsed by various global data protection regulations. However, its practical implementation remains a challenge due to the lack of a rigorous formulation. This paper addresses this gap and introduces an optimization framework for data minimization based on its legal definitions. It then adapts several optimization algorithms to perform data minimization and conducts a comprehensive evaluation in terms of their compliance with minimization objectives as well as their impact on user privacy. Our analysis underscores the mismatch between the privacy expectations of data minimization and the actual privacy benefits, emphasizing the need for approaches that account for multiple facets of real-world privacy risks.

==> archived_sections/archived_figure_scripts/fig_framework.tex <==
\begin{tikzpicture}[scale=1.]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Formalizing Data Minimization
\node (data) at (0,0) {\includegraphics[height=30px]{images/data.png}};
\node[above = -0.1cm of data] (datatitle) {Dataset\strut};

\node (minimizeddata) at (6.7,0) {\includegraphics[height=30px]{images/data_released.png}};
\node[text width=1.8cm,align=center,above = -0.1cm of minimizeddata] (minimizeddatatitle) {Minimized Dataset\strut};

\draw[-stealth,ultra thick] (data.east) -- node[above] {\textbf{Minimization\strut} \quad \raisebox{-.4\height}{\includegraphics[height=25px]{images/minimized_matrix.png}} \quad \quad \quad}(minimizeddata.west);

\draw[rounded corners](-0.8,-0.8)--(5.2,-0.8)--(5.2, 2.4)--(-0.8,2.4)--cycle;

\node[align=left, anchor=west] (formalization) at (-0.5,1.9) {\color{blue}\textbf{Formalizing Data Minimization\strut}}; 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Data Breach
\node (elbow) at (6.7,-2) {};
\node (elbowreid) at (1,-2.4) {};
\node (elbowrecon) at (5.5,-2.4) {};

\node[align=center,anchor=east] (formalization) at (6.6,-1.5) {\color{red}\textbf{Data Breach}}; 

%% Re-identification Risk
\node (reid) at (0,-3.1) {\includegraphics[height=20px]{images/reid.png}};
\node (reid_partial1) at (2,-2.6) {\includegraphics[height=20px]{images/reid_partial.png}};
\node (reid_partial2) at (2,-3.6) {\includegraphics[height=20px]{images/reid_partial.png}};
\draw[<->, ultra thick] (reid.east) -- (reid_partial2.west);

\draw[-stealth,ultra thick] (minimizeddata.south) -- (elbow.center) -| (elbowreid.center);

\node[align=center, text width=3cm] at (1, -4.4) (reidtitle) {Re-identifying Individuals};

%% Reconstruction Risk
\node (reconmin) at (4.3,-3.1) {\includegraphics[height=30px]{images/data_released.png}};
\node (reconorig) at (6.3,-3.1) {\includegraphics[height=30px]{images/data.png}};
\draw[-stealth, ultra thick] (reconmin.east) -- (reconorig.west);

\draw[-stealth,ultra thick] (minimizeddata.south) -- (elbow.center) -| (elbowrecon.center);
\node[align=center, text width=3cm] at (5.3, -4.4) (recontitle) {Reconstructing Missing Data};

\draw[rounded corners](-0.8,-1.1)--(7.3,-1.1)--(7.3, -5.1)--(-0.8,-5.1)--cycle;

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% DP Wall

\node[anchor=north] (reid_partial1) at (8.2,2.4) {\includegraphics[height=205px,width=10px]{images/wall.png}};

\node[align=left, anchor=west] at (8.5, -3.1) (reidtitle) {No Data Access \\Beyond This Wall};

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Measuring Utility
\node (trainingmodel) at (10.2,0) {\includegraphics[height=30px]{images/processing.png}};
\node[text width=1.5cm,align=center,above = -0.1cm of trainingmodel] (trainingmodeltitle) {Model Training\strut};

\draw[-stealth,ultra thick] (minimizeddata.east) -- (trainingmodel.west);

\node (trainedmodel) at (12.7,0) {\includegraphics[height=30px]{images/model.png}};
\node[text width=1.5cm,align=center,above = -0.1cm of trainedmodel] (trainedmodeltitle) {Trained Model\strut};

\draw[-stealth,ultra thick] (trainingmodel.east) -- (trainedmodel.west);

\node (testdata) at (15.2,0) {\includegraphics[height=30px]{images/data_test.png}};
\node[text width=1.5cm,align=center,above = 0.cm of testdata] (testdatatitle) {Test Dataset};

\draw[<->, ultra thick] (trainedmodel.east) -- (testdata.west);

\node[anchor=west,align=left] (utility) at (9.4,1.9) {\color{olive}\textbf{Measuring Utility}}; 

\draw[rounded corners](9.1,-0.8)--(16,-0.8)--(16, 2.4)--(9.1,2.4)--cycle;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Model Release/Breach

\node (elbowmia) at (12.7,-2) {};
\node (elbowmiacenter) at (14,-2.4) {};

\node[align=center,anchor=west] (modelbreach) at (12.8,-1.5) {\color{red}\textbf{Model Breach}}; 

\node (miapos) at (12.7,-2.6) {\includegraphics[height=25px]{images/mia_pos.png}};
\node (mianeg) at (12.7,-3.6) {\includegraphics[height=25px]{images/mia_neg.png}};
\node (datamia) at (15.2,-3.1) {\includegraphics[height=30px]{images/data.png}};
\draw[<->, ultra thick] (miapos.east) -- (datamia.170);
\draw[<->, ultra thick] (mianeg.east) -- (datamia.190);

\draw[-stealth,ultra thick] (trainedmodel.south) -- (elbowmia.center) -| (elbowmiacenter.center);

\node[align=center, text width=3cm] at (14, -4.4) (miatitle) {Infering Membership};

\draw[rounded corners](11.6,-1.1)--(16,-1.1)--(16, -5.1)--(11.6,-5.1)--cycle;
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\end{tikzpicture}

==> archived_sections/archived_figure_scripts/fig_nn_dataset_size_minimization.tex <==
\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ylabel={Accuracy},ymin=76,ymax=93,xticklabel= {\pgfmathprintnumber\tick\%},xmin=0,xmax=100,xlabel={Dataset Size},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,50,100},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(a) Bank Dataset}}]

\addplot [blue,no marks,thick] table[x=Size,y=Acc] {data/bank_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Size,y=Acc] {data/bank_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Size,y=Acc] {data/bank_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Size,y=Acc] {data/bank_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Size,y=Acc] {data/bank_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,91.54) -- (axis cs:100,91.54);
\node[anchor=south west] at (axis cs: 0,91.54) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,89.54) -- (axis cs:100,89.54);
\node[anchor=south west] at (axis cs: 0,89.54) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ymin=72,ymax=83,xticklabel= {\pgfmathprintnumber\tick\%},xmin=0,xmax=100,xlabel={Dataset Size},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,50,100},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(b) Wine Dataset}}]

\addplot [blue,no marks,thick] table[x=Size,y=Acc] {data/wine_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Size,y=Acc] {data/wine_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Size,y=Acc] {data/wine_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Size,y=Acc] {data/wine_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Size,y=Acc] {data/wine_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,81.48) -- (axis cs:100,81.48);
\node[anchor=south west] at (axis cs: 0,81.48) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,79.48) -- (axis cs:100,79.48);
\node[anchor=south west] at (axis cs: 0,79.48) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ylabel={Accuracy},ymin=60,ymax=81,xticklabel= {\pgfmathprintnumber\tick\%},xmin=0,xmax=100,xlabel={Dataset Size},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,50,100},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(c) Employment Dataset}}]

\addplot [blue,no marks,thick] table[x=Size,y=Acc] {data/employment_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Size,y=Acc] {data/employment_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Size,y=Acc] {data/employment_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Size,y=Acc] {data/employment_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Size,y=Acc] {data/employment_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,78.76) -- (axis cs:100,78.76);
\node[anchor=south west] at (axis cs: 0,78.76) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,76.76) -- (axis cs:100,76.76);
\node[anchor=south west] at (axis cs: 0,76.76) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[scale=0.01,
hide axis,
xmin=0, xmax=1,
ymin=0, ymax=1,
legend columns=4,
legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.1cm}}
]
\addlegendimage{ultra thick, blue}
\addlegendentry{Feature Selection};
\addlegendimage{ultra thick, red}
\addlegendentry{Random Subsampling};
\addlegendimage{ultra thick, green}
\addlegendentry{Personalized Random Subsampling};
\addlegendimage{ultra thick, brown}
\addlegendentry{Metamodeling};
\addlegendimage{ultra thick, magenta}
\addlegendentry{Metamodeling (LR)};

\end{axis}
\end{tikzpicture}

==> archived_sections/archived_figure_scripts/fig_nn_reconstruction_minimization.tex <==
\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ylabel={Accuracy},ymin=76,ymax=93,,xmin=0,xmax=1,xlabel={Reconstruction Risk},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,0.5,1},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(a) Bank Dataset}}]

\addplot [blue,no marks,thick] table[x=Recon,y=Acc] {data/bank_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Recon,y=Acc] {data/bank_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Recon,y=Acc] {data/bank_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Recon,y=Acc] {data/bank_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Recon,y=Acc] {data/bank_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,91.54) -- (axis cs:100,91.54);
\node[anchor=south west] at (axis cs: 0,91.54) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,89.54) -- (axis cs:100,89.54);
\node[anchor=south west] at (axis cs: 0,89.54) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ymin=72,ymax=83,,xmin=0,xmax=1,xlabel={Reconstruction Risk},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,0.5,1},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(b) Wine Dataset}}]

\addplot [blue,no marks,thick] table[x=Recon,y=Acc] {data/wine_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Recon,y=Acc] {data/wine_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Recon,y=Acc] {data/wine_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Recon,y=Acc] {data/wine_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Recon,y=Acc] {data/wine_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,81.48) -- (axis cs:100,81.48);
\node[anchor=south west] at (axis cs: 0,81.48) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,79.48) -- (axis cs:100,79.48);
\node[anchor=south west] at (axis cs: 0,79.48) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ylabel={Accuracy},ymin=60,ymax=81,,xmin=0,xmax=1,xlabel={Reconstruction Risk},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,0.5,1},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(c) Employment Dataset}}]

\addplot [blue,no marks,thick] table[x=Recon,y=Acc] {data/employment_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Recon,y=Acc] {data/employment_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Recon,y=Acc] {data/employment_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Recon,y=Acc] {data/employment_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Recon,y=Acc] {data/employment_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,78.76) -- (axis cs:100,78.76);
\node[anchor=south west] at (axis cs: 0,78.76) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,76.76) -- (axis cs:100,76.76);
\node[anchor=south west] at (axis cs: 0,76.76) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[scale=0.01,
hide axis,
xmin=0, xmax=1,
ymin=0, ymax=1,
legend columns=4,
legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.1cm}}
]
\addlegendimage{ultra thick, blue}
\addlegendentry{Feature Selection};
\addlegendimage{ultra thick, red}
\addlegendentry{Random Subsampling};
\addlegendimage{ultra thick, green}
\addlegendentry{Personalized Random Subsampling};
\addlegendimage{ultra thick, brown}
\addlegendentry{Metamodeling};
\addlegendimage{ultra thick, magenta}
\addlegendentry{Metamodeling (LR)};

\end{axis}
\end{tikzpicture}

==> archived_sections/archived_figure_scripts/fig_nn_reidentification_minimization.tex <==
\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ylabel={Accuracy},ymin=76,ymax=93,,xmin=0,xmax=1,xlabel={Reidentification Risk},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,0.5,1},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(a) Bank Dataset}}]

\addplot [blue,no marks,thick] table[x=Reid,y=Acc] {data/bank_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Reid,y=Acc] {data/bank_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Reid,y=Acc] {data/bank_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Reid,y=Acc] {data/bank_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Reid,y=Acc] {data/bank_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,91.54) -- (axis cs:100,91.54);
\node[anchor=south west] at (axis cs: 0,91.54) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,89.54) -- (axis cs:100,89.54);
\node[anchor=south west] at (axis cs: 0,89.54) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}%
\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ymin=72,ymax=83,,xmin=0,xmax=1,xlabel={Reidentification Risk},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,0.5,1},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(b) Wine Dataset}}]

\addplot [blue,no marks,thick] table[x=Reid,y=Acc] {data/wine_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Reid,y=Acc] {data/wine_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Reid,y=Acc] {data/wine_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Reid,y=Acc] {data/wine_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Reid,y=Acc] {data/wine_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,81.48) -- (axis cs:100,81.48);
\node[anchor=south west] at (axis cs: 0,81.48) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,79.48) -- (axis cs:100,79.48);
\node[anchor=south west] at (axis cs: 0,79.48) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis} [width=0.5\linewidth,height=0.4\linewidth,yticklabel= {\pgfmathprintnumber\tick\%},ylabel={Accuracy},ymin=60,ymax=81,,xmin=0,xmax=1,xlabel={Reidentification Risk},axis y line*=left,axis x line*=bottom,ylabel near ticks,ylabel style={align=center, text width=4cm},xtick={0,0.5,1},legend pos=south east, legend style={font=\tiny}, legend cell align={left}, title={\textbf{(c) Employment Dataset}}]

\addplot [blue,no marks,thick] table[x=Reid,y=Acc] {data/employment_nn/feature_selection.dat};
\addplot [red,no marks,thick] table[x=Reid,y=Acc] {data/employment_nn/random_subsampling.dat};
\addplot [green,no marks,thick] table[x=Reid,y=Acc] {data/employment_nn/personalized_random_subsampling.dat};
\addplot [brown,no marks,thick] table[x=Reid,y=Acc] {data/employment_nn/metamodeling_heuristic.dat};
\addplot [magenta,no marks,thick] table[x=Reid,y=Acc] {data/employment_nn/metamodeling_lr_heuristic.dat};

\draw[black, dashed] (axis cs:0,78.76) -- (axis cs:100,78.76);
\node[anchor=south west] at (axis cs: 0,78.76) {\tiny$\alpha=0\%$};
\draw[black, dashed] (axis cs:0,76.76) -- (axis cs:100,76.76);
\node[anchor=south west] at (axis cs: 0,76.76) {\tiny$\alpha=2\%$};

\end{axis}
\end{tikzpicture}

\begin{tikzpicture}
\begin{axis}[scale=0.01,
hide axis,
xmin=0, xmax=1,
ymin=0, ymax=1,
legend columns=4,
legend style={font=\scriptsize,/tikz/every even column/.append style={column sep=0.1cm}}
]
\addlegendimage{ultra thick, blue}
\addlegendentry{Feature Selection};
\addlegendimage{ultra thick, red}
\addlegendentry{Random Subsampling};
\addlegendimage{ultra thick, green}
\addlegendentry{Personalized Random Subsampling};
\addlegendimage{ultra thick, brown}
\addlegendentry{Metamodeling};
\addlegendimage{ultra thick, magenta}
\addlegendentry{Metamodeling (LR)};

\end{axis}
\end{tikzpicture}

==> archived_sections/archived_sec_data_minimization_principle.tex <==
We will begin by establishing our framework for data minimization. We have utilized legal language from six data protection regulations worldwide to define data minimization and its objectives. Our initial focus is on faithfully transforming the legal requirements into an optimization problem, which we find only considers dataset size and utility. Subsequently, we also discuss the privacy implications of data minimization within the context of these regulations and introduce several threat models to complete our framework. See Figure \ref{fig:framework} for an overall representation of our framework.

\subsection{From Policy to Operations}

We will start by formalizing a framework for data minimization in machine learning and define an optimization problem associated with the objectives of data minimization.

\input{tables/tab_legal}

\paragraph{Purpose Limitation:} Data protection regulations require that data shall only be collected for a \textit{specific, explicitly defined and lawful purpose} (POPIA, South Africa) and that the data collector shall not \textit{use (sensitive) personal information collected for additional purposes that are incompatible with the disclosed purpose for which the (sensitive) personal information was collected} (CPRA, USA). See Table \ref{tab:legal} for purpose limitation in other regulations (highlighted in {\color{magenta}magenta}). Clearly, before diving into data minimization, it is crucial to first define the purpose of data collection.

In machine learning, data collection is essential for training a learning model. More precisely, the purpose of collecting data can be quantified as the success of the learned model, i.e., through a utility function, commonly a loss function.
Consider a dataset $\cD = (\cX, \cY) = \{x_i, y_i\}^n_{i=1}$ consisting of $n$ data points, where each data point is a tuple comprising of input features $x_i \in \cR^{d}$ and the associated output label $y_i$. In a typical ML setup, the learning objective can be defined as:
\begin{align}
    \theta^* = \arg\max_{\theta} \textrm{ } U(\cX ,\cY, \theta)
\end{align}
Here $U(.)$ represents the utility function for the task at hand. For instance, when performing empirical risk minimization (ERM) for learning, the utility function can be defined as: 
\begin{align}
    U(\cX, \cY, \theta) = - \cL_{ERM}(\cX, \cY, \theta)\\
    \textrm{where} \quad \quad \cL_{ERM}(\cX, \cY, \theta) = \sum^n_{i=1} \ell \big( f_{\boldsymbol{\theta}}(x_i) ,y_i \big) +\lambda \| \bm{\theta}\|^2
\end{align}
Here $f_\theta(.)$ represents the inference function of a learned model with parameters $\theta$, $\ell(.)$ is an appropriate loss function depending on the learning task (e.g., MSE loss or cross entropy) and $\lambda$ is the regularization parameter.

\paragraph{Personalized Decisions:} Now that we have defined an explicit purpose for our data collection, we can focus on formalizing data minimization. Data minimization is simply a set of binary decisions regarding the collection and/or retention of each individual information in the dataset. These decisions are inherently personalized. For example, consider the ACSEmployment dataset, which contains information about individuals, including their age, income, race, military history, medical history, etc., with the objective of inferring their employment status. Clearly, some individuals' employment status can be inferred from their age and/or income alone, rendering the release of their military or medical history unnecessary, while for others these additional attributes may be crucial to understanding their employment status.

Formally, these decisions during data minimization can be captured using a binary matrix $\cB \in \{\phi,1\}^{n \times d}$, which we call the \emph{minimization matrix}. Here, the symbol $\phi$ represents the concealment or removal of redundant values in the dataset, i.e., $\forall a \in \R: a \times \phi = \phi$. The minimized input feature set $\cX'$ can then be defined as the element-wise product of the original feature set $\cX$ and the minimization matrix $\cB$, i.e., $\cX' = \cX \odot \cB$. Note that we are left with empty values $\phi$ in the minimized feature set $\cX'$. While some learning algorithms are capable of handling missing values in the dataset, in most cases one would also need to impute the minimized dataset using average statistics or more advanced techniques.

\paragraph{Data Minimization is Data-Dependent:} 
To accurately assess the relevance of data for a particular purpose, it is important to inspect the complete data, i.e. data minimization is inherently data-dependent. Making a decision on collecting and/or retaining parts of the data without considering its actual value can lead to valuable information being excluded or irrelevant data being included, thus compromising the utility of the minimized dataset. Moreover, making such preemptive choices can introduce biases in our dataset, since the expected value of data cannot capture the diversity of representation. Thus, throughout our discussion of data minimization, we will focus on the setting where the data handler has initial access to the complete data, and then makes decisions on retaining or deleting parts of the data, according to the objectives of data minimization discussed next.

% Most laws and regulations on data handling require that the data collector does not \textit{collect more data than is reasonably needed} (The Privacy Act) and the said data \textit{not be retained any longer than is necessary for achieving the purpose for which the information was collected} (POPIA). See Table \ref{tab:legal} for language on data collection and retention in other regulations (highlighted in {\color{green}green}). Formally, data minimization is simply a set of binary decisions regarding the collection and/or retention of each individual value in the dataset.

\paragraph{Limited and Necessary to the Purpose:} We have defined the purpose of data collection in ML and formalized a mathematical formulation of data minimization. Finally, we connect the two by focusing on the objective of data collection with respect to the defined purpose. Existing regulations require that collected data \textit{shall be adequate, relevant and limited to what is necessary in relation to the purposes for which they are processed} (GDPR, Europe), or similarly be \textit{relevant, proportional and non-excessive in relation to purposes of the data processing} (LGPD, Brazil). See Table \ref{tab:legal} for language on objectives of data collection in other regulations (highlighted in {\color{blue}blue}). In direct terms, data minimization aims to remove any redundant values in the dataset that do not contribute to the utility of the learned model.

We can define the objective of data minimization as finding an optimal minimization matrix $\cB^*$ that can minimize the dataset size while retaining its utility, i.e.: 
\begin{align}
    \cB^* = \arg\min_{\cB} ||\cB||_0 \quad \textrm{where} \quad \cB \in \cF_{\cB}
\end{align}
Here $||\cB||_0$ is the $l_0$ norm of the minimization matrix, defined as simply the number of indices where $\cB_{ij}=1$, and $\cF_{\cB}$ is a feasibility set of minimization matrices defined as:
\begin{align}
\label{eq:misalignment}
\cF_{\cB}=
\left\{
  \cB
\;\middle|\;
\begin{alignedat}{2}
  & \cA(\cX \odot \cB, \cX) \leq \alpha \\
  & \cB \in \{\phi,1\}^{n \times d}
\end{alignedat}
\right\}
\end{align}
Here $\cA(\cX_1, \cX_2)$ represents the misalignment in utility between two learning models trained on the datasets $(\cX_1, \cY)$ and $(\cX_2, \cY)$ respectively, and $\alpha$ is the maximum amount of misalignment permitted during minimization, which represents the threshold for maintaining utility. For instance, we can define misalignment as simply the difference in loss values between the two learned models, i.e.:
\begin{align}
    \cA(\cX \odot \cB, \cX) = \cL(\cX, \cY, \theta^*_{\cX \odot \cB}) - \cL(\cX, \cY, \theta^*_{\cX}) \\
    \textrm{where} \quad \theta^*_{\cX} = \arg\min_{\theta} \cL(\cX, \cY, \theta)
\end{align}
Here $\cL(.)$ represents the loss function used to measure the utility of the trained model. The misalignment is defined such that even though our model is trained on the minimized dataset with missing values, it should perform well on the full dataset, i.e., the inference behaviour remains unchanged.

We can thus formalize the overall data minimization objective as a bilevel optimization:
\begin{align}
    \arg\min_{\cB} ||\cB||_0 + \lambda*(\cL(\cX, \cY, \theta^*_{\cX \odot \cB}) - L_{c} - \alpha + t^2) \\
    \textrm{where} \quad \theta^*_{\cX \odot \cB} = \arg\min_{\theta} \cL(\cX \odot \cB, \cY, \theta)
\end{align}
Here $\lambda, t^2$ represent the lagrangian multiplier and the slack variable respectively, for the misalignment constraints in Eq. \ref{eq:misalignment}. $L_{c}$ is a constant value independent of the minimization matrix $\cB$, defined as $L_{c} = \cL(\cX, \cY, \theta^*_{\cX})$. Note that $\cB$ can only take certain discrete values, i.e., $\cB \in \{\phi,1\}^{n \times d}$.

\subsection{Privacy Leakage}

In current data protection regulations, personal data is defined as any information that directly \textit{identifies a particular individual}, or can be indirectly \textit{combined with other information to identify a particular individual} (PIPA, South Korea). See Table \ref{tab:legal} for other similar definitions of personal data across various regulations (highlighted in {\color{orange}orange}). It is clear that these regulations prioritize data minimization to avoid collecting unnecessary information that could compromise an individual's privacy. However, data minimization doesn't necessarily equate to the best practices for privacy protection under some utility constraints. For instance, additional data can in some cases provide anonymization to individuals, which would not align with the objectives of data minimization. 

Our work aims to clarify the relationship between data minimization and privacy to understand both the benefits and the limitations of data minimization in safeguarding individuals' privacy in a dataset. In order to measure the privacy benefits of data minimization, we will need to examine actual privacy attacks on the minimized dataset. We recognize the importance of considering a wide range of threat models that reflect real-world privacy risks and allow us to evaluate the extent of leakage under various objectives and degrees of access available to the adversary.

To achieve this, we will introduce three different privacy metrics, each designed to simulate a specific information leakage scenario. The first two metrics focus on data breach, i.e., a situation in which the adversary has access to the minimized dataset, and we want to quantify the amount of information about the original dataset that we were able to safeguard by performing data minimization. The third metric focuses on model breach, i.e., an inspection of the impact of data minimization on privacy leakage through the trained model. We will now define these threat models in detail.

\paragraph{Re-identification Risk (RIR):}
One of the central concerns in privacy leakage due to data breach is the re-identification of individuals even in the presence of only partial or anonymized features. Re-identification attacks rely on an auxiliary dataset(s) $\cX^A$ to obtain public information about an individual, which can be matched with the partial information in the target dataset to identify them~\cite{henriksen2016re}.

The effectiveness of the re-identification attack can be evaluated through the utilization of mean reciprocal rank (MRR) scores~\cite{}, which assess the quality of the rankings provided by an attacker. Specifically, for each data point $x_i^A$ in the auxiliary dataset $\cX^A$, the adversary generates a ranking of all data points in the minimized dataset $\cX' = \cX \odot \cB$ based on their likelihood of being the same corresponding individual. The re-identification risk (RIR) can then be quantified by computing the average MRR scores, where a score of $1$ is assigned to the correct match and a score of $0$ is assigned otherwise:
\begin{align}
    \textrm{RIR} = \frac{1}{|\cX^A|} \sum\limits_{i=1}^{|\cX^A|} \frac{1}{\textrm{index}(i, \textrm{rank}(x_i^A, \cX'))}
\end{align}
where $\textrm{rank}(x_i^A, \cX')$ represent the ranking of data points as predicted by the adversary, and $\textrm{index}(e, A)$ returns the index (1-based indexing) of some element $e$ in the array $A$. Here, we assume one-to-one mapping between auxiliary and minimized datasets, i.e., every $i^{th}$ data point in the auxiliary dataset and in the minimized dataset corresponds to the same individual.

\paragraph{Reconstruction Risk (RCR):}

Real-world datasets typically exhibit underlying associations between input features, making it possible to approximate missing features by studying the remaining data. Even if certain information is removed from the dataset, there is no guarantee that it cannot be reconstructed using the rest of the data. Reconstruction attacks thus aim to recover missing information from a target dataset, often using aggregate statistics about the dataset distribution.

Given the minimized dataset $\cX'$, the attacker's goal is to generate their optimal reconstruction $\cX^R$ of the original set of features $\cX$. The reconstruction risk (RCR) can be evaluated by measuring the similarity between the original features $x_i \in \cX$ and the reconstructed features $x_i^R \in \cX^R$, computed as the negative exponential of the euclidean distance:
\begin{align}
    \textrm{RCR} = \frac{1}{|\cX|} \sum\limits_{i=1}^{|\cX|} e^{-|| x_i - x_i^R ||_2}
\end{align}
While this metric treats the reconstruction of all features with equal importance, adjustments can be made to prioritize or disregard the reconstruction of specific features.

\paragraph{Membership Inference Risk (MIR):}

Membership inference attacks threaten the privacy of individuals by attempting to determine whether their data was included in the original dataset prior to minimization. While the previous privacy attacks were focused on the attacker accessing the minimized dataset $\cX'$, here we will instead focus on the attacker accessing a model trained on the minimized dataset $\theta^*_{\cX'}$, i.e., the traditional membership inference setting~\cite{}.

During a membership inference attack, the adversary assigns a likelihood score $L(x_q)$ to each query $x_q$, indicating the probability of it being a member of the original dataset $\cX$ given access to the model trained on the minimized dataset, i.e., $L(x_q) = P[x_q \in \cX | \theta^*_{\cX'}]$. Using these likelihood scores for both the original data points $\cX$ and a set of non-members $\cX_{nm}$, binary predictions for membership can be generated for any threshold $t$, denoted as $1_{L(x_q) \geq t}$. The membership inference risk (MIR) is the area under the curve (AUC) of the true positive rates and false positive rates across thresholds, i.e., $\vec{tpr}={tpr_{t=t_1}, tpr_{t=t_2}, ..}$ and $\vec{fpr}={fpr_{t=t_1}, fpr_{t=t_2}, ..}$
:
\begin{align}
    \textrm{MIR} = \textrm{AUC}(\vec{tpr}, \vec{fpr})
\end{align}

% \begin{mdframed}
%     Our work focuses on three main objectives: \emph{maintaining utility}, \emph{preserving privacy}, and \emph{ensuring computational efficiency}. We strive to strike a balance between dataset utility and safeguarding against potential privacy breaches, while recognizing the importance of computational efficiency in practical applications. We aim to develop a framework that can be easily adapted and deployed by data holders to perform minimization.
% \end{mdframed}





% \subsubsection{Data Imputation}
% Sometimes, prior to releasing the data, the data holder may find it necessary to impute missing values in the minimized dataset. This is particularly relevant when the dataset release is expected to be complete and devoid of any missing entries, as required to train many ML algorithms.

% Imputation involves filling in the missing values of the minimized features $x_i' \in \cX'$ with estimated or imputed values to get the features $x_i'' \in \cX''$. It should be noted that the imputed dataset will have less information compared to the minimized dataset, because it no longer contains information about the specific set of feature values that were minimized. In our paper, we employ a simple imputation method that assumes an underlying multivariate gaussian distribution between all features in the dataset and imputes missing values using statistical measures like mean and covariance. While this method is rudimentary, for the purposes of our study, this provides a suitable framework to demonstrate the effects of imputation on the minimized dataset.

% \subsubsection{Preserving Utility}
% In a supervised setting, in the context of data minimization, the preservation of utility can be quantified through the minimization of the empirical risk associated with training a model on the minimized dataset $\cD' = \{x_i \cdot \cB_i, y_i\}^n_{i=1}$. For a given loss function $\ell(\cdot)$, the objective is to find the optimal parameter values $\theta^*$ that minimize the empirical risk. This can be expressed as:

% $$ \theta^* = \text{argmin}_{\theta} \sum^n_{i=1}  \ell\bigg(f_{\theta}(x_i \cdot B_i), y_i\bigg) $$

% Here, $f_{\theta}$ denotes the model with parameters $\theta$. By minimizing this empirical risk, we aim to ensure that the minimized dataset retains its utility during training.

\nando{Shouldnt' we talk about the adversaries here?}
\subsection{Threat Models}

\paragraph{Re-identification Attack: } The objective of a re-identification attack is to identify an individual given only partial information. The attacker's goal is thus finding the best match in the minimized dataset $\cX' = \cX \odot \cB$ for each data point in the auxiliary dataset (in our setup, simply the original dataset $\cX$). We use the euclidean distance measure to rank the best matches. However, since the minimized dataset contains holes, i.e., $\phi$ values in it, we instead use a euclidean distance metric that skips the missing values and scales the measured distance for the rest of the indices accordingly.

\paragraph{Reconstruction Attack: } The aim of reconstruction attacks is to recover missing information from the minimized dataset. To do so, we employ an imputation method $\cP$ that takes the minimized dataset $\cX'$ and some aggregate statistics $\cS$ as inputs, producing a reconstructed dataset $\cX^{\cP(\cX', \cS)}$ with no missing values. Our imputation method $\cP$ creates a multivariate gaussian distribution assumption for the input dataset $\cX$ and uses the mean and co-variance across all features in the dataset (i.e., the aggregate statistics $\cS$) to measure the expected value of the missing information.

\paragraph{Membership Inference Attack: } Membership inference attacks aim to determine the presence or absence of an individual in the original training dataset. We will employ the likelihood ratio attack (LiRA)~\cite{}, by training multiple shadow models on public data available from the same distribution. We will consider two specific cases of membership inference attacks, \textit{(i)} attacker has no knowledge of the data minimization algorithm, \textit{(ii)} attacker has access to the minimization algorithm used before training the target model. We train shadow models as done in the literature for the first case, while we perform data minimization before training shadow models in the second case.



==> archived_sections/archived_sec_setting_and_objective.tex <==
\section{Setting and Objectives}



The general data protection regulations (GDPR) express data minimization as the collection and retention of personal data that is \textit{adequate, relevant, and limited to what is necessary in relation to the purposes for which they are processed}. According to GDPR, personal data is \textit{any information relating to an identified or identifiable natural person}.
Thus, data minimization boils down to the collection of data that is \textit{adequate} enough to provide good performance, has some \textit{relevance} to the task (can be judged by domain experts), and is \textit{limited} such that the identification of an individual from the collected data is as uncertain as possible while adhering to the adequacy requirements.

Existing work in feature selection or active learning can be adapted to perform data minimization on a global scale. However, the principles of data minimization are highly personalized. That is, the adequacy of, the relevance of, or anonymity due to partial information sharing can vary significantly across two different individuals, even for the same task. Thus, studying personalized data minimization for each individual separately is important to fulfill the regulatory requirements of data minimization.

\subsection{Data Minimization in Retrospective}

First, we focus on the setting where we have access to the complete dataset, but we want to only retain the data that is \textit{adequate, relevant, and limited to what is necessary in relation to the purposes for which they are processed}. Thus, we perform personalized data minimization in retrospective.

\begin{definition}[Personalized Data Minimization in Retrospective]
    Given a dataset $\cD = \{x_i, y_i\}^n_{i=1}$, personalized data minimization $\cP(\cD)$ is a mapping from every data point $x_i$ to a random variable $X_i$ such that $x_i \in \cR_{X_i}$, where $\cR_{X}$ represents the support of a random variable $X$. The resulting minimized dataset can be represented as $\cD^{\cP} = \{X_i, y_i\}^n_{i=1}$.
\end{definition}

In simpler terms, personalized data minimization reduces each observation to a random variable whose sample space includes the original observation.

\begin{definition}[Adequacy Indicator]
    Given two learned functions $f_1, f_2$ and a data point $(x, y)$, the adequacy indicator is a boolean indicator of whether the performance of $f_1$ on $(x, y)$ is adequate in context of the performance of $f_2$ on the same data point $(x, y)$.

\end{definition}
Example: For classification tasks, one possible adequacy indicator can be $1_{|f_2(x)=y \rightarrow f_1(x)=y|}$. That is, if $f_2$ outputs the correct prediction class, then $f_1$ should also output the correct prediction class.

\begin{definition}[Adequacy of Personalized Data Minimization]
    Given a training dataset $\cD$, a validation dataset $\cD_{val}$, a learning algorithm $\cA$, and an adequacy indicator function $\cI_A$, the adequacy of minimized dataset $\cD^{\cP}$ can be judged as,
    \begin{align}
        Pr[\cI_A(\cA(\cD^{\cP}), \cA(\cD), x_i, y_i)=1] \geq 1 - \delta, \quad \forall x_i, y_i \in \cD_{val}
    \end{align}
    where the hyperparameter $\delta$ controls the strictness of data minimization.
\end{definition}

In simpler terms, it is highly likely (with probability greater than $1-\delta$) that the output produced by the function learned on the minimized dataset provides an adequate output in context of the function learned on the original dataset.

\begin{definition}[Limited Data Under Adequate Personalized Data Minimization]
    Given a training dataset $\cD = \{x_i, y_i\}^n_{i=1}$, one can output several minimized datasets $\cD^{\cP} = \{X_i, y_i\}^n_{i=1}$ that follow the adequacy requirements. The objective is then to find the minimized dataset that has the least amount of re-identification risk, which can be defined as,
    \begin{align}
        arg \min_{X_i} Pr[X_i=x_i], \quad \forall i \in [1, n]
    \end{align}
\end{definition}

\subsection{Active Learning}
Next, we consider the setting where we don't have retrospective access to a large dataset and instead we aim to collect new data actively. In such a setting, even the collection of data needs to be \textit{adequate, relevant, and limited to what is necessary in relation to the purposes for which they are processed}.

\begin{definition}[Personalized Data Minimization in Active Learning]
    Given a dataset $\cD = \{x_i, y_i\}^k_{i=1}$, and a random variable $\bar{X}_{k+1}$ representing partial information of a new data point with label $y_{k+1}$, personalized data minimization during active learning $\cP(\cD, \bar{X}_{k+1})$ is the collection of additional observations on this new data point to reduce the random variable to $X_{k+1}$ such that $\cR_{X_{k+1}} \subseteq \cR_{\bar{X}_{k+1}}$, where $\cR_{X}$ represents the support of a random variable $X$. The data point is then added to the dataset as $\cD = \cD \oplus (X_{k+1}, y_{k+1})$, and the process is repeated again for another data point.
\end{definition}

\begin{definition}[Adequacy Under Active Learning]
    Given a training dataset $\cD$, a validation dataset $\cD_{val}$, an additional data point $(x_{k+1}, y_{k+1})$, a learning algorithm $\cA$, and an adequacy indicator function $\cI_A$, the adequacy of the minimized data point $X_{k+1}$ during active learning can be judged as,
    \begin{align}
        Pr[\cI_A(\cA(\cD \oplus (X_{k+1}, y_{k+1})), \cA(\cD \oplus (x_{k+1}, y_{k+1})), x_i, y_i)=1] \geq 1 - \delta, \quad \forall x_i, y_i \in \cD_{val}
    \end{align}
    where the hyperparameter $\delta$ controls the strictness of data minimization.
\end{definition}

\begin{definition}[Limited Data Under Active Learning]
    Given a training dataset $\cD$ and an additional data point $(x_{k+1}, y_{k+1})$, both sampled from the random variables $(X, Y)$, one can collect several different partial observations $X_{k+1}$ that follow the adequacy requirements. The objective is then to find the observations that has the least amount of re-identification risk (or maintains some form of anonymity?), which can be defined as,
    \begin{align}
        % arg \min_{X_{k+1}} MI(X, X_{k+1})
        ?
    \end{align}

    % where $MI()$ represents the mutual information between two random variables.
\end{definition}

% \subsection{Data Minimization and Differential Privacy}

% \subsection{Case Study: Causal Graphs with Feature Order}

% We will study a special case in this section to better understand the trends of data minimization. We introduce the problem statement with the following assumptions,

% \begin{itemize}
%     \item Bayesian Learning Classification Task: We will focus specifically on classification task in a structured learning setting for this case study.
%     \item Feature Exclusion: We will only perform data minimization through complete feature exclusion, i.e., the feature value $x_i^j$ will be mapped to the random variable $X_j$ which represents the overall distribution of feature $j$.
%     \item Feature Order: We assume the presence of an inherent order across features for data minimization, i.e., for any two features $i, j$ where $i < j$, we always minimize feature $j$ before minimizing feature $i$.
% \end{itemize}

% Under the above assumptions, we will introduce an algorithm to do data minimization and show that one can guarantee adequacy of the learned algorithm under data minimization.

% \subsection{Adequacy Guarantees}
% Under the above assumptions, the final objective can be reduced to the following. Given a training dataset $\cD$, a validation dataset $\cD_{val}$, and a bayesian learning algorithm $\cS$, we want to create a minimized dataset $\cD^{\cP}$ which satisfies the following,
% \begin{align}
%     arg \min_{\cD^{\cP}} \Sigma_{(X_i, y_i) \in \cD^{\cP}} ||X_i||_l \\
%     s.t. \quad Pr[f_{\cD^{\cP}}(x_i)=y_i \mid f_{\cD}(x_i)=y_i] \geq 1 - \delta, \quad \forall x_i, y_i \in \cD_{val}
% \end{align}

% where $f_{\cD}$ and $f_{\cD^{\cP}}$ are bayesian inference models learned on datasets $\cD$ and $\cD^{\cP}$ respectively, and $\delta$ is the adequacy guarantee hyperparameter. Each minimized data point $X_i$ is a concatenation of observed features $x^o$ (random variables with only one member in the sample space) and unobserved features $x^u$ (random variables spanning the complete feature space), and $||X_i||_l$ represents the number of observed features in a data point. In other words, the objective is to minimize the total amount of data collected (where each feature from each individual is equally weighted), while fulfilling the adequacy requirements.

% For every possible permutation of data minimization, the calculation of the corresponding adequacy can be quite expensive, as it requires retraining the inference function $f_{\cD^{\cP}}$ every time. Can we do better? We will show that doing data minimization in retrospective on the training dataset without the need to retrain after every minimization step is good enough to provide us with adequacy guarantees in this particular setting.

% The data minimization algorithm is as follows. We perform data minimization on the training set as if we were doing data minimization during inference. That is, we do the following,
% \begin{align}
%     \min ||X_i||_l \\
%     s.t. \quad Pr[f_{\cD}(X_i)=y_i] \geq 1 - \delta, \quad \forall x_i, y_i \in \cD_{val}
% \end{align}

% Thus, we minimize each data point separately using the model trained on the complete dataset, and then use the now incomplete data to train a new model from scratch. We show below that such a method will guarantee adequacy with hyperparameter $\delta$, i.e. the same as the one used during data minimization.



==> archived_sections/cuong_sections/notes.tex <==
\section{Notes on Data minimization solving}

Let's assume we have a binary logistic regression problem with a dataset consisting of $n$ samples and $m$ features. Let $\mathbf{X}$ be the feature matrix ($n \times m$), $\mathbf{y}$ be the target vector ($n \times 1$), and $\mathbf{w}$ be the weight vector ($m \times 1$). We'll also use a regularization parameter $\lambda$ (from the upper-level problem) for L2 regularization.

\paragraph{Upper-level problem (ULP)}: 
Minimize the dataset size:
\begin{equation}
\begin{aligned}
& \min_{\mathbf{B}} \; \sum_{i=1}^{n} \sum_{j=1}^{m} b_{ij} \\
& \text{subject to } \; b_{ij} \in \{0, 1\}, \; \forall i = 1, \ldots, n, \; \forall j = 1, \ldots, m
\end{aligned}
\end{equation}


\paragraph{Lower-level problem (LLP)}: 
Logistic regression with sparse feature matrix $\mathbf{B} \mathbf{X}$
\begin{equation}
    \min_{\mathbf{w}} L(\mathbf{w}) = \sum_{i=1}^n \left[ -y_i \log(p_i) - (1 - y_i) \log(1 - p_i) \right] + \frac{\lambda}{2} \lVert \mathbf{w} \rVert^2 \\
\end{equation}



where $p_i = \frac{1}{1 + \exp(-(\mathbf{B}\mathbf{X})_i \mathbf{w})}$ is the predicted probability for the i-th sample.

To apply KKT conditions, we first need to introduce inequality constraints. We can do this by reformulating the L2 regularization term using non-negative auxiliary variables, say $\mathbf{z}$ ($m \times 1$). Let's rewrite the regularization term as follows:

\begin{equation}
\frac{\lambda}{2} \lVert \mathbf{w} \rVert^2 = \frac{\lambda}{2} \sum_{j=1}^m w_j^2 = \frac{\lambda}{2} \sum_{j=1}^m \left(z_j^2 - z_j^2 + w_j^2\right) = \frac{\lambda}{2} \sum_{j=1}^m (z_j - w_j)(z_j + w_j)
\end{equation}

Now, the optimization problem becomes:


\begin{equation}
\begin{aligned}
\min_{\mathbf{w},\mathbf{z}} L(\mathbf{w}, \mathbf{z}) = 
    &\; \sum_{i=1}^n \left[ -y_i \log(p_i) - (1 - y_i) \log(1 - p_i) \right] + \frac{\lambda}{2} \sum_{j=1}^m (z_j - w_j)(z_j + w_j) \\
\text{subject to } 
    &\; z_j - w_j \geq 0, \; z_j + w_j \geq 0, \; \forall j = 1, \ldots, m
\end{aligned}
\end{equation}

\paragraph{KKT conditions}

\begin{enumerate}
    \item 
    Stationarity:
    \begin{equation}
    \begin{aligned}
    & \nabla_{\mathbf{w}} L(\mathbf{w}, \mathbf{z}) = 0 \\
    & \nabla_{\mathbf{z}} L(\mathbf{w}, \mathbf{z}) = 0
    \end{aligned}
    \end{equation}
    
    \item 
    Primal feasibility:
    \begin{equation}
    z_j - w_j \geq 0, \; z_j + w_j \geq 0, \; \
    \forall j = 1, \ldots, m
    \end{equation}
    
    \item 
    Dual feasibility:
    \begin{equation}
    \mu_j (z_j - w_j) = 0 \; \text{and} \; \nu_j (z_j + w_j) = 0, \; \forall j = 1, \ldots, m
    \end{equation}
    where $\mu_j$ and $\nu_j$ are the Lagrange multipliers for the inequality constraints.
    
    \item 
    Complementary slackness:
    \begin{equation}
    \mu_j \geq 0, \; \nu_j \geq 0, \; \forall j = 1, \ldots, m
    \end{equation}
    \end{enumerate}


\paragraph{Solving the lower-level problem}

\begin{enumerate}
    \item Calculate the gradients of the objective function with respect to $\mathbf{w}$ and $\mathbf{z}$. To do this, we can use the chain rule:
    \begin{equation}
    \begin{aligned}
    \frac{\partial L}{\partial w_j} &= -\sum_{i=1}^n \left[ y_i \frac{\partial \log(p_i)}{\partial w_j} + (1 - y_i) \frac{\partial \log(1 - p_i)}{\partial w_j} \right] + \lambda(z_j - w_j) - \lambda(z_j + w_j) \\
    \frac{\partial L}{\partial z_j} &= \lambda(z_j - w_j) + \lambda(z_j + w_j)
    \end{aligned}
    \end{equation}
    
    \item
    Set the gradients to zero to get the stationarity conditions:
    \begin{equation}
    \begin{aligned}
    \frac{\partial L}{\partial w_j} &= 0 \\
    \frac{\partial L}{\partial z_j} &= 0
    \end{aligned}
    \end{equation}
    
    \item 
    Solve the resulting system of nonlinear equations for $\mathbf{w}$, $\mathbf{z}$, $\boldsymbol{\mu}$, and $\boldsymbol{\nu}$ (either using numerical methods -- interior points, Newton's method) or exploiting the specific structure of the problem.
    
    \item 
    Check the primal feasibility, dual feasibility, and complementary slackness conditions. 
\end{enumerate} 


\paragraph{Alternative single-level problem}

\begin{equation}
\begin{aligned}
& \min_{\mathbf{w}, \mathbf{B}} \sum_{i=1}^n \left[ -y_i \log(p_i) - (1 - y_i) \log(1 - p_i) \right] + \frac{\lambda}{2} \lVert \mathbf{w} \rVert^2 + \gamma \sum_{i=1}^{n} \sum_{j=1}^{m} b_{ij} \\
& \text{subject to } \; 0 \leq b_{ij} \leq 1, \; \forall i = 1, \ldots, n, \; \forall j = 1, \ldots, m \\
& \text{and } p_i = \frac{1}{1 + \exp(-(\mathbf{B}\mathbf{X})_i \mathbf{w})}
\end{aligned}
\end{equation}

In this formulation, the regularization term $\gamma \sum_{i=1}^{n} \sum_{j=1}^{m} b_{ij}$ encourages sparsity in matrix $\mathbf{B}$, while the continuous constraint $0 \leq b_{ij} \leq 1$ replaces the original binary constraint. The parameter $\gamma$ controls the trade-off between the sparsity of $\mathbf{B}$ and the logistic regression problem's fit.


==> archived_sections/cuong_sections/sec_data_minimization_principle.tex <==
We will begin by establishing our framework for data minimization. We have utilized legal language from six data protection regulations worldwide to define data minimization and its objectives. Our initial focus is on faithfully transforming the legal requirements into an optimization problem, which we find only considers dataset size and utility. Subsequently, we also discuss the privacy implications of data minimization within the context of these regulations and introduce several threat models to complete our framework. See Figure \ref{fig:framework} for an overall representation of our framework.

\subsection{Formalizing Data Minimization}

We will start by formalizing a framework for data minimization in machine learning and define an optimization problem associated with the objectives of data minimization.

\input{tables/tab_legal}

\paragraph{Purpose Limitation:} Data protection regulations require that data shall only be collected for a \textit{specific, explicitly defined and lawful purpose} (POPIA, South Africa) and that the data collector shall not \textit{use (sensitive) personal information collected for additional purposes that are incompatible with the disclosed purpose for which the (sensitive) personal information was collected} (CPRA, USA). See Table \ref{tab:legal} for purpose limitation in other regulations (highlighted in {\color{magenta}magenta}). Clearly, before diving into data minimization, it is crucial to first define the purpose of data collection.

In machine learning, data collection is essential for training a learning model. More precisely, the purpose of collecting data can be quantified as the success of the learned model, i.e., through a utility function, commonly a loss function.
Consider a dataset $\cD = (\cX, \cY) = \{x_i, y_i\}^n_{i=1}$ consisting of $n$ data points, where each data point is a tuple comprising of input features $x_i \in \cR^{d}$ and the associated output label $y_i$. In a typical ML setup, the learning objective can be defined as:
\begin{align}
    \theta^* = \arg\max_{\theta} \textrm{ } U(\cX ,\cY, \theta)
\end{align}
Here $U(.)$ represents the utility function for the task at hand. For instance, when performing empirical risk minimization (ERM) for learning, the utility function can be defined as: 
\begin{align}
    U(\cX, \cY, \theta) = - \cL_{ERM}(\cX, \cY, \theta)\\
    \textrm{where} \quad \quad \cL_{ERM}(\cX, \cY, \theta) = \sum^n_{i=1} \ell \big( f_{\boldsymbol{\theta}}(x_i) ,y_i \big) +\lambda \| \bm{\theta}\|^2
\end{align}
Here $f_\theta(.)$ represents the inference function of a learned model with parameters $\theta$, $\ell(.)$ is an appropriate loss function depending on the learning task (e.g., MSE loss or cross entropy) and $\lambda$ is the regularization parameter.

\paragraph{Personalized Decisions:} Now that we have defined an explicit purpose for our data collection, we can focus on formalizing data minimization. Data minimization is simply a set of binary decisions regarding the collection and/or retention of each individual information in the dataset. These decisions are inherently personalized. For example, consider the ACSEmployment dataset, which contains information about individuals, including their age, income, race, military history, medical history, etc., with the objective of inferring their employment status. Clearly, some individuals' employment status can be inferred from their age and/or income alone, rendering the release of their military or medical history unnecessary, while for others these additional attributes may be crucial to understanding their employment status.

Formally, these decisions during data minimization can be captured using a binary matrix $\cB \in \{\phi,1\}^{n \times d}$, which we call the \emph{minimization matrix}. Here, the symbol $\phi$ represents the concealment or removal of redundant values in the dataset, i.e., $\forall a \in \R: a \times \phi = \phi$. The minimized input feature set $\cX'$ can then be defined as the element-wise product of the original feature set $\cX$ and the minimization matrix $\cB$, i.e., $\cX' = \cX \odot \cB$. Note that we are left with empty values $\phi$ in the minimized feature set $\cX'$. While some learning algorithms are capable of handling missing values in the dataset, in most cases one would also need to impute the minimized dataset using average statistics or more advanced techniques.

\paragraph{Data Minimization is Data-Dependent:} 
To accurately assess the relevance of data for a particular purpose, it is important to inspect the complete data, i.e. data minimization is inherently data-dependent. Making a decision on collecting and/or retaining parts of the data without considering its actual value can lead to valuable information being excluded or irrelevant data being included, thus compromising the utility of the minimized dataset. Moreover, making such preemptive choices can introduce biases in our dataset, since the expected value of data cannot capture the diversity of representation. Thus, throughout our discussion of data minimization, we will focus on the setting where the data handler has initial access to the complete data, and then makes decisions on retaining or deleting parts of the data, according to the objectives of data minimization discussed next.

% Most laws and regulations on data handling require that the data collector does not \textit{collect more data than is reasonably needed} (The Privacy Act) and the said data \textit{not be retained any longer than is necessary for achieving the purpose for which the information was collected} (POPIA). See Table \ref{tab:legal} for language on data collection and retention in other regulations (highlighted in {\color{green}green}). Formally, data minimization is simply a set of binary decisions regarding the collection and/or retention of each individual value in the dataset.

\paragraph{Limited and Necessary to the Purpose:} We have defined the purpose of data collection in ML and formalized a mathematical formulation of data minimization. Finally, we connect the two by focusing on the objective of data collection with respect to the defined purpose. Existing regulations require that collected data \textit{shall be adequate, relevant and limited to what is necessary in relation to the purposes for which they are processed} (GDPR, Europe), or similarly be \textit{relevant, proportional and non-excessive in relation to purposes of the data processing} (LGPD, Brazil). See Table \ref{tab:legal} for language on objectives of data collection in other regulations (highlighted in {\color{blue}blue}). In direct terms, data minimization aims to remove any redundant values in the dataset that do not contribute to the utility of the learned model.

We can define the objective of data minimization as finding an optimal minimization matrix $\cB^*$ that can minimize the dataset size while retaining its utility, i.e.: 
\begin{align}
    \cB^* = \arg\min_{\cB} ||\cB||_0 \quad \textrm{where} \quad \cB \in \cF_{\cB}
\end{align}
Here $||\cB||_0$ is the $l_0$ norm of the minimization matrix, defined as simply the number of indices where $\cB_{ij}=1$, and $\cF_{\cB}$ is a feasibility set of minimization matrices defined as:
\begin{align}
\label{eq:misalignment}
\cF_{\cB}=
\left\{
  \cB
\;\middle|\;
\begin{alignedat}{2}
  & \cA(\cX \odot \cB, \cX) \leq \alpha \\
  & \cB \in \{\phi,1\}^{n \times d}
\end{alignedat}
\right\}
\end{align}
Here $\cA(\cX_1, \cX_2)$ represents the misalignment in utility between two learning models trained on the datasets $(\cX_1, \cY)$ and $(\cX_2, \cY)$ respectively, and $\alpha$ is the maximum amount of misalignment permitted during minimization, which represents the threshold for maintaining utility. For instance, we can define misalignment as simply the difference in loss values between the two learned models, i.e.:
\begin{align}
    \cA(\cX \odot \cB, \cX) = \cL(\cX, \cY, \theta^*_{\cX \odot \cB}) - \cL(\cX, \cY, \theta^*_{\cX}) \\
    \textrm{where} \quad \theta^*_{\cX} = \arg\min_{\theta} \cL(\cX, \cY, \theta)
\end{align}
Here $\cL(.)$ represents the loss function used to measure the utility of the trained model. The misalignment is defined such that even though our model is trained on the minimized dataset with missing values, it should perform well on the full dataset, i.e., the inference behaviour remains unchanged.

In some scenarios, instead of minimizing the $\| \cB\|_0$ under the misalignment  constraint, it is more interested to put the constraint over $\| \cB\|_0$ and see what is  the maximum utility when using the model $\bm{\theta}_{\cX \odot \cB}$ that we can obtain. This can be formulated in the following optimization problem:

\textbf{Main optimization }
\begin{align}
\min_{\cB}& \, \,   \cL\big(\cX, \cY, \bm{\theta^{*}}_{\cX \odot \cB}\big)\\  \label{eq:main_obj}
\mbox{s.t:}  & \, \, \bm{\theta^{*}}_{\cX \odot \cB} = \mbox{argmin}_{\bm{\theta}} \cL\big(\cX \odot \cB, \cY, \bm{\theta}\big)  \label{eq:eq_constraint}
\\
\mbox{and}  & \, \, \cB \in \{0,1\}^{n\times d} \, \mbox{,} \, \| \cB\|_0 \leq k 
\label{eq:capacity_constraint}
\end{align}

Where $k$ is the capacity constraint over $\cB$, indicating the number of feature entries that we want to keep. In the scope of this paper, we will focus on this setting, since it allows the data owners the flexibility to control the amount of data they want to retain.
% We can thus formalize the overall data minimization objective as a bilevel optimization:
% \begin{align}
%     \arg\min_{\cB} ||\cB||_0 + \lambda*(\cL(\cX, \cY, \theta^*_{\cX \odot \cB}) - L_{c} - \alpha + t^2) \\
%     \textrm{where} \quad \theta^*_{\cX \odot \cB} = \arg\min_{\theta} \cL(\cX \odot \cB, \cY, \theta)
% \end{align}
% Here $\lambda, t^2$ represent the lagrangian multiplier and the slack variable respectively, for the misalignment constraints in Eq. \ref{eq:misalignment}. $L_{c}$ is a constant value independent of the minimization matrix $\cB$, defined as $L_{c} = \cL(\cX, \cY, \theta^*_{\cX})$. Note that $\cB$ can only take certain discrete values, i.e., $\cB \in \{\phi,1\}^{n \times d}$.

\subsection{Privacy Leakage}

In current data protection regulations, personal data is defined as any information that directly \textit{identifies a particular individual}, or can be indirectly \textit{combined with other information to identify a particular individual} (PIPA, South Korea). See Table \ref{tab:legal} for other similar definitions of personal data across various regulations (highlighted in {\color{orange}orange}). It is clear that these regulations prioritize data minimization to avoid collecting unnecessary information that could compromise an individual's privacy. However, data minimization doesn't necessarily equate to the best practices for privacy protection under some utility constraints. For instance, additional data can in some cases provide anonymization to individuals, which would not align with the objectives of data minimization. 

Our work aims to clarify the relationship between data minimization and privacy to understand both the benefits and the limitations of data minimization in safeguarding individuals' privacy in a dataset. In order to measure the privacy benefits of data minimization, we will need to examine actual privacy attacks on the minimized dataset. We recognize the importance of considering a wide range of threat models that reflect real-world privacy risks and allow us to evaluate the extent of leakage under various objectives and degrees of access available to the adversary.

To achieve this, we will introduce three different privacy metrics, each designed to simulate a specific information leakage scenario. The first two metrics focus on data breach, i.e., a situation in which the adversary has access to the minimized dataset, and we want to quantify the amount of information about the original dataset that we were able to safeguard by performing data minimization. The third metric focuses on model breach, i.e., an inspection of the impact of data minimization on privacy leakage through the trained model. We will now define these threat models in detail.

\paragraph{Re-identification Risk (RIR):}
One of the central concerns in privacy leakage due to data breach is the re-identification of individuals even in the presence of only partial or anonymized features. Re-identification attacks rely on an auxiliary dataset(s) $\cX^A$ to obtain public information about an individual, which can be matched with the partial information in the target dataset to identify them~\cite{henriksen2016re}.

The effectiveness of the re-identification attack can be evaluated through the utilization of mean reciprocal rank (MRR) scores~\cite{}, which assess the quality of the rankings provided by an attacker. Specifically, for each data point $x_i^A$ in the auxiliary dataset $\cX^A$, the adversary generates a ranking of all data points in the minimized dataset $\cX' = \cX \odot \cB$ based on their likelihood of being the same corresponding individual. The re-identification risk (RIR) can then be quantified by computing the average MRR scores, where a score of $1$ is assigned to the correct match and a score of $0$ is assigned otherwise:
\begin{align}
    \textrm{RIR} = \frac{1}{|\cX^A|} \sum\limits_{i=1}^{|\cX^A|} \frac{1}{\textrm{index}(i, \textrm{rank}(x_i^A, \cX'))}
\end{align}
where $\textrm{rank}(x_i^A, \cX')$ represent the ranking of data points as predicted by the adversary, and $\textrm{index}(e, A)$ returns the index (1-based indexing) of some element $e$ in the array $A$. Here, we assume one-to-one mapping between auxiliary and minimized datasets, i.e., every $i^{th}$ data point in the auxiliary dataset and in the minimized dataset corresponds to the same individual.

\paragraph{Reconstruction Risk (RCR):}

Real-world datasets typically exhibit underlying associations between input features, making it possible to approximate missing features by studying the remaining data. Even if certain information is removed from the dataset, there is no guarantee that it cannot be reconstructed using the rest of the data. Reconstruction attacks thus aim to recover missing information from a target dataset, often using aggregate statistics about the dataset distribution.

Given the minimized dataset $\cX'$, the attacker's goal is to generate their optimal reconstruction $\cX^R$ of the original set of features $\cX$. The reconstruction risk (RCR) can be evaluated by measuring the similarity between the original features $x_i \in \cX$ and the reconstructed features $x_i^R \in \cX^R$, computed as the negative exponential of the euclidean distance:
\begin{align}
    \textrm{RCR} = \frac{1}{|\cX|} \sum\limits_{i=1}^{|\cX|} e^{-|| x_i - x_i^R ||_2}
\end{align}
While this metric treats the reconstruction of all features with equal importance, adjustments can be made to prioritize or disregard the reconstruction of specific features.

\paragraph{Membership Inference Risk (MIR):}

Membership inference attacks threaten the privacy of individuals by attempting to determine whether their data was included in the original dataset prior to minimization. While the previous privacy attacks were focused on the attacker accessing the minimized dataset $\cX'$, here we will instead focus on the attacker accessing a model trained on the minimized dataset $\theta^*_{\cX'}$, i.e., the traditional membership inference setting~\cite{}.

During a membership inference attack, the adversary assigns a likelihood score $L(x_q)$ to each query $x_q$, indicating the probability of it being a member of the original dataset $\cX$ given access to the model trained on the minimized dataset, i.e., $L(x_q) = P[x_q \in \cX | \theta^*_{\cX'}]$. Using these likelihood scores for both the original data points $\cX$ and a set of non-members $\cX_{nm}$, binary predictions for membership can be generated for any threshold $t$, denoted as $1_{L(x_q) \geq t}$. The membership inference risk (MIR) is the area under the curve (AUC) of the true positive rates and false positive rates across thresholds, i.e., $\vec{tpr}={tpr_{t=t_1}, tpr_{t=t_2}, ..}$ and $\vec{fpr}={fpr_{t=t_1}, fpr_{t=t_2}, ..}$:
\begin{align}
    \textrm{MIR} = \textrm{AUC}(\vec{tpr}, \vec{fpr})
\end{align}

% \begin{mdframed}
%     Our work focuses on three main objectives: \emph{maintaining utility}, \emph{preserving privacy}, and \emph{ensuring computational efficiency}. We strive to strike a balance between dataset utility and safeguarding against potential privacy breaches, while recognizing the importance of computational efficiency in practical applications. We aim to develop a framework that can be easily adapted and deployed by data holders to perform minimization.
% \end{mdframed}





% \subsubsection{Data Imputation}
% Sometimes, prior to releasing the data, the data holder may find it necessary to impute missing values in the minimized dataset. This is particularly relevant when the dataset release is expected to be complete and devoid of any missing entries, as required to train many ML algorithms.

% Imputation involves filling in the missing values of the minimized features $x_i' \in \cX'$ with estimated or imputed values to get the features $x_i'' \in \cX''$. It should be noted that the imputed dataset will have less information compared to the minimized dataset, because it no longer contains information about the specific set of feature values that were minimized. In our paper, we employ a simple imputation method that assumes an underlying multivariate gaussian distribution between all features in the dataset and imputes missing values using statistical measures like mean and covariance. While this method is rudimentary, for the purposes of our study, this provides a suitable framework to demonstrate the effects of imputation on the minimized dataset.

% \subsubsection{Preserving Utility}
% In a supervised setting, in the context of data minimization, the preservation of utility can be quantified through the minimization of the empirical risk associated with training a model on the minimized dataset $\cD' = \{x_i \cdot \cB_i, y_i\}^n_{i=1}$. For a given loss function $\ell(\cdot)$, the objective is to find the optimal parameter values $\theta^*$ that minimize the empirical risk. This can be expressed as:

% $$ \theta^* = \text{argmin}_{\theta} \sum^n_{i=1}  \ell\bigg(f_{\theta}(x_i \cdot B_i), y_i\bigg) $$

% Here, $f_{\theta}$ denotes the model with parameters $\theta$. By minimizing this empirical risk, we aim to ensure that the minimized dataset retains its utility during training.

==> archived_sections/cuong_sections/sec_evaluations.tex <==
\subsection{TODO: Add Experiment Setup and Results}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_dataset_size_minimization} 
    \caption{Model Accuracy vs Dataset Size: Logistic Regression and Bag of Words}
	\label{fig:dataset_size}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_reidentification_minimization} 
    \caption{Model Accuracy vs Reidentification Risk: Logistic Regression (Tabular Datasets Only)}
	\label{fig:reid}
\end{figure*}


\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_reconstruction_minimization} 
    \caption{Model Accuracy vs Reconstruction Risk: Logistic Regression (Tabular Datasets Only)}
	\label{fig:recon}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_ner_minimization} 
    \caption{Model Accuracy vs Number of Named Entities: Bag of Words (Text Datasets Only)}
	\label{fig:ner}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_nn_dataset_size_minimization} 
    \caption{Model Accuracy vs Dataset Size: MLP Single Hidden Layer (Tabular Datasets Only)}
	\label{fig:nn_dataset_size}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_nn_reidentification_minimization} 
    \caption{Model Accuracy vs Reidentification Risk: MLP Single Hidden Layer (Tabular Datasets Only)}
	\label{fig:nn_reid}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_nn_reconstruction_minimization} 
    \caption{Model Accuracy vs Reconstruction Risk: MLP Single Hidden Layer (Tabular Datasets Only)}
	\label{fig:nn_recon}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_nn_mia_minimization} 
    \caption{Model Accuracy vs MIA Risk: MLP Single Hidden Layer (Tabular Datasets Only)}
	\label{fig:nn_mia}
\end{figure*}

\input{tables/tab_multiplicity}

==> archived_sections/cuong_sections/sec_experiment_setup.tex <==
\subsection{Threat Models}

\paragraph{Re-identification Attack: } The objective of a re-identification attack is to identify an individual given only partial information. The attacker's goal is thus finding the best match in the minimized dataset $\cX' = \cX \odot \cB$ for each data point in the auxiliary dataset (in our setup, simply the original dataset $\cX$). We use the euclidean distance measure to rank the best matches. However, since the minimized dataset contains holes, i.e., $\phi$ values in it, we instead use a euclidean distance metric that skips the missing values and scales the measured distance for the rest of the indices accordingly.

\paragraph{Reconstruction Attack: } The aim of reconstruction attacks is to recover missing information from the minimized dataset. To do so, we employ an imputation method $\cP$ that takes the minimized dataset $\cX'$ and some aggregate statistics $\cS$ as inputs, producing a reconstructed dataset $\cX^{\cP(\cX', \cS)}$ with no missing values. Our imputation method $\cP$ creates a multivariate gaussian distribution assumption for the input dataset $\cX$ and uses the mean and co-variance across all features in the dataset (i.e., the aggregate statistics $\cS$) to measure the expected value of the missing information.

\paragraph{Membership Inference Attack: } Membership inference attacks aim to determine the presence or absence of an individual in the original training dataset. We will employ the likelihood ratio attack (LiRA)~\cite{}, by training multiple shadow models on public data available from the same distribution. We will consider two specific cases of membership inference attacks, \textit{(i)} attacker has no knowledge of the data minimization algorithm, \textit{(ii)} attacker has access to the minimization algorithm used before training the target model. We train shadow models as done in the literature for the first case, while we perform data minimization before training shadow models in the second case.

\subsection{Data Minimization Baselines}

We introduce three baseline techniques for data minimization, namely feature selection, random subsampling, personalized random subsampling,

\paragraph{Feature Selection:} Feature selection is simply choosing the most important features while removing the rest and is a commonly used method to reduce dataset size in machine learning~\cite{}. The minimization matrix can be defined as:
\begin{align}
    \cB_{ij} = \phi \quad \forall j \in E_s
\end{align}
Here $E_s$ is the set of $s$ least important features in the dataset, and $s$ is a hyperparameter which controls the sparsity of the minimized dataset. We use the absolute value of the coefficients of a logistic regression trained on $\cX$ to measure the importance of each feature.

\paragraph{Random Subsampling:} Random subsampling is a minimization method that randomly chooses a subset of data points from the original dataset, and is another very common technique of reducing dataset size for faster training~\cite{}. The minimization matrix can be defined as:
\begin{align}
    \cB_{ij} = \phi \quad \forall \, U_i=0
\end{align}
Here $U \in \{0, 1\}^n$ is a randomly permuted binary vector, with exactly $s$ indices filled with $1$, i.e., $\Sigma_i U_{i} = s$, to control the desired sparsity of the minimization.

\paragraph{Personalized Random Subsampling:} Personalized random subsampling is an extension of random subsampling, but instead of removing complete data points it removes individual values in the dataset matrix, i.e. perform personalized minimization. The minimization matrix can be defined as:
\begin{align}
    \cB_{ij} = \phi \quad \forall \, U^P_{ij}=0
\end{align}
Here $U^P \in \{0, 1\}^{n \times d}$ is a randomly permuted binary matrix, with exactly $s$ indices filled with $1$, i.e., $\Sigma_{ij} U^P_{ij} = s$, to control the desired sparsity of the minimization.

% \textcolor{blue}{Some desirable theorems can be,
% \begin{enumerate}
%     \item Theorem: Under some given constraints of the dataset distribution (for example, maybe we can assume gaussian distribution), we show that the drop in performance for personalized random subsampling is bounded. That is, there are certain guarantees that you get with personalized random subsampling method.
%     \item Theorem: Under some given constraints, we show that the drop in performance for personalized random subsampling is always less than that of just random subsampling. That is, we motivate the 'personalized' nature of data minimization.
% \end{enumerate}}

\subsection{Datasets and Models}
[TODO]

\paragraph{Tabular Datasets: } We will perform most of our experiments and ablations studies on various tabular datasets. More specifically, we will study data minimization on the Bank Dataset, the Wine Dataset, and the Employment Dataset, respectively. For all datasets, we first divide the dataset by half into private and public splits (for membership inference attacks), and then we further divide the private data by half for train and test splits respectively.

\paragraph{Text Datasets: }

==> archived_sections/cuong_sections/sec_gradient_based_solution.tex <==
\subsection{Efficient approximation of target utility}
\label{sec:approximation_method}
The difficulty of solving the main optimization in Section \ref{sec:data_minimization} lies on the equality constraint in Equation \ref{eq:eq_constraint} and the binary constraint over $\cB$ in Equation \ref{eq:capacity_constraint}. Our first proposed method relies on approximating directly the target utility $\cL(\cX, \cY, \bm{\theta^{*}}_{\cX \odot \cB} )$ by the following Lemma \ref{lem:taylor}


\begin{lemma}
The target utility  of interest $\cL(\cX, \cY, \bm{\theta^{*}}_{\cX \odot \cB} )$ can be aproximated by the original utility $\cL(\cX, \cY, \bm{\theta^{*}}_{\cX} )$  as follows:

$$ \cL(\cX, \cY, \bm{\theta^{*}}_{\cX'} ) \approx \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) + (X'-X)^T L H^{-1} G + \cO\big( \| X'-X\|^2\big)$$,
where:

$$ L =\frac{\partial \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta}}  \,\, \text{(1st derivative w.r.t param )}$$


$$ H =\frac{\partial^2 \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta}^2} \, \, \mbox{ (Hessian matrix of param) } $$

$$G = \frac{\partial^2 \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta} \partial \cX} \, \, \mbox{ (2nd derivative w.r.t param and input) }$$

\label{lem:taylor}
\end{lemma}

It is noted that the matrix multiplication $L H^{-1} G$ is a constant w.r.t $\cB$ and we can put  $S =L H^{-1} G  \in R^{n\times d}$. Given Lemma \ref{lem:taylor}, and suppose the term $O\big(\|X'-X\|^2 \big)$ is negligible, then the main optimization in Section \ref{sec:data_minimization}  can be simply reduced to the following integer linear programming:

\begin{align}
\min_{\cB} & \, (X\cdot \cB - X)^T C \\
\mbox{s.t:} & \, \, \cB \in \{0,1\}^{n\times d} \, \mbox{,} \, \| \cB\|_0 \leq k \label{eq:integer_program}
\end{align}

The solution of the binary linear  programming turns out to be setting $\cB_{ij}=1$ for the $k$ largest entries $ ( \cX_{i,j} -\phi) C_{ij}$
 and $\cB_{ij}=0$ otherwise. 

==> archived_sections/cuong_sections/sec_introduction.tex <==
As data-driven systems and machine learning (ML) applications continue to proliferate, they introduce new privacy risks, necessitating robust data protection measures \cite{}. 
Several international data protection frameworks, such as the General Data Protection Regulation (GDPR)~\cite{}, the California Privacy Rights Act (CPRA)~\cite{}, and the Brazilian General Data Protection Law (LGPD)~\cite{}, have consequently adopted the principle of \emph{data minimization} as a privacy cornerstone.


Defined in Article 5(1)(c) of the GDPR, data minimization mandates organizations to \emph{collect, process, and retain only personal data that is adequate, relevant, and limited to what is necessary for specific objectives} (for further details, see Table \ref{tab:legal}). Therein, \emph{personal data} refers to \emph{any information relating to an identified or identifiable natural person}. 
In essence, this principle aims to reduce the amount of data collected and retained to minimize the potential for misuse, unauthorized access, or data breaches. 
%In essence, data handlers should not process or store data that may compromise individual privacy unless the data in question serves a precise, justifiable purpose, i.e. removing it will hurt their purpose.
% and Article 4(1)(c) of Regulation (EU) 2018/1725
% By adhering to this principle, organizations not only mitigate risks associated with data handling but also align with legal frameworks, enhancing user trust and regulatory compliance.

Despite being rooted in privacy-by-design principles and endorsed by various global data protection regulations, current academic discourse lacks a rigorous mathematical formulation of data minimization that can be implemented in real-wolrd ML applications. 
This leads to incomplete treatments that often overlook two crucial aspects of data minimization {\bf (1)} its personalized nature and {\bf (2)} its intrinsic link to privacy.

\paragraph{Personalization in data minimization.} Previous studies in structured data preprocessing like feature selection~\cite{}, data sampling~\cite{}, and active learning~\cite{}, have been adapted to match the objectives of data minimization. However, data minimization is inherently personalized, i.e. unique to each individual. The particular information required from one person for a specific purpose may differ greatly from what is necessary for another person for the same purpose. Most existing works on data minimization in ML do not address this personalized aspect of data minimization~\cite{}.

\paragraph{Data minimization and privacy.}
By minimizing the amount of personal data collected and/or processed, the risks of privacy violations can be reduced while still allowing for effective data analysis and model training. Yet, simply minimizing the amount of data is not the optimal approach to preserve the privacy of individuals. Given the expectations of privacy from data minimization in various data protection regulations, it is important to explore the extent to which the data minimization principle aligns with various real-world privacy risks. Unfortunately, the current literature on data minimization has predominantly focused on reducing the raw dataset size as the only measure of minimization quality and does not address the privacy implications of minimization.

% Thus, it is important to effectively tackle the privacy aspect and personalized nature of data minimization.

% TODO: Improving the Figure
\begin{figure*}
    \centering
    \input{figure_scripts/fig_framework} 
    \caption{An overview of our framework to study data minimization, and its place in a real-world ML pipeline. In the first half of the pipeline, we highlight the {\color{blue}formalization of data minimization} and quantify the risks of a {\color{red}data breach}. In the second half, i.e., under the assumption of secure data transmission to train the learning model, we establish the objectives of data minimization through {\color{olive}utility measurement} and further study potential privacy leakage through {\color{red}model breach/release}. Our framework offers a comprehensive perspective on the integration of data minimization into responsible data collection and management.}
	\label{fig:framework}
\end{figure*}

In this paper, we bridge the gap between the legal definitions and the lack of a mathematical foundation for data minimization. We propose a comprehensive and faithful mathematical interpretation of the data minimization principle, creating a unified framework for the ongoing discussion of data minimization in ML. Our framework incorporates personalized data minimization and encompasses both privacy concerns and the utility perspective, which is vital for ensuring the effectiveness and usability of ML models. 

We use our framework to introduce several robust algorithms for data minimization in ML. Through these examples, we demonstrate the value of incorporating data minimization into ML systems, not only to ensure legal compliance but also as a powerful tool to enhance the privacy of data-driven applications. We also study various properties of the minimized datasets, including the emergent personalization during optimization, the multiplicity of data minimization, and its compatibility with existing privacy defence mechanisms.

% We present a systematic approach for evaluating the trade-offs between privacy and utility, enabling practitioners to achieve a balanced implementation of data minimization in their systems.

% We illustrate the privacy benefits of data minimization by conducting a comprehensive analysis across different classes of attacks. Additionally, we present several baseline algorithms for data minimization that also address the personalized nature of the problem. We specifically emphasize scenarios where our proposed methods effectively mitigate privacy risks. Through these examples, we demonstrate the value of incorporating data minimization into ML systems, not only to ensure legal compliance but also as a powerful tool to enhance the privacy and security of data-driven applications.

\paragraph{Contributions.} 
The paper's key contributions are,

\begin{itemize}
    \item We present a comprehensive framework to formalize the data minimization principle as an optimization problem, giving us a mathematical foundation for data minimization in ML. Our framework is capable of handling both existing minimization algorithms and novel personalized minimization techniques as introduced in this paper.
    \item We introduce multiple threat models with varying attacker objectives to measure the change in real-world privacy risks after data minimization in ML, bringing the focus to data privacy.
    \item We provide several data minimization algorithms based on existing literature in optimization, and study minimization trends like changing susceptibility to minimization across modalities and learning functions, emerging personalization through optimization, and the extent of alignment with real-world privacy risks.
    \item \textcolor{red}{We propose effective/simple defense mechanisms against the privacy attacks}
\end{itemize}

The results of this work are significant as they bridge the gap between the legal and technical domains, offering a robust and versatile solution to the data minimization challenges faced by ML practitioners. Our framework not only offers a solid groundwork for future research on data privacy and utility but also serves as a practical guide for developing privacy-preserving ML systems in accordance with legal requirements for a large landscape of data protection regulations.

==> archived_sections/cuong_sections/sec_metamodeling.tex <==
\subsection{Modeling Lower Optimization}
\label{sec:meta}
Gradient-based methods described above face two major issues, i.e., discretization error and the need for differential imputation methods. We now describe a metamodeling approach to bilevel optimization that can avoid both of these issues. The metamodeling approach relies on avoiding the lower optimization, but instead modeling it using a simpler learnable function. That is, we want to replace the loss calculation $\cL(\cX, \cY, \theta^*_{\cX \odot \cB})$ which relies on the lower level optimization for $\theta^*_{\cX \odot \cB}$, with a new function $m(\cB)$ that can directly estimate the loss value without solving for $\theta^*_{\cX \odot \cB}$.

\paragraph{Generating Input-Output Pairs: } We are going to learn the mapping between the minimization matrix $\cB$, and the loss value $\cL(\cX, \cY, \theta^*_{\cX \odot \cB})$. To do so, we first need to generate some matrix-loss pairs that will be vital to learning the mapping.

We start by generating a random minimization matrix $\cB$, with sparsity $s$. This is the same as performing personalized random subsampling as described earlier. We then solve the lower optimization for this $\cB$ and obtain the loss value. We repeat these steps multiple times to create a dataset to train $m(\cB)$. By using these input-output pairs, we can create a global approximation of the loss. One might even repeat this process multiple times during the overall optimization to create more accurate local approximations of the matrix-loss relationship.

\paragraph{Modeling $m(\cB)$: } To be able to learn an approximate mapping between the minimization matrix and the loss value, we make the following simplifying assumption.
\begin{itemize}
    \item \textit{Independent Influence: } We assume that the influence of any index $ij$ on the final loss value is independent of the rest of the minimization matrix. Thus, if we can quantify the influence of each index on the loss $\cI_{ij}$, we can aggregate it as:
    \begin{align}
        m(\cB) = \frac{1}{n d} \sum^n_{i=1} \sum^d_{j=1} \cI_{ij}
    \end{align}
\end{itemize}

Since each index in the dataset can only exist in two states, i.e., minimized or not minimized, we can simplify the influence of each index as,
\begin{align}
    \cI_{ij} =
    \begin{cases}
      \cI^1_{ij}, & \text{if}\ B_{ij}=1 \\
      \cI^{\phi}_{ij}, & \text{if}\ B_{ij}=\phi
    \end{cases}
\end{align}

Thus, we simply need to learn the parameters $\cI^1_{ij}, \cI^{\phi}_{ij}$ to complete the mapping $m(\cB)$. Given that we assume independent influence of each index on the minimization matrix, we can learn these parameters by calculating the average loss when $B_{ij}=1$ and $B_{ij}=\phi$, respectively.
\begin{align}
    \cI^1_{ij} = \frac{1}{|P^1|} \sum^{|P^1|}_{k=1} \cL(\cX, \cY, \theta^*_{\cX \odot P^1_k}) \quad \textrm{where} \quad P^1 := \{\cB \, | \, \cB_{ij}=1\} \\
    \cI^{\phi}_{ij} = \frac{1}{|P^{\phi}|} \sum^{|P^{\phi}|}_{k=1} \cL(\cX, \cY, \theta^*_{\cX \odot P^{\phi}_k}) \quad \textrm{where} \quad P^{\phi} := \{\cB \, | \, \cB_{ij}=\phi\}
\end{align}

\paragraph{Data Minimization: } After learning the parameters $\cI^1_{ij}, \cI^{\phi}_{ij}$, thus learning the modeling function $m(\cB)$, we can now simplify the original optimization as:
\begin{align}
    & \argmin_{\cB} ||\cB||_1 + \lambda*(m(\cB) - L_{c} - \alpha + t^2) \\
    \Rightarrow & \arg\min_{\cB} \sum^{n}_{i=1} \sum^{d}_{j=1} (1 + \lambda \cI^1_{ij})*\mathbbm{1}_{[\cB_{ij}=1]} + \lambda \cI^{\phi}_{ij}*\mathbbm{1}_{[\cB_{ij}=\phi]}
\end{align}
Clearly, the optimal minimization algorithm under the metamodeling assumptions is to minimize the indices with the highest values of $\cI^1_{ij} - \cI^{\phi}_{ij}$, until the desired level of sparsity.

==> archived_sections/cuong_sections/sec_related_work.tex <==
\section{Related work}

\subsection{The Data Minimization Principle in Literature}

In recent years, several studies have made attempts to formalize the data minimization principle within the field of machine learning. \citet{goldsteen2021data} propose a method of universal feature generalization aimed at reducing the granularity of information collected, while \citet{tran2023personalized} focus on personalized data minimization techniques, during the inference phase. For data minimization during training, \citet{shanmugam2022learning} leverage a scaling law of learning to determine the optimal point at which data collection should cease. \citet{biega2020operationalizing} also addresses personalized data minimization during training, with a specific emphasis on recommendation systems.

However, these works primarily evaluate the quality of data minimization based on the dataset size, and while some studies, such as \citet{goldsteen2021data}, also consider more advanced metrics like information loss, they remain indirect measures and fall short of addressing the issue of privacy leakage. This is where our work differentiates itself from previous research, as we specifically focus on the consideration of privacy leakage by introducing various adversarial attacks as a key component of the data minimization framework.

\subsection{Data Minimization Techniques}

Data minimization can be categorized into two distinct types: active and retrospective. Active data minimization revolves around the objective of collecting a minimal amount of new data. On the other hand, retrospective data minimization has access to all available data and focuses on retaining only the essential data, while dropping the rest. Achieving an optimal tradeoff between utility and privacy is a key consideration in both active and retrospective data minimization strategies.

The process of acquiring an optimal amount of new data represents a fundamental challenge within the domain of active learning \cite{burr2012active,ren2021survey}. Certain approaches, such as active feature-value acquisition (AFA) \cite{saar2009active, huang2018active,li2021active}, have been utilized to actively collect new data at the finest granularity, i.e., personalized to each individual data point. However, these methodologies typically depend on a cost matrix that governs the acquisition process of each feature. In the context of data minimization, creating an independent cost matrix for each feature value is impractical, as it necessitates careful consideration of its impact on the privacy and utility of the final trained model. Consequently, we propose a personalized data minimization algorithm within the context of active learning, where both utility and privacy serve as overarching objectives guiding the data collection process.

In the retrospective category, existing work on data condensation can be leveraged for data minimization purposes. Techniques such as data sampling, clustering, dimensionality reduction, and others can be employed to achieve this objective \cite{mitra2002density,reddy2020analysis}. Some approaches also integrate the generation of synthetic data as a mechanism for data condensation \cite{zhao2021dataset,zhao2023improved}. However, it is noteworthy that prevailing research in dataset condensation often fails to adequately address privacy considerations, and even the extent of privacy benefits offered by synthetic data generation remains ambiguous \cite{carlini2022no}. Furthermore, the majority of existing work in data condensation primarily concentrates on universal data minimization, i.e., the complete removal of specific features from all data points or the complete elimination of certain data points from the dataset. In contrast, our algorithms adopt a personalized approach, meticulously designed with data minimization principles, and we substantiate the privacy advantages of our methods.

\subsection{Privacy Auditing with Adversarial Attacks}

Privacy auditing often involves the application of adversarial attacks as a means to assess the privacy leakage of machine learning models. These attacks serve as powerful tools to expose potential vulnerabilities and by simulating realistic threat scenarios, such as membership inference attacks \cite{shokri2017membership}, re-identification attacks \cite{henriksen2016re}, attribute inference attacks \cite{yeom2018privacy,jayaraman2022attribute}, etc., auditors can evaluate the effectiveness of privacy protection mechanisms and identify areas where sensitive information may be unintentionally revealed. By leveraging adversarial attacks for privacy auditing of data minimization algorithms, we create a proactive framework to provide valuable insights into the privacy benefits as well as other ethical concerns associated with data minimization, enabling organizations and researchers to make informed decisions.


==> archived_sections/cuong_sections/sec_theoretical_proofs_baseline_old.tex <==
\subsection{Theoretical analysis of baseline models}

In this section, for notional convenience we respectively denote $\bm{\theta^*}$ and $\bm{\hat{\theta}}$ to be model parameters learned on complete and minimized data. We also denote $\bm{g}_i(\btheta) = \nabla_{\btheta} \ell(f_{\btheta}(x_i), y_i) $. Lastly, we assume that  the baseline \textbf{Random Subsampling} performs randomly select with replacement a subset $S$ of from $D$. 


% We have the following theorem regarding the difference in expectation between $\bm{\theta^*}$ and $\bm{\hat{\theta}}$. 


% \begin{theorem}

% Suppose the loss function $\ell(.)$ is convex w.r.t $\bm{\theta}$, and suppose we perform \textbf{Random Subsampling} with replacement of fraction $0< p\leq 1$.  Furthermore, if  we denote $G = \max_{\bm{\theta}} \| \nabla_{\theta} \cL(\cX, \cY, \bm{\theta}) \|_2$  then the following holds:

% \begin{align}
% \mathbf{E}[\| \bm{\theta^*} -\bm{\hat{\theta}}\|^2] \leq (1-p) G
% \end{align}

% \end{theorem}
% \begin{proof}

% Our proof relies on the following Lemma  \ref{app:lem:1}

% \begin{lemma}[\citet{opt_paper}]
% \label{app:lem:1}
% Let $\cL(\cX, \cY, \btheta )$ be a differentiable function w.r.t  $\btheta$. 
% Then $\cL(\cX, \cY, \btheta)$ is $\lambda$-strongly convex w.r.t  $\btheta$    \emph{iff} for all vectors
%  $\btheta, \btheta'$: 
% \begin{equation}
%     (\nabla_{\btheta}\cL (\cX, \cY, \btheta ) - \nabla_{\btheta'} \cL(\cX, \cY, \btheta ) )^T (\btheta - \btheta') \geq \lambda \| \btheta -\btheta' \|^2.
% \end{equation}
% \end{lemma}

% Note that by the assumption the individual loss $\ell(f_{\btheta}(x), y)$ is convex hence the total  $\cL(\cX, \cY, \btheta) = \sum^n_{i=1}\ell(f_{\btheta}(x_i), y_i) + \lambda \| \btheta\|^2_2 $ is $\lambda$-strongly convex.


% \end{proof}

We have the following statement regarding the necessary condition when $\bm{\theta^*} = \hat{\btheta}$.
\begin{theorem}
\label{thm:subsampling}
Suppose the loss $\ell(.)$ is convex w.r.t $\btheta$ and furtheremore at the optimal point, the gradient of loss at any individual input vanishes, i.e $g_{i}(\btheta^*) = \nabla_{\btheta} \ell(f_{\btheta^*}(x_i), y_i)= \bm{0}^T$ $\forall x_i$. Then the model parameter $\hat{\btheta}$ learned with minimized data obtained  obtained by \textbf{Random Subsampling} (no matter with or with not replacement)  is exactly the same as $\btheta^*$  

\end{theorem}


\begin{proof}

Denote $S \subset \cD $ to be a random subset of $m << n$ training samples. By the assumption that the individual loss $\ell(.)$ is convex w.r.t $\btheta$ $\forall x_i$ then the following loss  function  is also convex:

$$ \hat{\cL}(\btheta) = \sum_{ (x_i,y_i) \in S} \ell(f_{\btheta}(x_i), y_i) $$.

Hence there is one single global minima that minimizes the loss $\hat{\cL}$ of the minimized data. Furthermore, by the assumption that $\nabla_{\btheta} \ell(f_{\btheta^*}(x_i), y_i)= \bm{0}^T$ $\forall x_i$, hence:

$$ \nabla_{\btheta^*} \hat{\cL}(\btheta) = \bm{0}^T$$

Hence $\btheta^*$ is also  the global minima of $\hat{\cL}$ which implies $\btheta^* = \hat{\btheta}$
\end{proof}
We provide the following example in which the assumption in Theorem \ref{thm:subsampling} holds.
\begin{example}
\label{ex:1}
Consider the linear regression task with the MSE loss $\ell(f_{\btheta}(x_i), y_i) = (\btheta^T x_i -y_i)^2$. Suppose there exists a parameter $\btheta^*$ such that  $y_i = \btheta^{*^{T}} x_i $, i.e, the groundtruth is a linear combination of input features.  Then using the \textbf{Random Subsampling} method we are guaranteed to retain the model parameter $\btheta^{*}$ learned on complete data.
\end{example}
We can see clearly that the example  \ref{ex:1} satisfies the conditions in Theorem \ref{thm:subsampling}. First of all, the MSE loss for linear regression is convex. Second the individual gradient  $\nabla_{\btheta} \ell(f_{\btheta^*}(x_i),y_i) = (y_i - \btheta^{*^T} x_i) x_i = \bm{0}^T$ by the assumption the groundtruth is a linear combination of input features. 


Furthermore we have the following statement regarding the  upper bound over the expected  $\mathbf{E}[ \| \btheta^* - \hat{\btheta}\|]$

\begin{theorem}
\label{thm:sampling_bound}
Suppose the loss function $\ell(f_{\btheta}(x_i), y_i)$ is convex  w.r.t $\btheta, \forall x_i$. If we denote $\Sigma$ to be the empirical covariance matrix of the set of deterministic vector $\{ g_i(\btheta^*) \}^n_{i=1}$  then the following holds:

\begin{align}
\mathbf{E}[\| \btheta^* - \hat{\btheta}\| ] \leq \frac{2 \text{Trace}(\Sigma)}{\lambda |S|} 
\end{align}
\end{theorem}

\textcolor{Theorem \ref{thm:sampling_bound} derives the upper bound on the difference between model parameters learned on minimized and complete data. It suggest the more number of training samples you can draw in \textbf{Random Subsampling} the smaller the difference. }

Our proof relies on the following classical theorem in statistis \cite{moore2009introduction}
\begin{lemma}
\label{lem:variance}

Consider a set of deterministic vector $\{ g_1(\btheta), ..,g_n(\btheta)\}^n_{i=1}$ with sample covariance variance $\Sigma$. If $S = \{ i | i \overset{\mathrm{iid}}{\sim} [n] \}$ then 

$$ \text{Trace}\left[Var[\frac{1}{|S|}\sum_{i \in S} g_i(\btheta)] \right] = \frac{\text{Trace}(\Sigma)}{|S|}$$
\end{lemma}


The Lemma \ref{lem:variance} implies that the more number of draw samples (i.e $|S|$ large) the smaller the  variance of sample mean.  

\begin{proof}
By the assumption that the individual loss $\ell(f_{\btheta}(x_i), y_i)$ is convex w.r.t $\btheta$ for all $x_i$, then the following empirical risk on minimized data is $\lambda$-strongly  convex:

\begin{align}
\hat{L}(\btheta) = \sum_{i\in S} \ell(f_{\btheta}(x_i), y_i) + \lambda \| \btheta\|^2_2. 
\end{align}
By the propery of strongly convex function it follows that:

\begin{align}
  ( \nabla_{\btheta} \hat{L}(\hat{\btheta}) -  \nabla_{\btheta} \hat{L}(\btheta^*)  )^T (\hat{\btheta} -\btheta^*)  \geq \frac{\lambda}{2} \| \hat{\btheta} - \btheta^* \|^2_2
\label{eq:diff}
\end{align}

Since $\hat{\btheta} = \text{argmin}_{\btheta} \hat{L}(\btheta)$ hence $\nabla_{\btheta}\hat{L}(\hat{\btheta}) = \bm{0}^T $. Thus the L.H.S of Equation \ref{eq:diff} can be reduced to $-\nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  $ 

Taking the expectation on both sides we obtain:

\begin{equation} \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right]\geq \frac{\lambda}{2} \mathbf{E}\left[ \| \hat{\btheta} -\btheta^*\|^2_2 \right]
\label{eq:1}
\end{equation}


Apply the Cauchy-Schwarz inequality for expectation, i.e  for any two random variables $X$ and $Y$ then $| \mathbf{E}[X^TY] | \leq  \sqrt{\mathbf{E}[X^TX]  \mathbf{E}[Y^TY] } $ it follows that:


\begin{align} \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right]& \leq \left| \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right] \right| \\
& \leq \sqrt{ \mathbf{E}[ \|  \nabla_{\btheta} \hat{L}(\btheta^*) \|^2_2] \mathbf{E}[ \| \hat{\btheta} -\btheta^*\|^2_2] } \\
& =  \sqrt{ \mathbf{E}[ \|  \nabla_{\btheta} \hat{L}(\btheta^*) \|^2_2] }  \sqrt{ \mathbf{E}[ \| \hat{\btheta} -\btheta^*\|^2_2}
\label{eq:2}
\end{align}

Combine Equation \ref{eq:1} and Equation \ref{eq:2} we obtain:
\begin{equation}
 \mathbf{E}\left[ \|   \nabla_{\btheta} \hat{L}(\btheta^*)\|^2_2 \right] \geq \frac{\lambda}{2} \mathbf{E}\left[ \| \hat{\btheta} -\btheta^* \|^2_2 \right] 
\label{eq:3}
\end{equation}
\newcommand{\indep}{\perp \!\!\! \perp}

By the following property  for any random variable $X$  if $X_i \indep X_j $ for $X_i, X_j$ are two arbitrary entries of $X$   then $\mathbf{E}[ ||X||^2_2 ] = (E[X])^T E[X] + \text{Trace}[Var[X]]$. Furthermore, 

$$ \mathbf{E}[  \nabla_{\btheta} \hat{L}(\btheta^*)] =\mathbf{E}[\sum_{i \in S} g_i(\btheta^*) ] = \sum_{i \in S} \mathbf{E}[ g_i(\btheta^*) ]  = \bm{0}^T$$

The last equation comes from the fact that $g_{i}(\btheta)$ is drawn from a set of $\{  g_i(\btheta^*) \}^n_{i=1}$ whose the mean is a zero vector. 

Thus:

\begin{align}  \mathbf{E}\left[ \|   \nabla_{\btheta} \hat{L}(\btheta^*)\|^2_2 \right] & = \bm{0}^T + \text{Trace}( Var[\nabla_{\btheta} \hat{L}(\btheta^*)]) = \frac{\text{Trace}(\Sigma)}{|S|}\\
& \geq \frac{\lambda}{2} \| \hat{\btheta} -\btheta^* \|^2_2
\end{align}







\end{proof}


==> archived_sections/inputs.tex <==
\usepackage{todonotes}
\usepackage{xcolor}
\usepackage{setspace}
\usepackage{multirow}
\usepackage{paralist}
\usepackage{booktabs} 
%\usepackage{enumitem}
\newtheorem{prop}{Proposition}
\newcommand{\Lap}{\textrm{Lap}}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand*{\prob}{\mathsf{P}}


\usepackage{amsmath}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{url}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{newfloat}
\usepackage{listings}
\DeclareCaptionStyle{ruled}{labelfont=normalfont,labelsep=colon,strut=off} % DO NOT CHANGE THIS
\lstset{%
	basicstyle={\footnotesize\ttfamily},% footnotesize acceptable for monospace
	numbers=left,numberstyle=\footnotesize,xleftmargin=2em,% show line numbers, remove this entire line if you don't want the numbers.
	aboveskip=0pt,belowskip=0pt,%
	showstringspaces=false,tabsize=2,breaklines=true}
\floatstyle{ruled}
\newfloat{listing}{tb}{lst}{}
\floatname{listing}{Listing}

%%% Comments
\newcommand{\nandoSide}[1]{\todo[caption={},color=cyan!20!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\tiny FF: #1}
\vspace{-8pt}
\end{spacing}}}
\newcommand{\pascalSide}[1]{\todo[caption={},color=green!20!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\tiny PVH: #1}
\vspace{-8pt}
\end{spacing}}}
\newcommand{\cuongSide}[1]{\todo[caption={},color=red!20!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\tiny CT: #1}
\vspace{-8pt}
\end{spacing}}}
\newcommand{\nando}[1]{\todo[inline,caption={},color=cyan!20!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\footnotesize FF: #1}
\vspace{-8pt}
\end{spacing}}}
\newcommand{\cuong}[1]{\textbf{Cuong}:{\color{red}{#1}}}
\definecolor{darkgreen}{RGB}{204,102,0}

\newcommand{\JE}[1]{\todo[inline,caption={},color=blue!10!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\footnotesize JEK: #1}
\vspace{-8pt}
\end{spacing}}}

\newcommand{\JESide}[1]{\todo[caption={},color=purple!50!]{
\begin{spacing}{0.6}
\vspace{-2pt}
{\tiny JEK: #1}
\vspace{-8pt}
\end{spacing}}}



\newcommand{\revSide}[2]{{\color{purple}{#1}}{\todo[caption={},color=purple!20!]{
\begin{spacing}{0.625}{\footnotesize #2}\end{spacing}}}}

\newcommand{\rev}[1]{{\color{purple}{#1}}
	\todo[caption={},color=purple!20!]
		{\begin{spacing}{0.625}
			{\footnotesize to review}
		\end{spacing}}
	}

\newcommand{\add}[1]{{\color{darkgreen}{#1}}}
\newcommand*{\defeq}{\stackrel{\text{def}}{=}}
\def\aux{\mathrm{aux}}

% Math-cal
\newcommand{\cA}{\mathcal{A}} \newcommand{\cB}{\mathcal{B}} 
\newcommand{\cC}{\mathcal{C}} \newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}} \newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}} \newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}} \newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}} \newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}} \newcommand{\cP}{\mathcal{P}}
\newcommand{\cR}{\mathcal{R}} \newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}} \newcommand{\cV}{\mathcal{V}}
\newcommand{\cZ}{\mathcal{Z}} \newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}} \newcommand{\cY}{\mathcal{Y}}
\newcommand{\cW}{\mathcal{W}} \newcommand{\cX}{\mathcal{X}}

\newcommand{\EE}{\mathbb{E}} \newcommand{\RR}{\mathbb{R}}
\newcommand{\NN}{\mathbb{N}} \newcommand{\ZZ}{{\mathbb{Z}}}
\newcommand{\CC}{{\mathbb{C}}}
\newcommand{\btheta}{{\bm{\theta}}}

%%% helpers
\newcommand{\MLap}{\mathcal{M}_{\mathrm{Lap}}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{Cov}}

\newcommand{\minimize}[1]{\underset{{#1}}{\text{minimize}}}
\newcommand{\maximize}[1]{\underset{{#1}}{\text{maximize}}}
% \newcommand{\st}{\text{subject to}}
\newcommand{\setcard}[1]{\scalebox{0.5}{$|#1|$}}
% \usepackage{mathtools}
\newcommand\norm[1]{\left\lVert#1\right\rVert}
\usepackage{esvect}\newcommand{\cev}[1]{\reflectbox{\ensuremath{\vec{\reflectbox{\ensuremath{#1}}}}}}
\DeclareMathOperator{\Tr}{Tr}
\newcommand{\se}[1]{\text{s}(#1)}
\newcommand{\re}[1]{\text{r}(#1)}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\newcommand{\smallk}{\scalebox{0.65}{$k$}}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\nint}\lfloor\rceil
% make optimal notation
\makeatletter
\newcommand{\oset}[3][0ex]{\mathrel{\mathop{#3}\limits^{\vbox to#1{\kern-2\ex@\hbox{$\scriptstyle#2$}\vss}}}}
\makeatother
\newcommand{\optimal}[1]{\oset{\scalebox{.5}{$\star$}}{#1}}
\newcommand{\loss}{{\scriptstyle\Delta}}
% rescale vdots and ddots for small matrix 
\usepackage{letltxmacro}
\LetLtxMacro\orgvdots\vdots
\LetLtxMacro\orgddots\ddots
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%



==> archived_sections/notes.tex <==
\section{Notes on Data minimization solving}

Let's assume we have a binary logistic regression problem with a dataset consisting of $n$ samples and $m$ features. Let $\mathbf{X}$ be the feature matrix ($n \times m$), $\mathbf{y}$ be the target vector ($n \times 1$), and $\mathbf{w}$ be the weight vector ($m \times 1$). We'll also use a regularization parameter $\lambda$ (from the upper-level problem) for L2 regularization.

\paragraph{Upper-level problem (ULP)}: 
Minimize the dataset size:
\begin{equation}
\begin{aligned}
& \min_{\mathbf{B}} \; \sum_{i=1}^{n} \sum_{j=1}^{m} b_{ij} \\
& \text{subject to } \; b_{ij} \in \{0, 1\}, \; \forall i = 1, \ldots, n, \; \forall j = 1, \ldots, m
\end{aligned}
\end{equation}


\paragraph{Lower-level problem (LLP)}: 
Logistic regression with sparse feature matrix $\mathbf{B} \mathbf{X}$
\begin{equation}
    \min_{\mathbf{w}} L(\mathbf{w}) = \sum_{i=1}^n \left[ -y_i \log(p_i) - (1 - y_i) \log(1 - p_i) \right] + \frac{\lambda}{2} \lVert \mathbf{w} \rVert^2 \\
\end{equation}



where $p_i = \frac{1}{1 + \exp(-(\mathbf{B}\mathbf{X})_i \mathbf{w})}$ is the predicted probability for the i-th sample.

To apply KKT conditions, we first need to introduce inequality constraints. We can do this by reformulating the L2 regularization term using non-negative auxiliary variables, say $\mathbf{z}$ ($m \times 1$). Let's rewrite the regularization term as follows:

\begin{equation}
\frac{\lambda}{2} \lVert \mathbf{w} \rVert^2 = \frac{\lambda}{2} \sum_{j=1}^m w_j^2 = \frac{\lambda}{2} \sum_{j=1}^m \left(z_j^2 - z_j^2 + w_j^2\right) = \frac{\lambda}{2} \sum_{j=1}^m (z_j - w_j)(z_j + w_j)
\end{equation}

Now, the optimization problem becomes:


\begin{equation}
\begin{aligned}
\min_{\mathbf{w},\mathbf{z}} L(\mathbf{w}, \mathbf{z}) = 
    &\; \sum_{i=1}^n \left[ -y_i \log(p_i) - (1 - y_i) \log(1 - p_i) \right] + \frac{\lambda}{2} \sum_{j=1}^m (z_j - w_j)(z_j + w_j) \\
\text{subject to } 
    &\; z_j - w_j \geq 0, \; z_j + w_j \geq 0, \; \forall j = 1, \ldots, m
\end{aligned}
\end{equation}

\paragraph{KKT conditions}

\begin{enumerate}
    \item 
    Stationarity:
    \begin{equation}
    \begin{aligned}
    & \nabla_{\mathbf{w}} L(\mathbf{w}, \mathbf{z}) = 0 \\
    & \nabla_{\mathbf{z}} L(\mathbf{w}, \mathbf{z}) = 0
    \end{aligned}
    \end{equation}
    
    \item 
    Primal feasibility:
    \begin{equation}
    z_j - w_j \geq 0, \; z_j + w_j \geq 0, \; \
    \forall j = 1, \ldots, m
    \end{equation}
    
    \item 
    Dual feasibility:
    \begin{equation}
    \mu_j (z_j - w_j) = 0 \; \text{and} \; \nu_j (z_j + w_j) = 0, \; \forall j = 1, \ldots, m
    \end{equation}
    where $\mu_j$ and $\nu_j$ are the Lagrange multipliers for the inequality constraints.
    
    \item 
    Complementary slackness:
    \begin{equation}
    \mu_j \geq 0, \; \nu_j \geq 0, \; \forall j = 1, \ldots, m
    \end{equation}
    \end{enumerate}


\paragraph{Solving the lower-level problem}

\begin{enumerate}
    \item Calculate the gradients of the objective function with respect to $\mathbf{w}$ and $\mathbf{z}$. To do this, we can use the chain rule:
    \begin{equation}
    \begin{aligned}
    \frac{\partial L}{\partial w_j} &= -\sum_{i=1}^n \left[ y_i \frac{\partial \log(p_i)}{\partial w_j} + (1 - y_i) \frac{\partial \log(1 - p_i)}{\partial w_j} \right] + \lambda(z_j - w_j) - \lambda(z_j + w_j) \\
    \frac{\partial L}{\partial z_j} &= \lambda(z_j - w_j) + \lambda(z_j + w_j)
    \end{aligned}
    \end{equation}
    
    \item
    Set the gradients to zero to get the stationarity conditions:
    \begin{equation}
    \begin{aligned}
    \frac{\partial L}{\partial w_j} &= 0 \\
    \frac{\partial L}{\partial z_j} &= 0
    \end{aligned}
    \end{equation}
    
    \item 
    Solve the resulting system of nonlinear equations for $\mathbf{w}$, $\mathbf{z}$, $\boldsymbol{\mu}$, and $\boldsymbol{\nu}$ (either using numerical methods -- interior points, Newton's method) or exploiting the specific structure of the problem.
    
    \item 
    Check the primal feasibility, dual feasibility, and complementary slackness conditions. 
\end{enumerate} 


\paragraph{Alternative single-level problem}

\begin{equation}
\begin{aligned}
& \min_{\mathbf{w}, \mathbf{B}} \sum_{i=1}^n \left[ -y_i \log(p_i) - (1 - y_i) \log(1 - p_i) \right] + \frac{\lambda}{2} \lVert \mathbf{w} \rVert^2 + \gamma \sum_{i=1}^{n} \sum_{j=1}^{m} b_{ij} \\
& \text{subject to } \; 0 \leq b_{ij} \leq 1, \; \forall i = 1, \ldots, n, \; \forall j = 1, \ldots, m \\
& \text{and } p_i = \frac{1}{1 + \exp(-(\mathbf{B}\mathbf{X})_i \mathbf{w})}
\end{aligned}
\end{equation}

In this formulation, the regularization term $\gamma \sum_{i=1}^{n} \sum_{j=1}^{m} b_{ij}$ encourages sparsity in matrix $\mathbf{B}$, while the continuous constraint $0 \leq b_{ij} \leq 1$ replaces the original binary constraint. The parameter $\gamma$ controls the trade-off between the sparsity of $\mathbf{B}$ and the logistic regression problem's fit.


==> archived_sections/sec_algorithms.tex <==
% \subsection{Our proposed optimization framework}

% \paragraph{Challenges with constraints} The two constraints in the previous section is not differentiable. We proposed the following proxy constraint that are fully differentiable. 

% First, w.r.t to the constraint in Equation \ref{eq:capacity}, we can use $l_1$ norm to promote sparisity, or the following dead-zone proxy function:

% $$DZ(b) = \begin{cases}
%         |b| - \frac{\alpha}{2}, \ \text{ if $|b| \geq \frac{\alpha}{2} $ }
%         \\
%         | 1- b| -\frac{\alpha}{2},\ \text{if  $|b| < \frac{\alpha}{2} $  }.
%         \end{cases} $$


% Second, for the privacy constraint (actually a counting constraint) in Equation \ref{eq:privacy_constraint}, we replace $\mathbf{1}[\Delta( x_i \cdot B_i; x_j \cdot B_j) \geq \delta]$ by the following:

% $$\max( \delta - \Delta( x_i \cdot B_i; x_j \cdot B_j), 0) \frac{1}{\delta} $$.

% Overall, our objective function can be rewritten as the following: 

% \begin{align}
% \min_{\bm{B^*}, \theta}  & \sum^n_{i=1} \ell\bigg(f_{\theta}(x_i \cdot B^*_i), y_i\bigg) + \lambda_s \sum^n_{i=1} \sum^d_{j=1} DZ(B_{i,j}) \\
% & + \lambda_p \sum^{n}_{i=1}\sum^n_{j \neq i}  \max( \delta - \Delta( x_i \cdot B_i; x_j \cdot B_j), 0) \frac{1}{\delta}
% \end{align}
















==> archived_sections/sec_algorithms_archived.tex <==
Having defined a bilevel optimization model, we will now discuss how to operationalize data minimization. This section first reviews three strong baselines that can be readily used as proxies to achieve some form of data minimization. Although these baselines fail to comply with the legal requirements of data minimization (either because they disregard its purpose or the data relevance principles), they provide bounds on the model quality degradation during data minimization and thus serve as excellent baselines for our evaluations (see Appendix \ref{sec:app_baseline} for more details). Next, we will introduce three classes of algorithms, adapted from the bi-level optimization literature, that will be used to solve the data minimization problem as posed in \eqref{eq:dm_goal}.

Before diving into the discussion of the algorithms, we notice that, although the data minimization principle is designed to optimize the dataset size while retaining the quality of the resulting model (see Constraint \ref{eq:fidelity}), many algorithms work on a dual view that instead optimizes for model quality when trained on the minimized data under a given sparsity constraints $\|\bm{B}\|_1 \leq k$. Such algorithms can then search for a sparsity parameter $k$ that satisfies the desired $\alpha$-drop in performance, relating back to the original constraints in \eqref{eq:dm_goal}.
% \iffalse 
% However, before we dive deeper, we note that most algorithms in the literature are designed for a different formulation than the one defined in \eqref{eq:dm_goal}. In particular, rather than optimizing for auxiliary constraints while maintaining model quality, existing algorithms in bi-level optimization instead optimize for model quality under given auxiliary constraints (in our case, the dataset size)~\cite{chen2022gradient}. Therefore, we rewrite the original optimization problem as:
% \begin{subequations}
% \label{eq:dm_dual_goal}
%     \begin{align}
%         \minimize_{\bm{B} \in \{\bot, 1\}^{n \times p}} \;\;
%             & J(\mhlgreen{\hat{\theta}}; \bX, \bY)
%             \label{eq:data_relevance_dual}\\
%         \textsl{s.t.}:\;\; 
%             & \mhlblue{\| \bm{B} \|_1} \leq k
%             \label{eq:fidelity_dual}
%             \\\;\;
%             & \mhlgreen{\hat{\theta} = 
%                 \argmin_\theta \frac{1}{n} \sum_{i=1}^n 
%                 \ell\left(f_\theta( \mhlblue{\bm{x}_i \odot \bm{B}_i}, y_i\right)}
%                 \label{eq:purpose_limitation_dual}
%     \end{align}
% \end{subequations}
% where $k$ is the size constraint over $\bm{B}$. We can still solve the original optimization in \eqref{eq:dm_goal}, i.e., find the smallest dataset size that maintains model quality above a threshold, by instead searching through the solutions of this optimization problem in \eqref{eq:dm_dual_goal} under changing size constraints. We will stick with this formulation for the rest of the paper, to measure and compare the utility and privacy of the minimized dataset across different size constraints.
% \fi 

\subsection{Baseline Algorithms}
This section reviews feature selection, random subsampling, and individualized random subsampling, as three strong baselines for data minimization purposes. These baselines are depicted pictorially in Figure \ref{fig:datamin}. 
% Although these methods do not comply with the legal principles of data minimization, they provide bounds on the model quality degradation during data minimization and can thus serve as excellent baselines for our evaluations (\rev{see Appendix \ref{sec:app_baseline} for more details}).

% \begin{figure}[!t]
\begin{wrapfigure}{r}{0.6\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{images/baselines.pdf}
    \caption{Baselines algorithm for data minimization. While they violate the legal requirements, they can help us give context to our evaluations.}
    \label{fig:datamin}
\end{wrapfigure}
% \end{figure}

\smallskip\noindent\textbf{Feature Selection ~\cite{blum1997selection}.} 
Feature selection is a breadth-based minimization strategy that retains only the most important features in the data. The algorithm works by first sorting the features of the dataset in order of their importance,  using a pre-established criterion, to identify a subset $S$ of the least important features. The minimized dataset $\bX'$ is formed from $\bX$ by removing all features in $S$. 
In our paper, the importance criterion is the absolute correlation between each feature and the output label, and the algorithm sets:
\begin{equation}
    \bm{B}_{ij} = \bot \quad \forall i \in [n], j \in  S
\end{equation}
where $|S|$ is a parameter controlling the minimization sparsity.

\smallskip\noindent\textbf{Random Subsampling.} 
Random subsampling is a depth-based minimization strategy that randomly chooses a subset of data points from the original dataset. In the context of data minimization, it sets the minimization matrix $\bm{B}$ as:
\begin{align}
    \bm{B}_{ij} = \bot \quad \forall j \in [p], \textrm{ with probability }\; k_p,
\end{align}
where $0 \leq k_p \leq 1$ is a probability value chosen so that $nk_p$ rows of the dataset $D$ are minimized, in expectation. 
%Here $U \in \{0, 1\}^{n}$ is a randomly permuted binary vector, with exactly $s$ indices filled with $1$, i.e., $\Sigma_{i} U_{i} = s$, to control the desired sparsity of the minimization matrix.

\smallskip\noindent\textbf{Individualized Random Subsampling.} 
Individualized random subsampling is an extension of random subsampling, but it removes individual entries (feature, sample) rather than complete rows, i.e., it performs individualized minimization. 
% The method works by randomly selecting a subset $S \in \{ (i,j) | i \in [n], j \in [p]  \} $ and removing all features in this set. The methods minimization matrix is:
The minimization matrix $\bm{B}$ is defined as:
\begin{align}
    \bm{B}_{ij} = \bot \quad \textrm{ with probability }\; k_p,
\end{align}
where $0 \leq k_p \leq 1$ is chosen so that $npk_p$ elements of the dataset $D$ are minimized, in expectation. 

% \begin{equation}
%     \bm{B}_{ij} = \bot \, \text{if}\, (i,j) \in S,
% \end{equation}

% where $|S|$ is a parameter controlling the minimization sparsity.

% where $0 \leq k_p \leq 1$ is a value chosen so that $k$ elements of the original dataset $D$ are minimized, in expectation. 
%Here $U^P \in \{0, 1\}^{n \times p}$ is a randomly permuted binary matrix, with exactly $s$ indices filled with $1$, i.e., $\Sigma_{ij} U^P_{ij} = s$, to control the desired sparsity of the minimization matrix.

\subsection{Data Minimization Algorithms}
\label{sec:data_min_alg}
We will now introduce three classes of algorithms to solve the data minimization optimization posed in ~\eqref{eq:dm_goal}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\smallskip\noindent\textbf{Approximating the Lower Level Program \cite{6079692}.}
\label{sec:taylor_approximation}
Solving the bi-level optimization discussed in the previous section is challenging due to the nested structure of the problem which requires solving a non-convex lower-level optimization within a non-convex upper-level optimization.
When the lower-level problem has a unique solution that can be explicitly expressed in a closed form, then the overall bilevel program can be rewritten as a single-level program which is much simpler to solve. Under the assumption that the minimized dataset $\bX' = \bX \odot \bm{B}$ is similar enough to the original dataset $\bX$, the target utility can be approximated, while ignoring second-order or higher terms in the Taylor expansion, as:
% One way to overcome this challenge is to bypass the dependence of the upper-level utility $J(\hat{\theta}; \bX, \bY)$ on the lower-level optimization output $\hat{\theta}$. We can achieve this approximation by using the taylor expansion of the target utility. Under the assumption of the minimized dataset $\bX'$ being similar enough to the original dataset $\bX$ that we can ignore second-order or higher terms, we can rewrite the target utility as:
\begin{align}
    J(\hat{\theta}; \bX, \bY) \approx J(\optimal{\theta}; \bX, \bY) + (\bX -\bX')^T L H^{-1} G
\end{align}
where $L, H, G$ are the gradients w.r.t.~the model's parameters, the Hessian w.r.t.~the model's parameters, and the second-order derivative w.r.t.~the model's parameters and the dataset, respectively, of the original utility on the complete dataset $J(\optimal{\theta}; \bX, \bY)$. This simplifies the original optimization as:%\eqref{eq:dm_dual_goal} as follows:
% \begin{subequations}
\begin{equation}
\label{eq:integer_program}
    % \begin{align}
    \minimize_{\bm{B} \in \{\bot, 1\}^{n \times p}} \;\;
    \| \bm{B} \|_1 \quad \quad
        \textsl{s.t.}:
        \;\; (\bX-\bX')^T L H^{-1} G \leq \alpha.
    % \end{align}
\end{equation}
% \end{subequations}
% \begin{subequations}
% \label{eq:integer_program}
%     \begin{align}
%     \minimize_{\bm{B} \in \{\bot, 1\}^{n \times p}} \;\; & (\bX'-\bX)^T L H^{-1} G \\
%         \textsl{s.t.}:\;\; 
%             & \| \bm{B} \|_1 \leq k
%     \end{align}
% \end{subequations}
Recall again that it is often convenient to view the optimization expressed in \eqref{eq:dm_goal} as a program that minimizes the loss $J(\hat{\theta}; \mathbf{X}, \mathbf{Y})$ under sparsity constraint over the minimization matrix $\bm{B}$. Under this view, and assuming a zero-imputation data preprocessing, i.e., replacing the missing values with zero as $\bX' = [\bX \odot \bm{B}]_{\bot \rightarrow 0}$, the above optimization problem simplifies into integer linear programming. The solution to this linear programming for a target sparsity $\|\bm{B}\|_1 \leq k$ is simply setting $\bm{B}_{ij} = 1$ for the $k$ largest entries of the matrix $( \bX_{ij} -\bX'_{ij} )\odot (L H^{-1} G)_{ij}$, and $\bm{B}_{ij} = \bot$ otherwise. Additional discussions on the algorithm's assumptions and the derivation are presented in Appendix \ref{sec:app_algorithms}.

% This approximation is a useful and efficient tool for minimization, especially in simple settings, but it may be inaccurate when the underlying assumptions are not met. For instance, when the minimized dataset is required to be highly sparse, it is likely no longer close to the original dataset, undermining the methods' assumptions. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\smallskip\noindent\textbf{Modeling the Target Utility \cite{wang2006review}.}
Instead of relying on the assumptions of low sparsity to approximate the target utility as above, we can take a more general approach by directly modelling and learning the mapping between the target utility and the minimized dataset. In other words, we want to learn a parametrized function $m_\omega(\bm{B}) \approx J(\hat{\theta}; \bX, \bY)$, where $\omega$ is a vector of parameters, to estimate the target utility without solving the lower-level optimization for $\hat{\theta}$.

To learn a tractable mapping $m_\omega(\bm{B})$, we restrict ourselves to linear functions of $\bm{B}$ and assume that each index of the dataset has an independent influence on the target utility. Therefore, if we quantify the influence of each index on the target utility as $\cI_{ij}$, the mapping $m_\omega(\bm{B})$ becomes:
\begin{equation}
    J(\hat{\theta}; \bX, \bY) \approx m_\omega(\bm{B}) = \frac{1}{n p} \sum^n_{i=1} \sum^p_{j=1} \cI_{ij}.
\end{equation} 
Here $\cI_{ij}$ can only exist in one of two binary states, i.e., $\cI_{ij} = \mathbbm{1}_{[\bm{B}_{ij}=1]} \cdot \cI^1_{ij} + \mathbbm{1}_{[\bm{B}_{ij}=\bot]} \cdot \cI^{\bot}_{ij}$. To learn the values of $\cI^1_{ij}$ and $\cI^{\bot}_{ij}$, we generate a large number of minimization matrix-target utility pairs by solving the lower-level optimization for each pair. We can then learn these parameters for each index ${ij}$ by averaging the target utility when $\bm{B}_{ij}=1$ and $\bot$, respectively. The final optimization thus becomes:%in \eqref{eq:dm_dual_goal} can thus be rewritten as:
% \begin{subequations}
\begin{equation}
\label{eq:metamodel}
    % \begin{align}
    \minimize_{\bm{B} \in \{\bot, 1\}^{n \times p}} \;\; 
    \| \bm{B} \|_1 \quad \quad
        \textsl{s.t.}:
        \;\; \frac{1}{n p} \sum^n_{i=1} \sum^p_{j=1} \cI_{ij} - J(\optimal{\theta}; \bX, \bY) \leq \alpha.
    % \end{align}
\end{equation}
% \end{subequations}
When considering a sparsity constraint $\|\bm{B}\|_1 \leq k$ on the minimization matrix, the solution to this formulation is retaining the $k$ entries with the highest value of the term $\cI^{\bot}_{ij} - \cI^1_{ij}$. Although the assumption 
of independent influence may not hold in all cases, %due to highly correlated input features in the dataset, 
our results (illustrated in the next section) show that this approach can substantially improve the accuracy of existing baselines. 
%the overall method of modeling the target utility can be improved in the future by using better modeling techniques to handle more complex settings.
More details on learning the mapping $m_\omega(\bm{B})$ are present in Appendix \ref{sec:app_algorithms}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\smallskip\noindent\textbf{Evolutionary Algorithms \cite{sinha2014finding}.}
So far, we have discussed methods that approximate the original optimization problem under various assumptions, enabling us to solve it more easily. An orthogonal class of algorithms, often applied to solve bi-level programs, are evolutionary algorithms. They trade the advantage of carrying no assumption with slow convergence, i.e., high computational demand, and higher risks of overfitting. %, while their either at the upper-level optimization or at both levels simultaneously. 
% In our context, we will use them for upper-level optimization only.

In our implementation of the evolutionary algorithm, we begin with a population of randomly generated minimization matrices $\bm{B}$ and then evolve them across iterations to reach our objective. We mutate and breed the current population at each stage of the process to create a larger pool of choices and carry out the lower-level optimization for every member of this pool, only retaining the best performers for the next generation. The entire process is repeated until convergence, or for a fixed number of iterations. Additional details are provided in Appendix \ref{sec:app_algorithms}.
%Evolutionary algorithms offer an advantage in that they are not constrained by any underlying assumptions and can even provide guarantees of convergence with enough iterations. However, to achieve convergence in a practical scenario, one needs to run several iterations with a large active population size. This can create a significant computational demand in comparison to other approximate methods we saw above.

==> archived_sections/sec_app_algorithms.tex <==
\subsection{Taylor Approximation of Target Utility}
\label{sec:taylor_approximation}

The difficulty of solving the main optimization in Section \ref{sec:data_minimization} lies on the equality constraint in Equation \ref{eq:eq_constraint} and the binary constraint over $\cB$ in Equation \ref{eq:capacity_constraint}. Our first proposed method called Taylor approx which relies on approximating directly the target utility $\cL(\cX, \cY, \bm{\theta^{*}}_{\cX \odot \cB} )$  by the original utility by the following Lemma \ref{lem:taylor}


\begin{lemma}
The target utility  of interest $\cL(\cX, \cY, \bm{\theta^{*}}_{\cX \odot \cB} )$ can be aproximated by the original utility $\cL(\cX, \cY, \bm{\theta^{*}}_{\cX} )$  as follows:

$$ \cL(\cX, \cY, \bm{\theta^{*}}_{\cX'} ) \approx \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) + (X'-X)^T L H^{-1} G + \cO\big( \| X'-X\|^2\big)$$,
where:

$$ L =\frac{\partial \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta}}  \,\, \text{(1st derivative w.r.t param )}$$


$$ H =\frac{\partial^2 \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta}^2} \, \, \mbox{ (Hessian matrix of param) } $$

$$G = \frac{\partial^2 \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta} \partial \cX} \, \, \mbox{ (2nd derivative w.r.t param and input) }$$
\label{lem:taylor}
\end{lemma}


Proof of Lemam \ref{lem:taylor} is base on  the combination of the first order Taylor approximation of the function $ \cL(\cX, \cY, \bm{\theta^{*}}_{\cX'} )$ around original data $\cX$ and the chain rule law. It is noted that the matrix multiplication $L H^{-1} G$ is a constant w.r.t $\cB$ and we can put  $S =L H^{-1} G  \in R^{n\times d}$. Given Lemma \ref{lem:taylor}, and suppose the term $O\big(\|X'-X\|^2 \big)$ is negligible, then the main optimization in Section \ref{sec:data_minimization}  can be simply reduced to the following integer linear programming:

\begin{align}
\min_{\cB} & \, (X\cdot \cB - X)^T C \\
\mbox{s.t:} & \, \, \cB \in \{0,1\}^{n\times d} \, \mbox{,} \, \| \cB\|_0 \leq k \label{eq:integer_program}
\end{align}

\nando{Note that this is not what we have in section 3, discuss the difference (imposing sparsity). Also better discuss why we just need to take the sorted vector -- this is an Eucledian  projection onto the nonconvex set $\{W \vert \text{card}(W) \leq k\}$ ,but the special structure of this set allows us to express this projection in closed form (keep the $k$ largest elements of $B$ and set $0$ to the rest}

The solution of the binary linear  programming turns out to be setting $\cB_{ij}=1$ for the $k$ largest entries $ ( \cX_{i,j} -\phi) C_{ij}$
 and $\cB_{ij}=0$ otherwise. 
 
% \subsection{Gradient Descent}

% Given the complex formulation of the bilevel optimization, one go to approach to solving such problems is gradient descent. We can perform gradient descent to learn both the lower level optimization parameters $\theta$ and the upper level minimization matrix $\cB$ simultaneously. However, to do so, we need to first make the following relaxations and assumptions about the problem statement.

% \begin{itemize}
%     \item \textit{Approximating the minimization matrix $\cB$:} To allow gradient based updates of the minimization matrix $\cB$, we need to make its domain continous. That is, we redefine the minimization matrix $\cB \in [0,1]^{n \times d}$.
%     \item \textit{Differentiable Imputation:} The choice of data imputation plays an important role in the forward pass of the learned model $f_{\theta}(.)$. But, for a gradient based solution, we need to make sure the imputation method used is differentiable, to allow gradient updates to pass through it.
%     \item \textit{Local Minima:} To be able to reduce the bilevel optimization to a single level optimization using KKT conditions, we need to introduce the assumption that the lower level optimization might only achieve local minima.
% \end{itemize}

% \paragraph{Single Level Optimization: } Given that we have made the assumption for the lower level optimization only achieving local minima, we can now rewrite our optimization as,
% \begin{align}
%     \argmin_{\cB} ||\cB||_1 + \lambda*(\cL(\cX, \cY, \theta^*_{\cX \odot \cB}) - L_{c} - \alpha + t^2) \\
%     \textrm{where} \quad \triangledown \cL(\cX \odot \cB, \cY, \theta^*_{\cX \odot \cB}) = 0
% \end{align}

% \textbf{TODO: What's the link between the bilevel optimization and the gradient based solution?}

% \paragraph{Learning Loss: } The first loss is the lower optimization, i.e. training for loss a model on the minimized dataset. This is important because any downstream utility of the model will be judged by its ability to learn from the minimized dataset.
% \begin{align}
%     LL = \cL(\cX \odot \cB, \cY, \theta)
% \end{align}

% \paragraph{Alignment Loss: } The second loss we consider for our gradient based solution is the alignment loss. We want the model learned on the minimized dataset to perform similar to a model that was trained on the original dataset.
% \begin{align}
%     AL = \cA(\cX \odot \cB, \cX)
% \end{align}

% \paragraph{Sparsity Loss: } Finally, we consider the sparsity loss, which encourages the model to minimize data during learning.
% \begin{align}
%     SL = ||\cB||_1
% \end{align}

% \paragraph{Data Minimization: } All three losses defined above are combined together to form the overall learning objective. We then update both the minimization matrix $\cB$ and the learning parameters $\theta$ together using gradient descent, thus simultaneously learning the best minimization matrix and its corresponding model parameters. Finally, the resultant minimization matrix is discretized. Pseudo code for the gradient based minimization is present in Algorithm \ref{alg:gradient}.

% \begin{algorithm}
% \caption{Gradient Based Solution}\label{alg:gradient}
% \begin{algorithmic}
% \STATE Given hyperparameters $\beta, \gamma, \kappa$, epochs
% \STATE $\cB, \theta \gets$ Random Initialization
% \STATE $i=0$
% \FOR{$i \leq \textrm{epochs}$}
%     \STATE LL $\gets$ Learning Loss
%     \STATE AL $\gets$ Alignment Loss
%     \STATE SL $\gets$ Sparsity Loss
%     \STATE loss = $\beta*LL + \gamma*AL + \kappa*SL$
%     \STATE 
%     \STATE $\cB_{grad}, \theta_{grad} \gets \frac{\partial loss}{\partial \cB}, \frac{\partial loss}{\partial \theta}$
%     \STATE
%     \STATE $\cB \gets \cB - lr_{\cB} * \cB_{grad}$
%     \STATE $\theta \gets \theta - lr_{\theta} * \theta_{grad}$
%     \STATE $i=i+1$
% \ENDFOR
% \RETURN Discretize($\cB$)
% \end{algorithmic}
% \end{algorithm}

\subsection{Meta Model: Modeling Lower Optimization}

Gradient-based methods described above face two major issues, i.e., discretization error and the need for differential imputation methods. We now describe a metamodeling approach to bilevel optimization that can avoid both of these issues. The metamodeling approach relies on avoiding the lower optimization, but instead modeling it using a simpler learnable function. That is, we want to replace the loss calculation $\cL(\cX, \cY, \theta^*_{\cX \odot \cB})$ which relies on the lower level optimization for $\theta^*_{\cX \odot \cB}$, with a new function $m(\cB)$ that can directly estimate the loss value without solving for $\theta^*_{\cX \odot \cB}$.

\paragraph{Generating Input-Output Pairs: } We are going to learn the mapping between the minimization matrix $\cB$, and the loss value $\cL(\cX, \cY, \theta^*_{\cX \odot \cB})$. To do so, we first need to generate some matrix-loss pairs that will be vital to learning the mapping.

We start by generating a random minimization matrix $\cB$, with sparsity $s$. This is the same as performing personalized random subsampling as described earlier. We then solve the lower optimization for this $\cB$ and obtain the loss value. We repeat these steps multiple times to create a dataset to train $m(\cB)$. By using these input-output pairs, we can create a global approximation of the loss. One might even repeat this process multiple times during the overall optimization to create more accurate local approximations of the matrix-loss relationship.

\paragraph{Modeling $m(\cB)$: } To be able to learn an approximate mapping between the minimization matrix and the loss value, we make the following simplifying assumption.
\begin{itemize}
    \item \textit{Independent Influence: } We assume that the influence of any index $ij$ on the final loss value is independent of the rest of the minimization matrix. Thus, if we can quantify the influence of each index on the loss $\cI_{ij}$, we can aggregate it as:
    \begin{align}
        m(\cB) = \frac{1}{n d} \sum^n_{i=1} \sum^d_{j=1} \cI_{ij}
    \end{align}
\end{itemize}

Since each index in the dataset can only exist in two states, i.e., minimized or not minimized, we can simplify the influence of each index as,
\begin{align}
    \cI_{ij} =
    \begin{cases}
      \cI^1_{ij}, & \text{if}\ B_{ij}=1 \\
      \cI^{\phi}_{ij}, & \text{if}\ B_{ij}=\phi
    \end{cases}
\end{align}

Thus, we simply need to learn the parameters $\cI^1_{ij}, \cI^{\phi}_{ij}$ to complete the mapping $m(\cB)$. Given that we assume independent influence of each index on the minimization matrix, we can learn these parameters by calculating the average loss when $B_{ij}=1$ and $B_{ij}=\phi$, respectively.
\begin{align}
    \cI^1_{ij} = \frac{1}{|P^1|} \sum^{|P^1|}_{k=1} \cL(\cX, \cY, \theta^*_{\cX \odot P^1_k}) \quad \textrm{where} \quad P^1 := \{\cB \, | \, \cB_{ij}=1\} \\
    \cI^{\phi}_{ij} = \frac{1}{|P^{\phi}|} \sum^{|P^{\phi}|}_{k=1} \cL(\cX, \cY, \theta^*_{\cX \odot P^{\phi}_k}) \quad \textrm{where} \quad P^{\phi} := \{\cB \, | \, \cB_{ij}=\phi\}
\end{align}

\paragraph{Data Minimization: } After learning the parameters $\cI^1_{ij}, \cI^{\phi}_{ij}$, thus learning the modeling function $m(\cB)$, we can now simplify the original optimization as:
\begin{align}
    & \argmin_{\cB} ||\cB||_1 + \lambda*(m(\cB) - L_{c} - \alpha + t^2) \\
    \Rightarrow & \arg\min_{\cB} \sum^{n}_{i=1} \sum^{d}_{j=1} (1 + \lambda \cI^1_{ij})*\mathbbm{1}_{[\cB_{ij}=1]} + \lambda \cI^{\phi}_{ij}*\mathbbm{1}_{[\cB_{ij}=\phi]}
\end{align}
Clearly, the optimal minimization algorithm under the metamodeling assumptions is to minimize the indices with the highest values of $\cI^1_{ij} - \cI^{\phi}_{ij}$, until the desired level of sparsity.

\subsection{Evolutionary Algorithms}

\input{tables/tab_algorithms}

==> archived_sections/sec_app_baseline_proofs.tex <==
We introduce three baseline techniques for data minimization, namely feature selection, random subsampling, personalized random subsampling,

\paragraph{Feature Selection:} Feature selection is simply choosing the most important features while removing the rest and is a commonly used method to reduce dataset size in machine learning~\cite{}. The minimization matrix can be defined as:
\begin{align}
    \cB_{ij} = \phi \quad \forall j \in E_s
\end{align}
Here $E_s$ is the set of $s$ least important features in the dataset, and $s$ is a hyperparameter which controls the sparsity of the minimized dataset. We use the absolute correlation between each feature and the output label to measure the importance of each feature. It turns out deriving the relationship between target utility and origial utility under general settings is challenging. We provide the following theorem that derives 


\begin{theorem}
\label{thm:feature_selection}
Suppose all input features and labels are jointly Gaussian, i.e $[\bm{x},y] \sim \mathcal{N}(\mu, \Sigma)$, where $\Sigma = \begin{bmatrix} \Sigma_{\bm{x},\bm{x}}, \Sigma_{\bm{x},y} \\ \Sigma_{y,\bm{x}}, \Sigma_{y,y} \end{bmatrix}$. Furthermore, we assume that all input features are mutually independent, i.e the covariance matrix $\Sigma_{\bm{x},\bm{x}} = diag([\sigma^2_i]^p_{i=1})$ is a diagonal matrix and $\sigma^2_i = Var[\bm{x}^i]$ the variance of i-th feature. Then the Bayes MSE error when using all input  $\bm{x}$ features and using a subset of input features in  $[d] \setminus E_s$ in turn are: $Var[y] - \sum^{d}_{i=1}\frac{(Cov(y, \bm{x}^i))^2}{\sigma^2_i} ]$
and  $Var[y] - \sum_{i \in [d] \setminus E_s}\frac{Cov(y, \bm{x}^i))^2}{\sigma^2_i}$
\end{theorem}

Theorem \ref{thm:feature_selection} suggests using a subset of feature $E_s$ introduces an additional MSE error of $ \sum^{d}_{i=1}\frac{(Cov(y, \bm{x}^i))^2}{\sigma^2_i} ] - \sum_{i \in [d] \setminus E_s}\frac{Cov(y, \bm{x}^i))^2}{\sigma^2)i]} = \sum_{i \in E_s} \frac{(Cov(y, \bm{x}^i))^2}{\sigma^2_i}   $. As long as all feature in the removed feature set $ E_s$ has small correlation with the label, i.e $Cov(y, \bm{x}^i)\approx 0$, such additional MSE error is neligible. 

\paragraph{Random Row Subsampling:} Random row subsampling is a minimization method that randomly chooses a subset $S$ of data samples with replacement from the original dataset, and is another very common technique of reducing dataset size for faster training~\cite{}. The motivation behind sampling with replacement (a.k.a boostrapping) is to retain the statistics of the minimized data. We provide 


\begin{theorem}
\label{thm:sampling_bound}
Suppose the loss function $\ell(f_{\btheta}(\bm{x}_i), y_i)$ is convex  w.r.t $\btheta, \forall (\bm{x}_i,y_i)$. If we denote $\Sigma$ to be the empirical covariance matrix of the set of deterministic individual gradient vector $\{ g_i(\btheta^*) \}^n_{i=1}$  where $g_i(\optimal{\theta})= \frac{\partial \ell(f_{\optimal{\theta}}(\bm{x}_i), y_i)}{\partial \btheta}$ then the following holds:

\begin{align}
\mathbf{E}[\| \btheta^*_{\cX'} - \btheta_{\cX}\| ] \leq \frac{2 \text{Trace}(\Sigma)}{\lambda |S|} 
\end{align}

\end{theorem}



Theorem \ref{thm:sampling_bound} derives the upper bound on the difference between model parameters learned on minimized and complete data. It suggest the more number of training samples you can draw, the smaller the difference between models trained on minimized data vs original data. 

Our proof relies on the following classical theorem in statistis\cite{moore2009introduction}.
\begin{lemma}
\label{lem:variance}

Consider a set of deterministic vector $\{ g_1(\btheta), ..,g_n(\btheta)\}^n_{i=1}$ with sample covariance variance $\Sigma$. If $S = \{ i | i \overset{\mathrm{iid}}{\sim} [n] \}$ then 

$$ \text{Trace}\left[Var[\frac{1}{|S|}\sum_{i \in S} g_i(\btheta)] \right] = \frac{\text{Trace}(\Sigma)}{|S|}$$
\end{lemma}


The Lemma \ref{lem:variance} implies that the more number of draw samples (i.e $|S|$ large) the smaller the  variance of sample mean.  

\begin{proof}
By the assumption that the individual loss $\ell(f_{\btheta}(x_i), y_i)$ is convex w.r.t $\btheta$ for all $(\bm{x}_i,y_i)$, then the following empirical risk on minimized data is $\lambda$-strongly  convex:

\begin{align}
\hat{L}(\btheta) = \sum_{i\in S} \ell(f_{\btheta}(\bm{x}_i), y_i) + \lambda \| \btheta\|^2_2. 
\end{align}
By the propery of strongly convex function it follows that:

\begin{align}
  ( \nabla_{\btheta} \hat{L}(\hat{\btheta}) -  \nabla_{\btheta} \hat{L}(\btheta^*)  )^T (\hat{\btheta} -\btheta^*)  \geq \frac{\lambda}{2} \| \hat{\btheta} - \btheta^* \|^2_2
\label{eq:diff}
\end{align}

Since $\hat{\btheta} = \text{argmin}_{\btheta} \hat{L}(\btheta)$ hence $\nabla_{\btheta}\hat{L}(\hat{\btheta}) = \bm{0}^T $. Thus the L.H.S of Equation \ref{eq:diff} can be reduced to $-\nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  $ 

Taking the expectation on both sides we obtain:

\begin{equation} \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right]\geq \frac{\lambda}{2} \mathbf{E}\left[ \| \hat{\btheta} -\btheta^*\|^2_2 \right]
\label{eq:1}
\end{equation}


Apply the Cauchy-Schwarz inequality for expectation, i.e  for any two random variables $X$ and $Y$ then $| \mathbf{E}[X^TY] | \leq  \sqrt{\mathbf{E}[X^TX]  \mathbf{E}[Y^TY] } $ it follows that:


\begin{align} \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right]& \leq \left| \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right] \right| \\
& \leq \sqrt{ \mathbf{E}[ \|  \nabla_{\btheta} \hat{L}(\btheta^*) \|^2_2] \mathbf{E}[ \| \hat{\btheta} -\btheta^*\|^2_2] } \\
& =  \sqrt{ \mathbf{E}[ \|  \nabla_{\btheta} \hat{L}(\btheta^*) \|^2_2] }  \sqrt{ \mathbf{E}[ \| \hat{\btheta} -\btheta^*\|^2_2}
\label{eq:2}
\end{align}

Combine Equation \ref{eq:1} and Equation \ref{eq:2} we obtain:
\begin{equation}
 \mathbf{E}\left[ \|   \nabla_{\btheta} \hat{L}(\btheta^*)\|^2_2 \right] \geq \frac{\lambda}{2} \mathbf{E}\left[ \| \hat{\btheta} -\btheta^* \|^2_2 \right] 
\label{eq:3}
\end{equation}
\newcommand{\indep}{\perp \!\!\! \perp}

By the following property  for any random variable $X$  if $X_i \indep X_j $ for $X_i, X_j$ are two arbitrary entries of $X$   then $\mathbf{E}[ ||X||^2_2 ] = (E[X])^T E[X] + \text{Trace}[Var[X]]$. Furthermore, 

$$ \mathbf{E}[  \nabla_{\btheta} \hat{L}(\btheta^*)] =\mathbf{E}[\sum_{i \in S} g_i(\btheta^*) ] = \sum_{i \in S} \mathbf{E}[ g_i(\btheta^*) ]  = \bm{0}^T$$

The last equation comes from the fact that $g_{i}(\btheta)$ is drawn from a set of $\{  g_i(\btheta^*) \}^n_{i=1}$ whose the mean is a zero vector. 

Thus:

\begin{align}  \mathbf{E}\left[ \|   \nabla_{\btheta} \hat{L}(\btheta^*)\|^2_2 \right] & = \bm{0}^T + \text{Trace}( Var[\nabla_{\btheta} \hat{L}(\btheta^*)]) = \frac{\text{Trace}(\Sigma)}{|S|}\\
& \geq \frac{\lambda}{2} \| \hat{\btheta} -\btheta^* \|^2_2
\end{align}

\end{proof}
% The minimization matrix can be defined as:
% \begin{align}
%     \cB_{ij} = \phi \quad \forall \, U_i=0
% \end{align}
% Here $U \in \{0, 1\}^n$ is a randomly permuted binary vector, with exactly $s$ indices filled with $1$, i.e., $\Sigma_i U_{i} = s$, to control the desired sparsity of the minimization.

\paragraph{Personalized Random Subsampling:} Personalized random subsampling is an extension of random subsampling, but instead of removing complete data points it removes individual values in the dataset matrix, i.e. perform personalized minimization. The minimization matrix can be defined as:
\begin{align}
    \cB_{ij} = \phi \quad \forall \, U^P_{ij}=0
\end{align}
Here $U^P \in \{0, 1\}^{n \times d}$ is a randomly permuted binary matrix, with exactly $s$ indices filled with $1$, i.e., $\Sigma_{ij} U^P_{ij} = s$, to control the desired sparsity of the minimization.

\begin{theorem}[Utility bound for personalized random subsampling]

The target utility  of interest $\cL(\cX, \cY, \bm{\theta^{*}}_{\cX \odot \cB} )$ under personalized random subsampling can be upper bounded by the original utility $\cL(\cX, \cY, \bm{\theta^{*}}_{\cX} )$  as follows:

$$ \cL(\cX, \cY, \bm{\theta^{*}}_{\cX'} ) \leq  \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) +  s \times \|X \|_{\infty} \times \| L H^{-1} G\|_2 + \cO\big( \| X'-X\|^2\big).$$

Where:
\begin{equation} L =\frac{\partial \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta}}  \,\, \text{(1st derivative w.r.t param )}
\label{eq:item1}
\end{equation}


\begin{equation} H =\frac{\partial^2 \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta}^2} \, \, \mbox{ (Hessian matrix of param) } 
\label{eq:item2}
\end{equation}

\begin{equation}
G = \frac{\partial^2 \cL(\cX, \cY, \bm{\theta^{*}}_{\cX} ) }{\partial \bm{\theta} \partial \cX} \, \, \mbox{ (2nd derivative w.r.t param and input) }
    \label{eq:item3}
\end{equation}



\end{theorem}

==> archived_sections/sec_app_datasets.tex <==
\paragraph{Tabular Datasets:} We will perform our experiments and ablations studies on four different tabular datasets, i.e., the bank marketing dataset~\cite{moro2014data}, the wine quality dataset~\cite{cortez2009modeling}, and two different tasks (ACSIncome and ACSEmployment) from the folktables dataset~\cite{ding2021retiring}. 

The bank marketing dataset~\cite{moro2014data} is a telemarketing dataset from the UCI Machine Learning Repository, with information on 11,162 bank customers who were offered term deposit accounts. The dataset contains 16 features for each data point, including personal information, financial details, and marketing campaign attributes. The dataset is used for a binary classification task, predicting whether the customer ultimately opened a term deposit account.

The wine quality dataset~\cite{cortez2009modeling} is another dataset from the UCI Machine Learning Repository, with 12 attributes each for a total of 6,463 unique wines. We transform this dataset into a binary classification task, by selecting one attribute (red wine or white wine) as the prediction target and utilize the remaining 11 attributes as input features.

Folktables dataset~\cite{ding2021retiring} is a recently collected census dataset designed to improve and update the older and commonly used UCI Adult Income dataset~\cite{Dua:2019}. In our paper, we will use two specific tasks from the folktables dataset: (i) ACSIncome, a dataset with the binary classification task of predicting whether an individual's income is above $\$50,000$, given a set of 10 unique features containing personal information, and (ii) ACSEmployment, a dataset with the binary classification task of predicting whether an individual is currently employed, given a set of 16 unique features. In both tasks, we randomly selected a subset of 5,000 data points for our experiments.

\paragraph{Handwritten Digits Dataset:} We use the optical recognition of handwritten digits dataset~\cite{xu1992methods}, made of $8 \times 8$ single channel images with integer pixel values between $[0, 16]$. The dataset contains a total of 1797 images, across 10 different classes, each representing a digit.

\paragraph{20 Newsgroup Dataset:} We use the 20 newsgroup text dataset~\cite{}, a collection of 18,846 news posts across 20 diverse sets of topics. As recommended, we strip any newsgroup-related metadata from these posts to ensure a more realistic classification setting. Furthermore, to limit the size of each news post, we truncate them to only the first 50 tokens.

==> archived_sections/sec_baselines.tex <==
\section{Minimization: Powerful Baselines}

We introduce three baseline techniques for data minimization, namely feature selection, random subsampling, personalized random subsampling,

\paragraph{Feature Selection:} Feature selection is simply choosing the most important features while removing the rest, and is a commonly used method to reduce dataset size in machine learning. The minimization matrix can be defined as:
\begin{align}
    \cB_{ij} = \phi \quad \forall j \in E_s
\end{align}
Here $E_s$ is the set of $s$ least important features in the dataset. We use the absolute value of the coefficients of a logistic regression trained on the dataset $\cD$ to measure the importance of each feature.

\paragraph{Random Subsampling:} Random subsampling is a minimization method that randomly chooses a subset of datapoints from the original dataset, and is another very common technique of reducing dataset size for faster training. The minimization matrix can be defined as:
\begin{align}
    \cB_{ij} = \phi \quad \forall \, U_i=0
\end{align}
Here $U$ is a randomly generated binary vector of size $|U|=n$, such that the probability of generation $P[U_i=0] = s$ controls the desired sparsity $s$ of the minimization.

\textcolor{red}{I think the above might need revision. Becareful, if you randomly delete one training sample with probability s, it does not mean at the end you always left with $n(1-s)$ samples. But sometimes, you can have more than $n(1-s)$ and sometimes you can have less than $n(1-s)$. On expectation, you get $n(1-s)$. }
\textcolor{blue}{(What would be a good way to write 'exactly' s\% of data was removed randomly from the dataset? I wasn't able to figure out a simple mathematical version of the same.)}

\paragraph{Personalized Random Subsampling:} Personalized random subsampling is an extension of random subsampling, but instead of removing complete data points it removes individual values in the dataset matrix, i.e. perform personalized minimization. The minimization matrix can be defined as:
\begin{align}
    \cB_{ij} = \phi \quad \forall \, U_{ij}=0
\end{align}
Here $U$ is a randomly generated binary matrix of size $|U|=n \times d$, such that the probability of generation $P[U_{ij}=0] = s$ controls the desired sparsity $s$ of the minimization.

% \input{sections/sec_theoretical_proofs_baseline_old}

\textcolor{blue}{Some desirable theorems can be,
\begin{enumerate}
    \item Theorem: Under some given constraints of the dataset distribution (for example, maybe we can assume gaussian distribution), we show that the drop in performance for personalized random subsampling is bounded. That is, there are certain guarantees that you get with personalized random subsampling method.
    \item Theorem: Under some given constraints, we show that the drop in performance for personalized random subsampling is always less than that of just random subsampling. That is, we motivate the 'personalized' nature of data minimization.
\end{enumerate}}

==> archived_sections/sec_evaluations.tex <==
\subsection{TODO: Add Experiment Setup and Results}

List of Insights
\begin{itemize}
    \item First highlight the data minimization trends across a wide range of datasets, including tabular, text, and image. This includes discussions of regularization due to data minimization, and discussions of what minimization looks like visually.
    \item Talk about Different Minimization Algorithms and Their Performance With Changing Sparsity, Changing Model Complexity, Changing Data Complexity, Etc.
    \begin{itemize}
        \item Show the ablation study of different imputation methods in taylor approximation.
        \item Show how taylor approximation fails for higher sparsity.
        \item Show the ablation study of different number of iterations and sparsity value during data creation for metamodeling.
        \item Show how metamodeling method fails for datasets with highly correlated features, like for example the handwritten image dataset.
        \item Show the ablations study of number of iterations and population size for evolutionary methods.
        \item Show the runtime of different methods, and how it scales with bigger datasets, bigger models.
    \end{itemize}
    \item Highlight the consistency of the minimization method for different algorithms across random seeds and across increasing sparsity.
    \item Introduce the efficacy of our adversarial attacks, the improvement of privacy under minimization, and yet the misalignment between data minimization and privacy (i.e., one thing does not 'ALWAYS' mean the other thing).
    \item Introduce DP-SGD into the pipeline, and show the comparison of DP-SGD with data minimization as well as their compatibility with each other.
    \item Introduce defences for various attacks into the pipeline (as a part of the 'utility') and show how does it effect the downstream privacy vs other factors previously studied.
    \item Talk about fairness in data minimization, and more specifically the impact of minimization in various subgroups of the data.
    
\end{itemize}



\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_reidentification_minimization} 
    \caption{Model Accuracy vs Reidentification Risk: Logistic Regression (Tabular Datasets Only)}
	\label{fig:reid}
\end{figure*}


\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_reconstruction_minimization} 
    \caption{Model Accuracy vs Reconstruction Risk: Logistic Regression (Tabular Datasets Only)}
	\label{fig:recon}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_ner_minimization} 
    \caption{Model Accuracy vs Number of Named Entities: Bag of Words (Text Datasets Only)}
	\label{fig:ner}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_nn_dataset_size_minimization} 
    \caption{Model Accuracy vs Dataset Size: MLP Single Hidden Layer (Tabular Datasets Only)}
	\label{fig:nn_dataset_size}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_nn_reidentification_minimization} 
    \caption{Model Accuracy vs Reidentification Risk: MLP Single Hidden Layer (Tabular Datasets Only)}
	\label{fig:nn_reid}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_nn_reconstruction_minimization} 
    \caption{Model Accuracy vs Reconstruction Risk: MLP Single Hidden Layer (Tabular Datasets Only)}
	\label{fig:nn_recon}
\end{figure*}

\begin{figure*}[hbtp]
    \centering
    \input{figure_scripts/fig_nn_mia_minimization} 
    \caption{Model Accuracy vs MIA Risk: MLP Single Hidden Layer (Tabular Datasets Only)}
	\label{fig:nn_mia}
\end{figure*}

\input{tables/tab_multiplicity}
\subsection{Defense Methods against the Inference Attacks}
Different data minimization methods in Section \ref{sec:algorithms} focus only on utility of the learning models without any attention to the information leakage. In this subsection, we introduce a general defense framework against the inference attacks in data minimization problem. We assume that the data minimization process procedues a utility score matrix $\cU \in {n\times d}$, where each entry $\cU_{i,j}$ indicates the utility of feature $X_{ij}$. The higher  the value of $\cU_{i,j}$ is, the better the learning model $\hat{\btheta}$ will be if it is retained during minimization process. Our defense mechanism relies on constructing a privacy matrix score $\cP \in {n\times d}$, where $\cP_{i,j}$ represents for the amount of information leakage if  feature $\bm{x}_{ij}$ is revealed. $\cP$ is constructed differently for reconstruction and reidentification attack.

\paragraph{Denfese framework} Our proposed defense method first constructing the total utility-privacy score $ \cU + \beta \times \cP$  ($\beta>0$) which is a weighted combination between utility and privacy score. Note that in our experiment, we normalize both utility and privacy scores to be in the range $[0,1]$. The data minimization framework will keep only the top $k$ feature entries $\bm{x}_{ij}$ that have highest utility-privacy sscore. In the following discussion, we provide the implementation of privacy score for reconstruction and reidentification attack.

\paragraph{Privacy score for reidentification attack} In reidentification attack, the risks comes from publishing so-called \emph{unique} features of individuals. For example, considering a cancer patient database, if the outputs of data minimization process reveal some unique attributes like phone number, zip codes, then the adversary can identify well these patients from some public/axulirary data. In contrast, if the output of data minimization process releasing  less unique attributes like gender, races,... the adversay find it more difficult to identify such cancer patient since many individuals sharing the same gender, races. Based on this motivation, we propose the following  privacy scores $\cP$ against the reidentification attack:

$$ \cP_{ij} = - | \text{Dom}(\bm{x}^j)|,$$
where $\text{Dom}(a)$ denotes the domain of feature attribute $a$.

\paragraph{Privacy score for reconstruction attack}  In reconstruction attacks, the risks comes from releasing the features that have high correlation with other features. In fact, upon releasing these features, the adversary with knowledge from the underlying data distributon $P(\bm{x})$ can infer the missing features. To defend such attack, we propose the following privacy scores $\cP$:

$$\cP_{i,j} =- \sum_{h\neq j} | \text{Corr}(\bm{x}_j, \bm{x}_h)|,$$

where $\text{Corr}(a,b)$ compute the Pearson correlation between two vector $a$ and $b$.



==> archived_sections/sec_our_setting.tex <==
\subsection{Data minimization under retrospective} 
Under the retrospective setting a data holder processeses a training data $\cD = \{x_i, y_i\}^n_{i=1}$ of $n$ individuals, where $x_i \in \cX =R^{d}, y_i \in \cY$ are respectively input and output feature. The dataset will typicall  be used to train a learning model that minmizes the following empirical risk:

$$ \theta^* = \text{argmin}_{\theta} \sum^n_{i=1}  \ell\bigg(f_{\theta}(x_i), y_i\bigg) $$

The data holder would like to process the data to remove redundant information under data minimization principle and publish it or deliver it to the third party. The minimized data might be combined with third party's local data to train a learning data in the subsequent step.
In this paper, we consider one typical data minimization process which involves deleting/or retaining  a feature $x_{ij}$ for i-th user. The decision can be captured by  a binary indicator matrix $\bm{B} \in \{0,1\}^{n\times d}$, where $B_{i,j}=1$ indicates the $j$-th feature of i-th training sample should be retained, and $B_{i,j}=NULL$ if it should be discarded.  In the following, we denote $X= \{x_i\}^n_{i=1} \in R^{n\times d}$ to be the original feature matrix, and $X' = X \cdot B$ to the minimized dataset. Since $X'$ contains some missing values, the data holder might want to replace the missing values by some imputation method and obtain $X"$. 

The goal of the data users is to retain the quality and avoid privacy leakage. 


\paragraph{Retaining accuracy as possible} The first goal in data minimization is to collect minimum data without any loss in accuracy over original data. This can be formulated as follows:

\begin{align} &\min_{\bm{B}} \sum^n_{i=1} \ell\bigg(f_{\theta^*}(x_i), y_i\bigg) \\
& \text{s.t:} \, \, \theta^* = \text{argmin} \sum^n_{i=1} \ell\bigg(f_{\theta^*}(x_i \cdot \bm{B}_i), y_i\bigg),
\label{eq:main_obj}
\end{align}

where $B_i$ denotes the $i$-th row of the matrix $\bm{B}$. In other words, we would like to identify a binary matrix such that when we train a model $f_{\theta}$ over the minimized data, the model also minimizes the loss over the original data. 




\paragraph{Capacitiy constraint over set of selected entries} In addition to retaining high accuracy, we also the number of entries we should discard is at most  $C$, $\| B\|_0 \geq C$. We replace the $l_0$ constraint by the following $l_p$ ($0<p<1$) constraint:

\begin{equation} B^* =  \argmin_{B \in \{0,1\}^{n\times d}} \| B\|_p 
\label{eq:capacity}
\end{equation}

\paragraph{Privacy constraint over $B$}
We also want to make sure that the data minimization process does not reveal any sensitive information of users $x_i$. We will discuss two attack models in Section \ref{sec:attack_model}




\subsection{Attack models}
\label{sec:attack_model}
In the scope of this paper, we consider two different attacks: \emph{reconstruction} and \emph{membership inference attack} (MIA)

\paragraph{Data reconstruction attacks} In the reconstruction attacks, the adversary wants to reconstruct the original feature data $X$ based on the published data $X"$. If we denote $\tilde{X}$ to be the reconstructed data, then the success of the attack  is measured by the reconstruction error $$\| \tilde{X} -X \|$$.


\paragraph{Membership inference attack}
In this attack, given one record $x$ from the underlying data distribution $P(x)$, the adversary wants to determinef if $x \in D$.  He constructs a score function $g(x)$ that tells how likely $x \in D$. 
The success of MIA can be measured by the AUC between $\bm{1}\{x \in D \}$ and $g(x)$.




% In addition, we would like the reamining features entries can keep privacy of the original dataset. We consider the uniquness as a proxy measure for privacy in this context. This can be formulated as follows:


% \begin{equation} \forall i \in [n] \sum^n_{j=1} \mathbf{1}[\Delta( x_i \cdot B_i; x_j \cdot B_j) \geq \delta] \geq k
% \label{eq:privacy_constraint}
% \end{equation}

% In particular, the uniquness constraint requires the number of individuals in the dataset that are $\delta$-proximal to $x_i$  is at least $k$.

% \paragraph{Overall optimization problem}

% Combining the main objective in Equation \ref{eq:main_obj}, and the capacity constraint in Equation \ref{eq:privacy_constraint}, we obtain the following:


% \begin{align} 
% \begin{split}
% \min_{\bm{B^*}, \theta}  & \sum^n_{i=1} \ell\bigg(f_{\theta}(x_i \cdot B^*_i), y_i\bigg)\\
% \mbox{s.t} &  \, B^* =  \argmin_{B \in \{0,1\}^{n\times d}} \| B\|_p  \\
% \mbox{and:} & \, \forall i \in [n] \sum^n_{j=1} \mathbf{1}[\Delta( x_i \cdot B_i; x_j \cdot B_j) \geq \delta] \geq k
% \label{eq:privacy_constraint}
% \end{split}
% \end{align}


\subsection{Data minimization under active learning setting}

==> archived_sections/sec_privacy_metrics.tex <==
\section{Privacy Metrics}

\subsubsection{Re-identification Risk (RIR)}

The effectiveness of the re-identification attack is evaluated through the utilization of mean reciprocal rank (MRR) scores, which assess the quality of the rankings provided by the attacker. Specifically, for each data point $x_i$ in the auxiliary dataset $\mathcal{X}$, the adversary generates a ranking of all data points in the minimized dataset $\mathcal{X}'$ based on their likelihood of being the data point corresponding to the original feature vector $x_i$. The re-identification risk can then be quantified by computing the average MRR scores, where a score of $1$ is assigned to the correct match and a score of $0$ is assigned to all other matches, and can be defined alternatively as follows:
\begin{align}
    \textrm{RIR} = \frac{1}{|\cX|} \sum\limits_{i=1}^{|\cX|} \frac{1}{\textrm{index}(i, \textrm{rank}(x_i, \cX'))},
\end{align}
where $\textrm{rank}(x_i, \cX')$ represent the ranking of data points as predicted by the adversary, and $\textrm{index}(e, A)$ returns the index (1-based indexing) of some element $e$ in the array $A$.

\subsubsection{Reconstruction Risk (RCR)}

Given the minimized dataset $\cX'$ (and potentially access to some public data $D_{pub}$), the attacker's goal is to generate their optimal reconstruction $\cX^R$ of the original set of features $\cX$. The reconstruction risk can be evaluated by measuring the similarity between the original features $x_i \in \cX$ and the reconstructed features $x_i^R \in \cX^R$, computed as the negative exponential of the euclidean distance as illustrated below:
\begin{align}
    \textrm{RCR} = \frac{1}{|\cX|} \sum\limits_{i=1}^{|\cX|} e^{-|| x_i - x_i^R ||_2},
\end{align}
As noted previously, this metric treats the reconstruction of all features equally, while adjustments can be made to prioritize or disregard the reconstruction of specific features.

\subsubsection{Membership Inference Risk (MIR)}

During a membership inference attack, the adversary assigns a likelihood score $L(x_q)$ to each query $x_q$, indicating the probability of it being a member of the original dataset $\cX$ given access to the minimized dataset $\cX'$, i.e., $L(x_q) = P[x_q \in \cX | \cX']$. Using these likelihood scores for both the complete set of original data points $\cX$ and a set of non-members $\cX_{nm}$, binary predictions for membership can be generated using a threshold $t$, denoted as $1_{L(x_q) \geq t}$. The membership inference risk is then quantified as the area under the curve (AUC) of the true positive rate (TPR) and false positive rate (FPR) of various thresholds $\vec{tpr}={tpr_{t=t_1}, tpr_{t=t_2}, ..}$ and $\vec{fpr}={fpr_{t=t_1}, fpr_{t=t_2}, ..}$ respectively, as shown below:
\begin{align}
    \textrm{MIR} = \textrm{AUC}(\vec{tpr}, \vec{fpr}),
\end{align}

==> archived_sections/sec_problem_statement.tex <==
\section{Problem Statement}

\subsection{Formalizing Data Minimization}

Let us consider a dataset $\cD \in \cR^{n \times k}$ consisting of $n$ data points, where each data point is described by $k$ features. Data minimization can be defined using a binary matrix $\cB \in \cR^{n \times k}$, which indicates the features revealed for model training. Consequently, the minimized dataset $\cD^m$ can be represented as the element-wise product of $\cD$ and $\cB$, i.e., $\cD^m = \cD \otimes \cB$. The objective of data minimization is to identify an optimal binary matrix $\cB^*$ that allows an ML model trained on the minimized dataset $\cD^{m*} = \cD \otimes \cB^*$ to exhibit comparable utility to a model trained on the original dataset $\cD$, while simultaneously minimizing the potential information leakage between $\cD$ and $\cD^{m*}$.

\subsubsection{Active Data Minimization} In the active setting, we initially start with an empty or partially filled binary matrix $\cB$ for the purpose of minimization. The objective is to gradually disclose features in order to enhance the utility of a model trained on the revealed dataset, while still preserving the privacy benefits obtained through the minimization process. This approach is forward-looking, as we make decisions regarding which features to reveal based on our anticipation of their potential value, without having knowledge of their specific values. Once a feature is revealed, we do not discard or remove the feature in any subsequent steps, which remains an area for further exploration and investigation.

\subsubsection{Retrospective Data Minimization} In the retrospective setting, we already have access to the complete dataset, i.e., the initial binary matrix $\cB_{i,j} = 1 \textrm{ } \forall i, j$, and the process of data minimization entail selectively discarding or removing feature values to introduce privacy benefits while retaining the dataset utility. In contrast to the active setting, retrospective data minimization takes a backward-looking perspective, leveraging the complete dataset to make informed decisions about which feature values to discard. The objective is to strike a balance between privacy preservation and maintaining the utility of the dataset.

Overall, while active data minimization focuses on gradually revealing features to enhance model utility, retrospective data minimization takes a different approach by starting with the complete dataset and systematically dropping feature values. Both approaches have their merits and can be applied depending on the specific requirements and constraints of the data minimization task.

\subsection{Threat Models}

We now present a comprehensive introduction of various threat models that will be employed to measure privacy leakage in our framework. We recognize the importance of considering a wide range of threat models that reflect real-world privacy risks. Therefore, each threat model is designed to simulate a specific privacy breach scenario, enabling us to evaluate the extent of information leakage under various objectives and degrees of access available to the adversary.

\subsubsection{Re-identification Attacks}

One of the central concerns in privacy leakage through a target dataset is the re-identification of individuals even in the presence of only partial (or anonymized) features. Re-identification attacks rely on an auxiliary dataset(s) to obtain public information about an individual, which can be matched with the partial information available in the target dataset to identify them \cite{henriksen2016re}.
In our setup, the minimized dataset $\cD^m = \cD \otimes \cB$ is the target dataset under attack, and we simply use the original dataset $\cD$ as the auxiliary dataset to establish an upper bound on re-identification risk without relying on specific auxiliary features. The attacker's goal is to find the best match in the minimized dataset for each individual data point in the original dataset.

The success rate of the re-identification attack is measured using mean reciprocal rank (MRR) scores, which assess the quality of the mapping between the two datasets. More precisely, for every datapoint in the auxiliary dataset $x_i \in \cD$, the matching algorithm ranks all data points in the target dataset $\cD^m$, based on euclidean distance $||.||_2$. The attack's success, or in other words the re-identification risk, can be measured as the average MRR across all data points, i.e.,
\begin{align}
    \textrm{Re-identification Risk} = \frac{1}{|\cD|} \sum\limits_{i=1}^{|\cD|} \frac{1}{\textrm{rank}(x_i, \cD^m)}, \\ 
    \textrm{rank}(x_i, \cD^m) = \textrm{index}(i, \textrm{ } \underset{j \in |\cD^m|}{argsort} || b_j \otimes x_j - x_i ||_2),
\end{align}
where $\textrm{index}(e, A)$ returns the index (1-based indexing) of some element $e$ in the array $A$.

\subsubsection{Reconstruction Attacks}

Real-world datasets typically exhibit underlying associations between input features, making it possible to approximate missing features by studying the remaining data. Thus, even if certain information is missing from a partial (or anonymized) dataset, it does not guarantee that this particular information cannot be reconstructed using the rest of the data.
Reconstruction attacks, distinct from re-identification attacks, aim to recover missing information from a target dataset irrespective of its importance in re-identifying individuals, often using aggregate statistics alongside the dataset itself.

In our setup, we employ an imputation method $\cP$ that takes the minimized dataset $\cD^m$ and aggregate statistics $\cS$ as inputs, producing a reconstructed dataset $\cD^{\cP(\cD^m, \cS)}$ with no missing values. The quality of aggregate statistics can help us control the attacker's degree of access. Reconstruction risk is measured by computing the similarity between original and reconstructed features, with similarity defined as the negative exponential of the euclidean distance, i.e.,
\begin{align}
    \textrm{Reconstruction Risk} = \frac{1}{|\cD|} \sum\limits_{i=1}^{|\cD|} \textrm{sim}(x_i, x^{\cP(\cD^m, \cS)}_i), \\
    \textrm{sim}(x_1, x_2) = e^{-|| x_1 - x_2 ||_2}
\end{align}
Although our approach treats all features equally, modifications can be made to prioritize or ignore the reconstruction of specific features if desired.

\subsubsection{Membership Inference Attacks}

Membership inference attacks threaten the privacy of individuals by attempting to determine whether their data was included in the original dataset prior to minimization. The level of attacker access can vary, ranging from the complete minimized dataset (\textit{white-box}) to solely a model trained on the minimized dataset (\textit{gray-box}) or even just the outputs of such a model (\textit{black-box}). We will leverage existing literature on membership inference attacks to perform gray-box and black-box attacks by training shadow models explicitly for this purpose. For the white-box attack, we will employ a combination of re-identification followed by reconstruction to measure the likelihood of membership for a data point, given the minimized dataset.

In each of the three scenarios, the membership inference attacks yield a metric $L(x_i)$ that indicates the membership status of a data point $x_i$ in the training set. One can then generate binary classifications for membership based on a given threshold $t$ as $1_{L(x_i) \geq t}$. The membership inference risk can then be measured as the area under the true positive rate-false positive rate curve for changing thresholds, i.e.,
\begin{align}
    \textrm{Membership Inference Risk} = \textrm{AUC}(\vec{tpr}, \vec{fpr}),\\ 
    \vec{tpr}=\{tpr_{t_1}, tpr_{t_2}, ..\}, \vec{fpr}=\{fpr_{t_1}, fpr_{t_2}, ..\},\\ 
    tpr_{t_k} = P [L(x_i) \geq t_k | y_i=1], \\
    fpr_{t_k} = P [L(x_i) \geq t_k | y_i=0],
\end{align}
where $P[.]$ is the empirical probability of an event.

% For our setup, we will use the likelihood ratio attack (LiRA) to measure the membership inference risk of the models trained on the minimized dataset. Note that while our models are trained on the minimized dataset, the real risk of membership is still associated with the original data points, and thus we will perform membership inference directly on the original data points.

% Specifically, we start by using various overlapping subsets of auxiliary data available to the attacker to train multiple shadow models. We assume the attacker has access to the data minimization algorithm, and thus can replicate the minimize and training pipeline for shadow models and auxiliary data. Next, we then pass each data point under observation through all shadow models as well as the target model and calculate the likelihood of the data point being in the training set of the target model, given that we know it is not in the training set of any of the shadow models. As mentioned previously, this likelihood calculation is performed on the original data point, and not its minimized counterpart, since we want to ascertain the membership of the original data point.

% More specifically, we first train a $n$ shadow models $M^s_1, M^s_2, M^s_3, .., M^s_n$ on random subsets of the minimized and imputed auxiliary dataset $(X_{aux}^{\cP(B)}, y_{aux}) \in D_{aux}$. We then pass the datapoint $x_i \in \{X^{mem} + X^{nonmem}\}$ through all the shadow models as well as the target model $M^t$ trained on $X^{mem}$ to get the output logit values and [Insert the LiRA attack explanations and likelihood calculations here].

\subsection{Unifying the Framework}

We aim to address two critical aspects that have been missing in the data minimization literature: the formalization of the process itself and the quantification of utility and privacy benefits within minimized datasets. Our proposed framework presents a versatile approach to discussing data minimization, irrespective of the specific method employed or whether it is implemented actively or retrospectively. Alternative approaches beyond those proposed in our study can be explored to develop better minimization algorithms, improve model training on minimized datasets, devise more effective attacks, and even identify new attack scenarios. Nonetheless, the framework we introduce establishes a robust foundation for researchers to engage in discussions surrounding the data minimization principle and provide a mathematical framework to track the progress in this field. For a comprehensive overview of our framework, please refer to Figure \ref{fig:framework}.

% In the next section,  Through the training of a model using minimized data (and techniques such as data imputation), we are able to evaluate the utility of the minimization method. Subsequently, we delve into real-world attack scenarios to assess the resulting privacy implications or benefits of the minimized dataset.

% The dynamic interplay between attackers and defenders in privacy attacks will drive the advancement of attack methods and necessitate corresponding improvements in data minimization techniques. As the game evolves, more sophisticated attacks underscore the need for enhanced minimization methods, while progress in minimization pushes attackers to refine their strategies, thus perpetuating the cycle. 

% TODO: Improving the Figure
% \begin{figure*}[hbtp]
%     \centering
%     \input{figure_scripts/fig_framework} 
%     \caption{Caption.}
% 	\label{fig:framework}
% \end{figure*}

==> archived_sections/sec_theoretical_proofs_baseline_old.tex <==
\subsection{Theoretical analysis of baseline models}

In this section, for notional convenience we respectively denote $\bm{\theta^*}$ and $\bm{\hat{\theta}}$ to be model parameters learned on complete and minimized data. We also denote $\bm{g}_i(\btheta) = \nabla_{\btheta} \ell(f_{\btheta}(x_i), y_i) $. Lastly, we assume that  the baseline \textbf{Random Subsampling} performs randomly select with replacement a subset $S$ of from $D$. 


% We have the following theorem regarding the difference in expectation between $\bm{\theta^*}$ and $\bm{\hat{\theta}}$. 


% \begin{theorem}

% Suppose the loss function $\ell(.)$ is convex w.r.t $\bm{\theta}$, and suppose we perform \textbf{Random Subsampling} with replacement of fraction $0< p\leq 1$.  Furthermore, if  we denote $G = \max_{\bm{\theta}} \| \nabla_{\theta} \cL(\cX, \cY, \bm{\theta}) \|_2$  then the following holds:

% \begin{align}
% \mathbf{E}[\| \bm{\theta^*} -\bm{\hat{\theta}}\|^2] \leq (1-p) G
% \end{align}

% \end{theorem}
% \begin{proof}

% Our proof relies on the following Lemma  \ref{app:lem:1}

% \begin{lemma}[\citet{opt_paper}]
% \label{app:lem:1}
% Let $\cL(\cX, \cY, \btheta )$ be a differentiable function w.r.t  $\btheta$. 
% Then $\cL(\cX, \cY, \btheta)$ is $\lambda$-strongly convex w.r.t  $\btheta$    \emph{iff} for all vectors
%  $\btheta, \btheta'$: 
% \begin{equation}
%     (\nabla_{\btheta}\cL (\cX, \cY, \btheta ) - \nabla_{\btheta'} \cL(\cX, \cY, \btheta ) )^T (\btheta - \btheta') \geq \lambda \| \btheta -\btheta' \|^2.
% \end{equation}
% \end{lemma}

% Note that by the assumption the individual loss $\ell(f_{\btheta}(x), y)$ is convex hence the total  $\cL(\cX, \cY, \btheta) = \sum^n_{i=1}\ell(f_{\btheta}(x_i), y_i) + \lambda \| \btheta\|^2_2 $ is $\lambda$-strongly convex.


% \end{proof}

We have the following statement regarding the necessary condition when $\bm{\theta^*} = \hat{\btheta}$.
\begin{theorem}
\label{thm:subsampling}
Suppose the loss $\ell(.)$ is convex w.r.t $\btheta$ and furtheremore at the optimal point, the gradient of loss at any individual input vanishes, i.e $g_{i}(\btheta^*) = \nabla_{\btheta} \ell(f_{\btheta^*}(x_i), y_i)= \bm{0}^T$ $\forall x_i$. Then the model parameter $\hat{\btheta}$ learned with minimized data obtained  obtained by \textbf{Random Subsampling} (no matter with or with not replacement)  is exactly the same as $\btheta^*$  

\end{theorem}


\begin{proof}

Denote $S \subset \cD $ to be a random subset of $m << n$ training samples. By the assumption that the individual loss $\ell(.)$ is convex w.r.t $\btheta$ $\forall x_i$ then the following loss  function  is also convex:

$$ \hat{\cL}(\btheta) = \sum_{ (x_i,y_i) \in S} \ell(f_{\btheta}(x_i), y_i) $$.

Hence there is one single global minima that minimizes the loss $\hat{\cL}$ of the minimized data. Furthermore, by the assumption that $\nabla_{\btheta} \ell(f_{\btheta^*}(x_i), y_i)= \bm{0}^T$ $\forall x_i$, hence:

$$ \nabla_{\btheta^*} \hat{\cL}(\btheta) = \bm{0}^T$$

Hence $\btheta^*$ is also  the global minima of $\hat{\cL}$ which implies $\btheta^* = \hat{\btheta}$
\end{proof}
We provide the following example in which the assumption in Theorem \ref{thm:subsampling} holds.
\begin{example}
\label{ex:1}
Consider the linear regression task with the MSE loss $\ell(f_{\btheta}(x_i), y_i) = (\btheta^T x_i -y_i)^2$. Suppose there exists a parameter $\btheta^*$ such that  $y_i = \btheta^{*^{T}} x_i $, i.e, the groundtruth is a linear combination of input features.  Then using the \textbf{Random Subsampling} method we are guaranteed to retain the model parameter $\btheta^{*}$ learned on complete data.
\end{example}
We can see clearly that the example  \ref{ex:1} satisfies the conditions in Theorem \ref{thm:subsampling}. First of all, the MSE loss for linear regression is convex. Second the individual gradient  $\nabla_{\btheta} \ell(f_{\btheta^*}(x_i),y_i) = (y_i - \btheta^{*^T} x_i) x_i = \bm{0}^T$ by the assumption the groundtruth is a linear combination of input features. 


Furthermore we have the following statement regarding the  upper bound over the expected  $\mathbf{E}[ \| \btheta^* - \hat{\btheta}\|]$

\begin{theorem}
\label{thm:sampling_bound}
Suppose the loss function $\ell(f_{\btheta}(x_i), y_i)$ is convex  w.r.t $\btheta, \forall x_i$. If we denote $\Sigma$ to be the empirical covariance matrix of the set of deterministic vector $\{ g_i(\btheta^*) \}^n_{i=1}$  then the following holds:

\begin{align}
\mathbf{E}[\| \btheta^* - \hat{\btheta}\| ] \leq \frac{2 \text{Trace}(\Sigma)}{\lambda |S|} 
\end{align}
\end{theorem}

\textcolor{Theorem \ref{thm:sampling_bound} derives the upper bound on the difference between model parameters learned on minimized and complete data. It suggest the more number of training samples you can draw in \textbf{Random Subsampling} the smaller the difference. }

Our proof relies on the following classical theorem in statistis \cite{moore2009introduction}
\begin{lemma}
\label{lem:variance}

Consider a set of deterministic vector $\{ g_1(\btheta), ..,g_n(\btheta)\}^n_{i=1}$ with sample covariance variance $\Sigma$. If $S = \{ i | i \overset{\mathrm{iid}}{\sim} [n] \}$ then 

$$ \text{Trace}\left[Var[\frac{1}{|S|}\sum_{i \in S} g_i(\btheta)] \right] = \frac{\text{Trace}(\Sigma)}{|S|}$$
\end{lemma}


The Lemma \ref{lem:variance} implies that the more number of draw samples (i.e $|S|$ large) the smaller the  variance of sample mean.  

\begin{proof}
By the assumption that the individual loss $\ell(f_{\btheta}(x_i), y_i)$ is convex w.r.t $\btheta$ for all $x_i$, then the following empirical risk on minimized data is $\lambda$-strongly  convex:

\begin{align}
\hat{L}(\btheta) = \sum_{i\in S} \ell(f_{\btheta}(x_i), y_i) + \lambda \| \btheta\|^2_2. 
\end{align}
By the propery of strongly convex function it follows that:

\begin{align}
  ( \nabla_{\btheta} \hat{L}(\hat{\btheta}) -  \nabla_{\btheta} \hat{L}(\btheta^*)  )^T (\hat{\btheta} -\btheta^*)  \geq \frac{\lambda}{2} \| \hat{\btheta} - \btheta^* \|^2_2
\label{eq:diff}
\end{align}

Since $\hat{\btheta} = \text{argmin}_{\btheta} \hat{L}(\btheta)$ hence $\nabla_{\btheta}\hat{L}(\hat{\btheta}) = \bm{0}^T $. Thus the L.H.S of Equation \ref{eq:diff} can be reduced to $-\nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  $ 

Taking the expectation on both sides we obtain:

\begin{equation} \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right]\geq \frac{\lambda}{2} \mathbf{E}\left[ \| \hat{\btheta} -\btheta^*\|^2_2 \right]
\label{eq:1}
\end{equation}


Apply the Cauchy-Schwarz inequality for expectation, i.e  for any two random variables $X$ and $Y$ then $| \mathbf{E}[X^TY] | \leq  \sqrt{\mathbf{E}[X^TX]  \mathbf{E}[Y^TY] } $ it follows that:


\begin{align} \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right]& \leq \left| \mathbf{E}\left[ -( \nabla_{\btheta} \hat{L}(\btheta^*))^T(\hat{\btheta} -\btheta^*)  \right] \right| \\
& \leq \sqrt{ \mathbf{E}[ \|  \nabla_{\btheta} \hat{L}(\btheta^*) \|^2_2] \mathbf{E}[ \| \hat{\btheta} -\btheta^*\|^2_2] } \\
& =  \sqrt{ \mathbf{E}[ \|  \nabla_{\btheta} \hat{L}(\btheta^*) \|^2_2] }  \sqrt{ \mathbf{E}[ \| \hat{\btheta} -\btheta^*\|^2_2}
\label{eq:2}
\end{align}

Combine Equation \ref{eq:1} and Equation \ref{eq:2} we obtain:
\begin{equation}
 \mathbf{E}\left[ \|   \nabla_{\btheta} \hat{L}(\btheta^*)\|^2_2 \right] \geq \frac{\lambda}{2} \mathbf{E}\left[ \| \hat{\btheta} -\btheta^* \|^2_2 \right] 
\label{eq:3}
\end{equation}
\newcommand{\indep}{\perp \!\!\! \perp}

By the following property  for any random variable $X$  if $X_i \indep X_j $ for $X_i, X_j$ are two arbitrary entries of $X$   then $\mathbf{E}[ ||X||^2_2 ] = (E[X])^T E[X] + \text{Trace}[Var[X]]$. Furthermore, 

$$ \mathbf{E}[  \nabla_{\btheta} \hat{L}(\btheta^*)] =\mathbf{E}[\sum_{i \in S} g_i(\btheta^*) ] = \sum_{i \in S} \mathbf{E}[ g_i(\btheta^*) ]  = \bm{0}^T$$

The last equation comes from the fact that $g_{i}(\btheta)$ is drawn from a set of $\{  g_i(\btheta^*) \}^n_{i=1}$ whose the mean is a zero vector. 

Thus:

\begin{align}  \mathbf{E}\left[ \|   \nabla_{\btheta} \hat{L}(\btheta^*)\|^2_2 \right] & = \bm{0}^T + \text{Trace}( Var[\nabla_{\btheta} \hat{L}(\btheta^*)]) = \frac{\text{Trace}(\Sigma)}{|S|}\\
& \geq \frac{\lambda}{2} \| \hat{\btheta} -\btheta^* \|^2_2
\end{align}







\end{proof}


==> archived_sections/sec_threat_models.tex <==
\section{Threat Models}
\label{sec:threat_models}

\subsection{Attacker Access}

Attacker access can be categorized along: access to the minimized data and access to additional public data. First, let us examine the different settings related to access to the minimized data. The \emph{black-box} scenario occurs when an attacker only has access to the final data released after the imputation process, i.e., $\cD'' = \{x_i'', y_i\}^n_{i=1}$. In this case, the attacker lacks any additional knowledge of the data minimization techniques applied. On the other hand, the \emph{white-box} scenario involves the attacker having access to the actual minimized dataset $\cD' = \{x_i' = x_i \cdot B_i, y_i\}^n_{i=1}$ immediately after the minimization process. In this setting, the attacker possesses additional insights into the employed data minimization strategies as they have knowledge of the exact feature subset that was minimized. By considering both black box and white box access, we can thoroughly assess the potential risks associated with the release of the minimized data.

Furthermore, attackers may exploit additional public data $D_{pub} =(\cX_{pub}, \cY_{pub})$ to extract valuable information about the overall data distribution. This supplementary data, which is distinct from the minimized dataset, can provide insights into statistical patterns and characteristics that may not be apparent from the released dataset alone. Leveraging additional public data can be advantageous in both the black box and white box settings, as it allows attackers to gain a more comprehensive understanding of the underlying data. We also consider the potential utilization of additional public data in our paper, to ensure that our evaluation of privacy risks and the efficacy of data minimization techniques remains robust and realistic.

\subsection{Attacker Objectives and Associated Risks}

We now present an introduction of various threat models that we employ to measure privacy leakage in our framework. We recognize the importance of considering a wide range of threat models that reflect real-world privacy risks.

\subsubsection{Re-identification Attacks}

An important aspect to consider regarding privacy leakage in the minimized dataset is the potential for re-identification of individuals, even when only partial (i.e., minimized) features are available. Re-identification attacks take advantage of publicly available information to match with the released dataset, revealing the identities of individuals. When attackers have access to diverse attributes of individuals through public information, they can effectively re-identify individuals and extract additional information about them from the released dataset. This poses a threat to the intended privacy safeguards implemented for the dataset.

In our setup, the minimized dataset $\cD'$ (or $\cD''$) is the target dataset for potential attacks. To estimate the upper bound of re-identification risk, we consider the original set of features $\cX = \{x_i\}^n_{i=1}$ as public information available to the attacker. This setup poses a risk where the adversary can determine the correct label $y_i$ for an individual, even when only the public set of features $x_i$ and the dataset with partial information $(\cX', \cY)$ (or $(\cX'', \cY)$) were originally released. Various other forms of auxiliary public information and associated re-identification risks can also be explored, but we do not discuss them in detail here.

Consequently, the attacker's objective is to find the best matching feature in the minimized dataset for each individual data point in the original set of features. More precisely, for a given individual in the auxiliary dataset $x_i$, the attackers ranks all data points in the released dataset $\cX'$ (or $\cX''$) based on their likelihood to be the minimized data point corresponding to the same individual $i$.

\subsubsection{Reconstruction Attacks}

Real-world datasets often exhibit inherent correlations among input features, allowing for the estimation of missing features based on the remaining data. Consequently, data minimization does not guarantee the inability to reconstruct the minimized information using the remaining data. Reconstruction attacks, which differ from re-identification attacks, focus on recovering missing information from a target dataset regardless of its significance in identifying individuals. These attacks typically use aggregate statistics in conjunction with the dataset itself and can recover missing information, rendering minimization ineffective.

More precisely, the objective of the attacker is to reconstruct the original set of features $\cX$ based on the minimized set of features $\cX'$ (or $\cX''$). The attacker may utilize additional public data $D_{pub}$ and external statistics related to the underlying data distribution to achieve this goal.
For the scope of this work, we treat the reconstruction of all features to be equally important. However, one can easily prioritize or ignore the reconstruction of certain features, if desired.

\subsubsection{Membership Inference Attacks}

Membership inference attacks pose a significant privacy threat as they seek to uncover whether an individual's data was included in the original dataset prior to the minimization process. While re-identification attacks focus on precisely identifying individuals with prior knowledge of their presence in the training dataset, membership inference attacks operate under the assumption of uncertainty. Attackers aim to determine whether their data belongs to the dataset or not, without necessarily aiming to identify specific individuals in the minimized dataset. This distinction highlights the importance of membership inference attacks and emphasizes their potential impact on privacy preservation efforts during data minimization.

While traditional membership inference attacks are typically aimed at extracting information from a learning model, our approach diverges by focusing on applying such attacks to data minimization algorithms, which presents unique characteristics. However, the underlying principles remain unchanged. The primary objective of the attacker is to exploit the information within the minimized dataset $\mathcal{X}'$ (or $\mathcal{X}''$) to determine whether a query data point $x_q$ was originally included in the complete dataset $\mathcal{X}$. By analyzing the properties and patterns present in the minimized dataset, the attacker can make inference about the membership status of a query data point, thus compromising the privacy safeguards of individuals whose data is being scrutinized.

% \paragraph{Data availablity}
% Access to the some  fully labeled public data  $D_{pub}$ is important aspect for the adversary in reconstruction/reidentification attacks. In particular, if the adversary has some knowledge on the underlying data distribution $P(X)$, he can use this knowledge to infer the missing entries $X_{U}$ given the revealed entries $X_R = x_R$ for one particular user $x$ by estimating $P(X_U |X_R =x_R)$.

% We measure the knowledge of the adversary by the size of the public data $ | D_{pub}|$. We assume that  the more number of public samples, the more accurate the underlying distribution $P(X)$ he/she can estimate, which suggests a more successful privacy attacks (MIA/reconstruction/reidentification).
% In addition to access to some public data, we also consider the following settings regarding adversary's knowledge on data minimization process.  

% \paragraph{Black-box attacks}

% Under this setting, the adversary can provide an arbitray input $x \in R^d$ and obtain the model prediction from $f_{\theta}(.)$ which is constructed from $(\bm{X'} = \bm{X} \cdot \bm{B}, Y)$. The adversary can not observe the minimized data $\bm{X}'$. 

% Based on the model's prediction $f_{\theta}(x)$  and some public fully labeled data $D_{pub} $ the adversary perform the attacks:
% \begin{itemize}
% \item MIA: Identify if  a given record $x$ to belong to the private training data $\cD = (\bm{X}, Y)$.
% \item Reconstruction attack:  Suppose the adversary partialy knows some attributes $x_P$ of one record $x \sim \cD$, he/she would like to infer the sensitive attributes $x_S$.


% \end{itemize}

% \paragraph{White-box attacks}

% Under this setting, we assume that the adversary can have access to minimized dataset $\bm{X}'$. Note that since accessing to  $\bm{X'}$, the adversary does not need to care on the model $f_{\theta}(.)$ that was trained in $(\bm{X'}, Y)$. The adversary still would like to perform two privacy attacks based on $\bm{X'}$, and some public data $X_{pub}$.

% \begin{itemize}
% \item  MIA: Identify if a given record appears on private data $\cD$

% \item Reconstruction attacks: Given $\bm{X}'$ that partially reveal some entries, and the public data $X_{pub}$ the adversary tries to reconstruct $\bm{X}$.

% \end{itemize}
% \paragraph{White-box$^+$ attacks}

% % \verb|\checkmark|: \checkmark \par
% % \verb|\cmark|: \cmark \par
% % \verb|\xmark|: \xmark

% \begin{table}[h!]
% \centering
% \begin{tabular}{| c c c c||} 
%  \hline
%   & Black-box & White-box & White-box$^+$\\ [0.5ex] 
%  \hline\hline
%  Public data & \checkmark & \checkmark  & \checkmark  \\ 
%  $f_{\theta}$ trained on $(\bm{X}', Y)$ & \checkmark  & \checkmark & \checkmark \\
% $\bm{X}'$ & \xmark & \checkmark & \checkmark \\
% Alg to generate $\bm{X'}$ from $\bm{X}$  & \xmark  & \xmark & \checkmark \\  
%  \hline
% \end{tabular}
% \caption{Summary of knowledge of adversary for each category of attacks.}
% \label{table:1}
% \end{table}

% \begin{table*}
% \begin{center}
% % \setlength\tabcolsep{2.8pt}
% \begin{tabular}{ccccc}
% \toprule[2pt]
% \multirow{2}{*}{\textbf{Attacker Objective}} & \multicolumn{3}{c}{\textbf{Attacker Access}} & \multirow{2}{*}{\textbf{Privacy Metric}} \\
%  & \textbf{$D'$} & \textbf{$D''$} & \textbf{$D_{pub}$} & \\
% \midrule

% \multirow{4}{*}{Re-identification Attack} & \xmark & \checkmark & \xmark & -- \\
%  & \xmark & \checkmark & \checkmark & -- \\
%  & \checkmark & \checkmark & \xmark & -- \\
%  & \checkmark & \checkmark & \checkmark & -- \\
% \midrule

% \multirow{4}{*}{Reconstruction Attack} & \xmark & \checkmark & \xmark & -- \\
%  & \xmark & \checkmark & \checkmark & -- \\
%  & \checkmark & \checkmark & \xmark & -- \\
%  & \checkmark & \checkmark & \checkmark & -- \\
% \midrule

%  \multirow{4}{*}{Membership Inference Attack} & \xmark & \checkmark & \xmark & -- \\
%  & \xmark & \checkmark & \checkmark & -- \\
%  & \checkmark & \checkmark & \xmark & -- \\
%  & \checkmark & \checkmark & \checkmark & -- \\

% \bottomrule[2pt]

% \end{tabular}
% \end{center}
% \caption{Threat Models and Privacy Metrics}\label{tab:threat_models}
% \end{table*}


==> sections/archived_to_shorten/sec_algorithms_archived.tex <==
Having defined a bilevel optimization problem, we next outline how to operationalize data minimization, starting with three strong baselines. These baselines, although not fully compliant with legal data minimization standards (either because they disregard its purpose or the data relevance principles), provide a measure of model quality degradation during the process, detailed in Appendix \ref{sec:app_baseline}. We then introduce three algorithm classes from bi-level optimization literature to address the data minimization challenge as formulated in \eqref{eq:dm_goal}.

Before diving into the discussion of the algorithms, we notice that, although the data minimization principle is designed to optimize the dataset size while retaining the quality of the resulting model (see Constraint \ref{eq:fidelity}), many algorithms work on a dual view that instead optimizes for model quality when trained on the minimized data under a given sparsity constraints $\|\bm{B}\|_1 \leq k$. Such algorithms can then search for a sparsity parameter $k$ that satisfies the desired $\alpha$-drop in performance, relating to the original constraints in \eqref{eq:dm_goal}.
% \iffalse 
% However, before we dive deeper, we note that most algorithms in the literature are designed for a different formulation than the one defined in \eqref{eq:dm_goal}. In particular, rather than optimizing for auxiliary constraints while maintaining model quality, existing algorithms in bi-level optimization instead optimize for model quality under given auxiliary constraints (in our case, the dataset size)~\citep{chen2022gradient}. Therefore, we rewrite the original optimization problem as:
% \begin{subequations}
% \label{eq:dm_dual_goal}
%     \begin{align}
%         \minimize_{\bm{B} \in \{\bot, 1\}^{n \times p}} \;\;
%             & J(\mhlgreen{\hat{\theta}}; \bX, \bY)
%             \label{eq:data_relevance_dual}\\
%         \textsl{s.t.}:\;\; 
%             & \mhlblue{\| \bm{B} \|_1} \leq k
%             \label{eq:fidelity_dual}
%             \\\;\;
%             & \mhlgreen{\hat{\theta} = 
%                 \argmin_\theta \frac{1}{n} \sum_{i=1}^n 
%                 \ell\left(f_\theta( \mhlblue{\bm{x}_i \odot \bm{B}_i}, y_i\right)}
%                 \label{eq:purpose_limitation_dual}
%     \end{align}
% \end{subequations}
% where $k$ is the size constraint over $\bm{B}$. We can still solve the original optimization in \eqref{eq:dm_goal}, i.e., find the smallest dataset size that maintains model quality above a threshold, by instead searching through the solutions of this optimization problem in \eqref{eq:dm_dual_goal} under changing size constraints. We will stick with this formulation for the rest of the paper, to measure and compare the utility and privacy of the minimized dataset across different size constraints.
% \fi 

\subsection{Baseline Algorithms}

\begin{figure}
% \begin{wrapfigure}[6]{r}{0.55\textwidth}
    \centering
    % \vspace{-12pt}
    % \includegraphics[width=0.51\linewidth]{images/dm_abstract.pdf}
% \end{wrapfigure}
% \begin{wrapfigure}[11]{r}{0.55\textwidth}
    % \centering
    % \hfill
    \includegraphics[width=1\linewidth]{images/baselines.pdf}
    \caption{\textbf{(Left)} Data minimization as a set of individualized binary decisions, visualizing the matrix $\bm{B}$. \textbf{(Right)} Three baselines algorithm for data minimization. While they violate the legal requirements, they can help us give context to our evaluations.}
    \label{fig:datamin}
% \end{wrapfigure}
\end{figure}

We define three baselines: feature selection, random subsampling, and individualized random subsampling, depicted pictorially in Figure \ref{fig:datamin}. \textit{Feature selection}~\citep{blum1997selection} is a breadth-based strategy that retains only the most important features in the data. We use the absolute correlation between each feature and the label to measure its importance. \textit{Random subsampling}, on the other hand, is a depth-based strategy that randomly selects a subset of data points, minimizing the dataset by excluding certain rows. Finally, \textit{individualized random subsampling} extends this to individualized minimization, by randomly selecting a subset of individual entries (feature, sample) to reduce the dataset size.

% \begin{equation}
%     \bm{B}_{ij} = \bot \, \text{if}\, (i,j) \in S,
% \end{equation}

% where $|S|$ is a parameter controlling the minimization sparsity.

% where $0 \leq k_p \leq 1$ is a value chosen so that $k$ elements of the original dataset $D$ are minimized, in expectation. 
%Here $U^P \in \{0, 1\}^{n \times p}$ is a randomly permuted binary matrix, with exactly $s$ indices filled with $1$, i.e., $\Sigma_{ij} U^P_{ij} = s$, to control the desired sparsity of the minimization matrix.

\subsection{Data Minimization Algorithms}
\label{sec:data_min_alg}
We briefly introduce the three algorithms adopted to solve the optimization posed in Problem~\ref{eq:dm_goal}. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\smallskip\noindent\textbf{Approximating the Lower Level Program \citep{6079692}.}
\label{sec:taylor_approximation}
Solving a bi-level optimization problem presents a significant computational challenge due to its nested structure. Nevertheless, this complexity can be substantially reduced if the lower-level problem admits a unique solution expressible in closed form. Operating under the premise that the minimized dataset $\bX' = \bX \odot \bm{B}$ closely resembles the original dataset $\bX$, we can approximate the target utility  \ref{eq:purpose_limitation} using a first-order Taylor expansion to derive a closed-form solution. This approach not only streamlines the problem but also renders it tractable.
%%

Recall that it is often convenient to view the optimization expressed in \eqref{eq:dm_goal} as a program that minimizes the loss $J(\hat{\theta}; \mathbf{X}, \mathbf{Y})$ under sparsity constraint over the minimization matrix $\bm{B}$. Under this view, the resulting optimization simplifies into integer linear programming, and its solution for a target sparsity $\|\bm{B}\|_1 \leq k$ is simply setting $\bm{B}_{ij} = 1$ for the $k$ entries with the largest importance scores, and $\bm{B}_{ij} = \bot$ otherwise. The importance scores are calculated using first- and second-order gradients w.r.t. the model's parameters and inputs. Additional details about the algorithm, the importance scores, the underlying assumptions, and the complete derivation are present in Appendix \ref{sec:app_algorithms}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\smallskip\noindent\textbf{Modeling the Target Utility \citep{wang2006review}.}
Instead of relying on the assumptions of low sparsity to approximate the target utility as above, we can take a more general approach by directly modelling and learning the mapping between the target utility and the minimized dataset. In other words, we want to learn a parametrized function $m_\omega(\bm{B}) \approx J(\hat{\theta}; \bX, \bY)$, where $\omega$ is a vector of parameters, to estimate the target utility without solving the lower-level optimization for $\hat{\theta}$.

By restricting $m_\omega(\bm{B})$ to be a linear function of $\bm{B}$, we can quantify the influence of each value in the dataset on the target utility as $\cI_{ij}$. Here $\cI_{ij}$ can only exist in one of two binary states, i.e., $\cI_{ij} = \mathbbm{1}_{[\bm{B}_{ij}=1]} \cdot \cI^1_{ij} + \mathbbm{1}_{[\bm{B}_{ij}=\bot]} \cdot \cI^{\bot}_{ij}$. To learn these values, we generate a large number of minimization matrix-final utility pairs. The final solution simplifies into integer linear programming as above but with the importance score matrix defined as $\cI^{\bot}_{ij} - \cI^1_{ij}$. More details on the algorithm, learning the mapping $m_\omega(\bm{B})$, generating the data, and the complete derivation are present in Appendix \ref{sec:app_algorithms}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\smallskip\noindent\textbf{Evolutionary Algorithms \citep{sinha2014finding}.}
So far, we have discussed methods that approximate the original optimization problem under various assumptions, enabling us to solve it more easily. An orthogonal class of algorithms, often applied to solve bi-level programs, are evolutionary algorithms. They trade the advantage of carrying no assumption with slow convergence, i.e., high computational demand, and higher risks of overfitting.
In our implementation of the evolutionary algorithm, we begin with a population of randomly generated minimization matrices $\bm{B}$ and then evolve them across multiple iterations to reach our objective. We mutate and breed the current population at each stage of the process to create a larger pool of choices and carry out the lower-level optimization for every member of this pool, only retaining the best performers for the next generation. The entire process is repeated until convergence, or for a fixed number of iterations. Additional details on the mutation and breeding methods are provided in Appendix \ref{sec:app_algorithms}.
%Evolutionary algorithms offer an advantage in that they are not constrained by any underlying assumptions and can even provide guarantees of convergence with enough iterations. However, to achieve convergence in a practical scenario, one needs to run several iterations with a large active population size. This can create a significant computational demand in comparison to other approximate methods we saw above.

==> sections/archived_to_shorten/sec_defenses_archived.tex <==
In the previous section, we saw that data minimization may not always guarantee privacy. In the following, we now present some simple yet effective adjustments to the minimization problem to align better with privacy and demonstrate the feasibility of a more comprehensive minimization objective, managing both utility and privacy.

\subsection{Feature-Level Privacy Scores}
To counteract the two distinct data breach risks, i.e., re-identification and reconstruction, we propose a simple augmentation to the minimization objective. Given the output of a minimization algorithm $\bm{B}^a = [\optimal{\bm{B}}]_{\bot \rightarrow 0}$, we define privacy scores $\bm{V}$, such that the score matrix $\bm{C}_{ij} = \bm{B}^a_{ij} + \beta\bm{V}_{ij}$ determines the indices that should be retained or removed. For simplicity, we will only define feature-level privacy scores, which are not personalized, i.e., $\bm{V}_{ij} = \bm{V}_{qj},\; \forall i, q \in [n], j \in [p]$.
Here, $\beta$ serves as a hyperparameter to tune the emphasis on privacy. Ultimately, we minimize values with the lowest $\bm{C}_{ij}$ scores to achieve the target sparsity. We now present the privacy scores for the re-identification and reconstruction attacks, respectively.

% For this paper, Note that we will only use simple feature-level privacy scores for our experiments, which are not personalized, i.e., $\bm{V}_{ij} = \bm{V}_{qj}\, \forall i, q, j$. 

\begin{itemize}[leftmargin=*, parsep=0pt, itemsep=0pt, topsep=2pt]
    \item \textbf{Privacy Scores to Reduce Re-identification.} In re-identification attacks, the risk arises from disclosing \emph{unique} features (e.g., phone number, SSN) rather than non-unique features (e.g., gender, race), as they make it easier to identify individuals. Following this rationale, we propose using the negative of the number of unique values for a feature as its privacy score. Minimizing distinctive features can increase the difficulty of re-identification.
    \item \textbf{Privacy Scores to Reduce Reconstruction.} In reconstruction attacks, the risk stems from features that exhibit a high correlation with other features, which can be exploited by adversaries to deduce missing values. Thus, to mitigate reconstruction risks, we propose using the negative of the average correlation of each feature with every other feature as a measure of its independence and thus its privacy score.
\end{itemize}

\noindent The privacy scores $\bm{V}$ are normalized within the range $[0, 1]$ before being combined with the minimization matrix.

% For example, considering a cancer patient database, if the outputs of data minimization process reveal some unique attributes like phone number, zip codes, then the adversary (e.g., insurance company) can identify well these patients from some public/axulirary data. 

% Different data minimization methods in Section \ref{sec:algorithms} focus only on utility of the learning models without any attention to the information leakage. In this subsection, we introduce a general defense framework against the inference attacks in data minimization problem. We assume that the data minimization process procedues a utility score matrix $\cU \in R^{n\times d}$, where each entry $\cU_{i,j}$ indicates the utility of feature $X_{ij}$. The higher  the value of $\cU_{i,j}$ is, the better the learning model $\hat{\btheta}$ will be if it is retained during minimization process. Our defense mechanism relies on constructing a privacy matrix score $\cP \in {n\times d}$, where $\cP_{i,j}$ represents for the amount of information leakage if  feature $\bm{x}_{ij}$ is revealed. $\cP$ is constructed differently for reconstruction and reidentification attack.

% In re-identification attack, the risks comes from publishing so-called \emph{unique} features of individuals. For example, considering a cancer patient database, if the outputs of data minimization process reveal some unique attributes like phone number, zip codes, then the adversary (e.g., insurance company) can identify well these patients from some public/axulirary data. In contrast, if the output of data minimization process releasing  less unique attributes like gender, races,... the adversay find it more difficult to identify such cancer patient since many individuals sharing the same gender, races. Based on this motivation, we propose the following  privacy scores $\cP$ against the reidentification attack:

% $$ \cP_{ij} = - | \text{Dom}(\bm{x}^j)|,$$
% where $\text{Dom}(a)$ denotes the domain of feature attribute $a$.

% \paragraph{Privacy scores for reconstruction attack}  In reconstruction attacks, the risks comes from releasing the features that have high correlation with other features. In fact, upon releasing these features, the adversary with knowledge from the underlying data distributon $P(\bm{x})$ can infer the missing features. To defend such attack, we propose the following privacy scores $\cP$:

% $$\cP_{i,j} =- \sum_{h\neq j} | \text{Corr}(\bm{x}_j, \bm{x}_h)|,$$

% where $\text{Corr}(a,b)$ compute the Pearson correlation between two vector $a$ and $b$.

\smallskip\noindent\textbf{Evaluating Privacy Score Modifications.}
%We will now evaluate the proposed modifications with privacy scores and their impact on the minimized datasets. 
For a given level of sparsity, it can be expected that incorporating privacy scores will decrease data breach risks, but potentially reduce accuracy. The critical issue is whether we can attain a more favourable trade-off between privacy and utility, regardless of the sparsity. We present the results in Figure \ref{fig:reid_recon_defense} for the handwritten digits dataset, varying the hyperparameter $\beta$. Results for other datasets are detailed in Appendix \ref{sec:app_defense}.

At $\beta=1.5$, integrating privacy scores enhances the privacy-utility trade-off, cutting the re-identification risk by over 50\% while maintaining the same accuracy. The impact on reconstruction risk is less dramatic, but improvements are evident. Increasing the focus on privacy to $\beta=3$ results in a less optimal trade-off, yet still better than at $\beta=0$. %The ideal privacy hyperparameter likely falls between these two points for this dataset. 
This notable effect of a basic feature-level privacy score underscores the necessity of directly addressing privacy in the minimization process, instead of relying on its incidental emergence.

% \begin{figure*}
%     \centering
%     \footnotesize
%     % \input{figure_scripts/fig_reidentification_defense}
%     % \input{figure_scripts/fig_reconstruction_defense}
%     \input{figure_scripts/fig_defenses}
%     % \input{figure_scripts/fig_algorithms_legend_defense}
%     \caption{\textbf{(Left)} Re-identification and reconstruction risks on the handwritten digits dataset, using feature-level privacy scores. The best trade-offs can be seen at $\beta=1.5$, highlighting the importance of considering privacy during minimization. \textbf{(Right)} Membership inference risks under DP-SGD in the lower-level problem, showing minor yet consistent improvements in the privacy-utility trade-off.}
% 	\label{fig:reid_recon_defense}
% \end{figure*}

% \subsection{Information Leakage Risks and DP-SGD}

% Finally, we analyze privacy-centric modifications in data minimization to counter membership inference. 
% An effective mitigation can be obtained by introducing a differentially private learning algorithm, DP-SGD~\citep{abadi2016deep}, into the lower-level program of the bi-level optimization in \eqref{eq:dm_goal}. We test its compatibility with data minimization by re-evaluating membership inference in this new setting. Note, we do not introduce DP-SGD into utility calculation, i.e., once the data is minimized, the rest of the pipeline outside the ``wall'' remains unchanged.

% \smallskip\noindent\textbf{Evaluating DP-SGD Modifications.} 
% By incorporating DP-SGD into the minimization optimization without altering other components, we want to assess the compatibility between these two methods. 
% The results, collected in Figure \ref{fig:reid_recon_defense}, clearly demonstrate a reduction in membership inference risks at the same accuracy threshold, with prominent improvements for methods that were more susceptible to information leakage, such as modelling target utility algorithm.
% DP-SGD is indeed compatible with minimization, reinforcing the benefits of considering privacy during minimization.

==> sections/archived_to_shorten/sec_eval_minimization_privacy_archived.tex <==
While various minimization algorithms can effectively reduce data with an emphasis on utility, as discussed in Section \ref{sec:legal_implication}, there is an expectation of privacy associated with data minimization that is currently unexplored in literature~\citep{rastegarpanah2021auditing,shanmugam2022learning,biega2020operationalizing,chen2023studying}. In this section, we provide a novel empirical evaluation of minimization algorithms on real-world privacy attacks.

\subsection{Inference Attacks}
\label{sec:attacks}

% We begin by defining the adversaries used in this paper to measure the privacy risks, as described in Section \ref{sec:threat_models}.

\noindent\textbf{Reconstruction Attack.} 
The attackers aim to recover missing information from the minimized dataset. To do so, we employ an imputation method $\cP$ that takes the minimized dataset $\bX'$ and some aggregate statistics $\cS$ as inputs, producing a reconstructed dataset $\bX^{\cP(\bX', \cS)}$. Our imputation method $\cP$ is simply the data imputation defined in Section \ref{sec:experiment_setup}.

\noindent\textbf{Re-identification Attack.} 
The attaker's objective is to identify an individual given only partial information. The attacker's goal is thus finding the best match in the minimized dataset $\bX' = \bX \odot \bm{B}$ for each data point in the auxiliary dataset (in our setup, simply the original dataset $\bX$). We use a modified Euclidean distance measure that skips missing values and scales the measured distance for the rest accordingly, to rank the best matches.

% \prakhar{Why auxiliary data? Give an example.}

% \noindent\textbf{Membership Inference Attack.} 
% The attacker aims to determine the presence or absence of an individual in the original training dataset.
% We use the SOTA membership inference attack RMIA~\citep{zarifzadehLowCostHighPowerMembership2023}, by training $8$ reference models on random $50\%$ subsets of the public data split. We operate under the practical assumption that the adversary is unaware of the data minimization applied prior to training the target model and evaluate the membership inference on the original dataset.

% We will consider two specific cases of membership inference attacks, \textit{(i)} attacker has no knowledge of the data minimization algorithm, \textit{(ii)} attacker has access to the minimization algorithm used before training the target model. We train shadow models as done in the literature for the first case, while we perform data minimization before training shadow models in the second case.

% \prakhar{Can we add another inference attack to address privacy leakage for the language setting? Or at least explain why the language setting is different.}

\subsection{Evaluating Privacy Leakage}
\label{sec:privacy_leackage}

We evaluate the inference risks across different minimization sparsities and measure the alignment of re-identification, reconstruction, and membership inference risks with dataset size, compiled in Figure~\ref{fig:reid_recon}. Our privacy risk evaluations are confined to only the numerical datasets. Moreover, for membership inference attacks, we exclusively focus on the handwritten digits dataset, as the only dataset where we train neural networks.
% given the ongoing debate on data privacy in language~\citep{brown2022does,mireshghallah2023can}, 

% Results are compiled in Figure~\ref{fig:reid_recon} for the re-identification and reconstruction, and Figure~\ref{fig:mia}(a) for membership inference.

% To evaluate the inference risks we reuse the experiment setup in Figure \ref{fig:dataset_size}, i.e., minimization across different sparsities, and measure the re-identification, reconstruction, and membership inference risks. For membership inference, we exclusively focus on the handwritten digits, as the only dataset where we train neural networks. Moreover, given the ongoing debate on data privacy in language~\citep{brown2022does,mireshghallah2023can}, our privacy evaluations are confined to only the numerical datasets. Results are compiled in Figure~\ref{fig:reid_recon} for the re-identification and reconstruction, and Figure~\ref{fig:mia}(a) for membership inference. 

\begin{figure*}[hbt!]
    \centering
    \footnotesize
    \input{figure_scripts/fig_reidentification_minimization}
    \input{figure_scripts/fig_reconstruction_minimization}
    \input{figure_scripts/fig_algorithms_legend}
    % \input{figure_scripts/fig_algorithms_legend}
    \caption{\textbf{(a, b, d, e)} Re-identification and reconstruction risks under changing sparsity. While the overall trends show improvement in privacy with data minimization, they are not aligned with the trends of dataset size.
    \textbf{(c, f)} Privacy risks under feature-level privacy scores. The lowest risk values can be seen at $\beta=1.5$, highlighting the importance of considering privacy during minimization.}
	\label{fig:reid_recon}
\end{figure*}

\noindent\textbf{Data Minimization and Re-identification Risk.}
We first focus on the re-identification risks for the handwritten digits dataset (Figure \ref{fig:reid_recon}(a)). Due to the dataset's large feature space, re-identification risk remains remarkably high even after extensive minimization. For example, the re-identification risk is close to $1$ for most algorithms even at $\approx 20\%$ dataset size. Thus, while minimization algorithms were able to reduce dataset size significantly under utility constraints (see Figure \ref{fig:dataset_size}), they cannot achieve the same improvements in re-identification risk, highlighting their misalignment. 
Strikingly, random subsampling emerges as an effective strategy to reduce dataset size while being aligned with re-identification risks, despite performing poorly in terms of utility. Random subsampling is aligned with re-identification risk, as completely removing a data point also removes any risk of its re-identification.
While the misalignment between dataset size and re-identification risk is less pronounced in the bank dataset (Figure \ref{fig:reid_recon}(b)), we still see regions where reducing dataset size doesn't result in an equivalent reduction in the re-identification risk and regions where only minor reduction in dataset size creates significant drops in re-identification risk.

Note also the behaviour of feature selection across different datasets. Despite its ability to maintain reasonable utility after minimization (see Figure \ref{fig:dataset_size}), feature selection is highly ineffective in mitigating re-identification risks for any dataset. This inadequacy can be attributed to the persistence of certain features in the minimized dataset that are capable of uniquely identifying individuals, even when other features are removed. Similar trends can be expected between re-identification risk and other breadth-based minimization techniques in the literature~\citep{rastegarpanah2021auditing,goldsteen2021data,staab2024principle}. These findings underscore the misalignment between the reliance on dataset size for minimization and the expectations of reduction in re-identification risks.

\noindent\textbf{Data Minimization and Reconstruction Risk.}
Next, we shift focus to the results of reconstruction risks, as shown in Figure~\ref{fig:reid_recon}(d,e). Notice that even at the smallest dataset size, the risks associated with reconstruction remain notably high for both datasets. Thus, it's possible to successfully reconstruct a substantial part of the dataset even after extreme minimization.
% even when a significant portion of the data is removed, 
% it by using aggregate data statistics.
Additionally, our results reveal that the handwritten digits dataset, despite showing a substantial misalignment with re-identification risks, is comparatively easier to protect against reconstruction. This is likely due to its higher feature variance relative to the bank dataset. Thus, not only is the dataset size not aligned with privacy risks, but even the various privacy risks are not aligned with each other, motivating further the explicit involvement of appropriate privacy constraints during minimization.

% Reconstruction risks show smoother trends than re-identification risks. However, the risk of reconstruction even in the smallest dataset size and its variation across datasets underscore that data reconstruction does not always align with minimization requirements in data protection regulations.

% \noindent\textbf{Data Minimization and Membership Inference Risk.}
% Finally, we assess the membership inference risk under various minimization algorithms in Figure \ref{fig:reid_recon}(c). As previously mentioned, information leakage through a trained model is not an expected benefit of data minimization, which mainly aims to address data breach scenarios. Nevertheless, we still observe that certain minimization algorithms are effective at reducing membership inference risks with decreasing dataset size, i.e., models trained on minimized datasets leak less information. Yet, these improvements are not perfectly aligned, carrying forward the same trends we saw in the two data breach scenarios above.

% \begin{figure*}
%     \centering
%     \input{figure_scripts/fig_nn_mia_minimization}
%     \caption{Membership inference risks under changing sparsity on the handwritten digits dataset. The minimization algorithms can reduce inference risks and are pushed to even better trade-offs by introducing DP-SGD in the lower-level objective.}
% 	\label{fig:mia}
% \end{figure*}

==> sections/archived_to_shorten/sec_eval_minimization_utility_archived.tex <==
We now present a detailed evaluation of data minimization techniques under utility considerations, studying minimization behaviour across various datasets, modalities, and sparsity. Through this evaluation, we aim to gain insights into the practical implications of data minimization, as well as a deeper understanding of its strengths and limitations.

\subsection{Data Minimization Algorithms}

Having defined a bilevel optimization problem, we now outline how to operationalize data minimization, with three strong baselines and three algorithm classes from bi-level optimization literature to address the data minimization challenge as formulated in \eqref{eq:dm_goal}.
Note that although the data minimization principle is designed to optimize the dataset size while retaining the quality of the model (see Constraint \ref{eq:fidelity}), these algorithms work on a dual view that instead optimizes for model quality when trained on the minimized data under a given sparsity constraints $\|\bm{B}\|_1 \leq k$. Such algorithms can then search for a sparsity parameter $k$ that satisfies the desired $\alpha$-drop in performance.
% , relating to the original constraints in \eqref{eq:dm_goal}.
% \iffalse 
% However, before we dive deeper, we note that most algorithms in the literature are designed for a different formulation than the one defined in \eqref{eq:dm_goal}. In particular, rather than optimizing for auxiliary constraints while maintaining model quality, existing algorithms in bi-level optimization instead optimize for model quality under given auxiliary constraints (in our case, the dataset size)~\citep{chen2022gradient}. Therefore, we rewrite the original optimization problem as:
% \begin{subequations}
% \label{eq:dm_dual_goal}
%     \begin{align}
%         \minimize_{\bm{B} \in \{\bot, 1\}^{n \times p}} \;\;
%             & J(\mhlgreen{\hat{\theta}}; \bX, \bY)
%             \label{eq:data_relevance_dual}\\
%         \textsl{s.t.}:\;\; 
%             & \mhlblue{\| \bm{B} \|_1} \leq k
%             \label{eq:fidelity_dual}
%             \\\;\;
%             & \mhlgreen{\hat{\theta} = 
%                 \argmin_\theta \frac{1}{n} \sum_{i=1}^n 
%                 \ell\left(f_\theta( \mhlblue{\bm{x}_i \odot \bm{B}_i}, y_i\right)}
%                 \label{eq:purpose_limitation_dual}
%     \end{align}
% \end{subequations}
% where $k$ is the size constraint over $\bm{B}$. We can still solve the original optimization in \eqref{eq:dm_goal}, i.e., find the smallest dataset size that maintains model quality above a threshold, by instead searching through the solutions of this optimization problem in \eqref{eq:dm_dual_goal} under changing size constraints. We will stick with this formulation for the rest of the paper, to measure and compare the utility and privacy of the minimized dataset across different size constraints.
% \fi 



\begin{figure}
% \begin{wrapfigure}[6]{r}{0.55\textwidth}
    \centering
    % \vspace{-12pt}
    % \includegraphics[width=0.51\linewidth]{images/dm_abstract.pdf}
% \end{wrapfigure}
% \begin{wrapfigure}[11]{r}{0.55\textwidth}
    % \centering
    % \hfill
    \includegraphics[width=1\linewidth]{images/baselines.pdf}
    \caption{\textbf{(Left)} Data minimization as a set of individualized binary decisions, visualizing the matrix $\bm{B}$. \textbf{(Right)} Three baselines algorithm for data minimization. While they violate the legal requirements, they can help us give context to our evaluations.}
    \label{fig:datamin}
% \end{wrapfigure}
\end{figure}

\smallskip\noindent\textbf{Baseline Techniques.}
We define three baselines: feature selection, random subsampling, and individualized random subsampling, depicted pictorially in Figure \ref{fig:datamin}. \textit{Feature selection}~\citep{blum1997selection} is a breadth-based strategy that minimizes unimportant features in the data. We use the correlation between each feature and the label to measure its importance. \textit{Random subsampling}, on the other hand, is a depth-based strategy that randomly selects a subset of data points, minimizing the dataset by excluding certain rows. Finally, \textit{individualized random subsampling} extends this to individualized minimization, by randomly selecting a subset of individual entries (feature, sample) to reduce the dataset size. These baselines, although not fully compliant with legal data minimization standards (either because they disregard its purpose or the data relevance principles), provide a measure of model quality degradation during the process, detailed in Appendix \ref{sec:app_baseline}.

% \begin{equation}
%     \bm{B}_{ij} = \bot \, \text{if}\, (i,j) \in S,
% \end{equation}

% where $|S|$ is a parameter controlling the minimization sparsity.

% where $0 \leq k_p \leq 1$ is a value chosen so that $k$ elements of the original dataset $D$ are minimized, in expectation. 
%Here $U^P \in \{0, 1\}^{n \times p}$ is a randomly permuted binary matrix, with exactly $s$ indices filled with $1$, i.e., $\Sigma_{ij} U^P_{ij} = s$, to control the desired sparsity of the minimization matrix.

\smallskip\noindent\textbf{Data Minimization Algorithms.}
We briefly introduce three classes of algorithms adopted to solve the optimization posed in Problem~\ref{eq:dm_goal}. This includes, \textit{(i)} approximating the lower level program \citep{6079692}, which focuses on finding an approximate closed form solution to the lower-level problem, thus simplifying the original optimization, \textit{(ii)} modeling the target utility \citep{wang2006review}, which instead attempts to model the lower-level mapping and estimate it online without solving the optimization, and \textit{(iii)} evolutionary algorithms \citep{sinha2014finding}, which trade the advantage of carrying no assumption with slow convergence and high computational demand. Additional details about these algorithms and a comparative analysis can be found in Appendix \ref{sec:app_algorithms}.



\subsection{Experiment Setup}
\label{sec:experiment_setup}

\smallskip\noindent\textbf{Datasets.} Our evaluation focuses on classification using a tabular dataset (marked with symbol $^\diamond$), and an image dataset (symbol \(^\heartsuit\)), and a language dataset (symbol \(^\clubsuit\)), to cover a diverse set of distributions and modalities. More specifically, we use \textbf{(i) the bank marketing dataset}~\citep{moro2014data},
% taken from a telemarketing campaign with financial information of individuals and a binary label to represent the success of the campaign on 11,162 customers, 
taken from a telemarketing campaign with financial information of 11,162 customers,
% \textbf{(ii) the ACSEmployment task}, from the folktables dataset~\citep{ding2021retiring}, 
% with census information about individuals and a binary label to represent an individual's employment status,
% with census information and employment status of individuals,
(\textbf{iii) the handwritten digits dataset}~\citep{xu1992methods}, containing a total of 1,797 handwritten digit images across 10 different classes (i.e., digits), 
% each an $8 \times 8$ single channel image with integer pixel values between $[0, 16]$, 
and \textbf{(iv) the 20 newsgroups dataset}~\citep{lang1995newsweeder}, a collection of news posts across 20 topics.
% , i.e. target labels during classification.
We also provide results on several additional datasets in Appendix \ref{sec:app_defense}.

Due to their large size, a random subset of 5,000 data points is taken from the 20 newsgroups dataset for our evaluations. As recommended by \citet{lang1995newsweeder}, we also strip newsgroup-related metadata from the 20 newsgroups dataset. Finally, to limit the size of each news post, we truncate them to the first 50 tokens.

\smallskip\noindent\textbf{Data Splits.} Datasets are randomly split into two equal groups, private and public data. The 20 newsgroups dataset is already split into these groups based on the dates of the posts. The public data is used as the test data, to calculate statistics for data imputation, and train reference models for membership inference (more details in Section \ref{sec:attacks}).

The private data is further split into two equal groups, i.e. members and non-members. The members' group is our training data $\bX$, i.e., also the data that will be minimized in our pipeline. The non-members' group is only used for evaluating membership inference attacks. As we will not perform membership inference for the text dataset, i.e., the 20 newsgroups dataset, we do not perform this split and use the complete private data for training and minimization.

% \smallskip\noindent\textbf{Minimization Algorithms' Hyperparameters. }
% For modelling the target utility $m_\omega(\bm{B})$, we generate $500$ minimization matrix-target utility pairs for every numerical dataset and similarly $100$ pairs for the 20 newsgroups dataset. During the evolutionary algorithm, we iterate for $100$ steps with an active population size of $5$ for numerical datasets, and $50$ steps with an active population size of $3$ for the 20 newsgroups dataset.

\smallskip\noindent\textbf{Learning Setup and Data Imputation.}
We use logistic regression for the tabular dataset, a multi-layer perceptron with a single hidden layer containing $10$ neurons for the handwritten digits dataset, and a multinomial naive bayes classifier on tf-idf scores for the 20 newsgroups dataset. Both numerical datasets are passed through a MinMaxScaler for feature normalization, while the 20 newsgroups dataset is tokenized with the BERT tokenizer~\citep{kenton2019bert}. 
% Details of the minimization algorithms' hyperparameters are deferred to Appendix \ref{}.

For the numerical datasets, we perform data imputation under a multivariate gaussian distribution assumption~\citep{hoff2007extending}. We first calculate the mean value of each feature column, as well as the overall covariance matrix, using the public data split. During imputation, we then calculate the conditional distribution for missing values, given the other revealed values, and impute it with the mean of this distribution. For the 20 newsgroups dataset, we simply use masked language modelling with BERT~\citep{kenton2019bert} to fill in the missing text during imputation.

\subsection{Efficacy of Data Minimization}

First, we assess the ability of data minimization algorithms to reduce the dataset size across several modalities. Figure \ref{fig:dataset_size} summarizes the results, comparing the amount of data that could be minimized (y-axis) given a maximum drop in accuracy (x-axis) when compared to the accuracy returned by the classifier trained over the original, not-minimized, dataset. 
The results indicate a strong trend: A substantial amount of data can often be removed without sacrificing utility, suggesting that much of the collected data is superfluous in the datasets analyzed. This trend holds across different settings but with varying levels of susceptibility to minimization.

\begin{figure}[tb!]
    \centering
    \footnotesize
    \input{figure_scripts/fig_dataset_size_minimization}
    \input{figure_scripts/fig_algorithms_legend}
    \caption{Percentage of dataset minimized under different performance degradation thresholds ($\alpha$) across various algorithms, datasets, and modalities. Detailed results with changing minimization sparsities can be found in Appendix \ref{sec:app_defense}.} 
    % Threshold checks, for example, the dotted lines for $\alpha=2\%$ and $\alpha=5\%$ drop in accuracy, can be used to determine the minimum dataset size that meets a certain performance constraint ($\alpha$) for the original optimization problem defined in \eqref{eq:dm_goal}.}
    \label{fig:dataset_size}
\end{figure}


Notably, the baseline methods for minimization tested are found effective in reducing substantial amounts of data, possibly because they leverage existing structural redundancies in the dataset. For instance, feature selection excels with the handwritten digit dataset, where outer boundary pixels are never covered by the digits, and thus can be easily removed with minimal impact on model performance. Similarly, both random and individualized subsampling methods provide good minimization under loose accuracy drop thresholds, only gradually degrading with stricter thresholds.

While baseline methods demonstrate success, the proposed optimization algorithms consistently outperform them across all datasets. Nevertheless, different algorithms outshine others in specific scenarios. Evolutionary algorithms, for instance, surpass others on the bank dataset, driving minimization to extreme sparsity even under strict accuracy drop thresholds. It highlights a strength of minimization at its core: reducing the dataset size to a mere $18.75\%$ (and $6.25\%$) subset of the original bank dataset still allows the model to maintain utility with only a $2\%$ (and $5\%$) drop in accuracy. Similarly, approximating the target utility excels on the handwritten digits dataset, possibly due to its compatibility with the values of redundant features in the dataset (empty pixels are represented with $0$, compatible with the zero-imputation assumption of the algorithm). The handwritten digits dataset is particularly susceptible to minimization, given the abundance of redundant pixels in each image. Finally, while the text dataset is least susceptible to minimization, modelling the target utility method still yields a non-negligible reduction in dataset size under various thresholds (over 40\% of the data can be removed under a small (2\%) drop in accuracy). An in-depth discussion of the strengths and weaknesses of these algorithms is provided in Appendix \ref{sec:app_algorithms}.
% \nando{when discussing the algorithms, let us remember that we have a table to summarize their performance in the Appendix.}

\begin{wrapfigure}[16]{r}{0.5\textwidth}
    \centering
    \vspace{-36pt}
    \footnotesize
    \input{figure_scripts/fig_multiplicity}
    \caption{Pairwise overlap between minimized datasets across five runs with changing randomness of the evolutionary algorithm on the bank dataset. Despite similar utility, the minimization has very little overlap between any two pairs of runs.}
    \label{fig:multiplicity}
\end{wrapfigure}

\subsection{Multiplicity in Data Minimization}
\label{sec:multiplicity}

% \begin{figure}[t!]
% \end{figure}
In the previous section, we saw the effectiveness of data minimization across various settings. Next, we delve into the issue of multiplicity. We execute the evolutionary algorithm on the bank dataset multiple times with varied randomness (five repetitions, with a 25\% minimization target), and record the percentage overlap of retained data between all run pairs as well the final utility in Figure~\ref{fig:multiplicity}. Despite maintaining similar utility and dataset size, we observe little overlap between these runs (the highest overlap of a mere $25.51\%$). Clearly, there are many distinct ways to achieve data minimization, all satisfying data relevance, i.e., no more data can be removed without hurting the utility. Thus, we can achieve the same minimization objective with a diverse range of algorithms, providing great flexibility. However, at the same time, these different minimized datasets may also carry varying privacy risks due to the information they contain about missing features (as discussed in Section \ref{sec:legal_implication}). This highlights a misalignment between privacy expectations and real-world risks, explored further in Section \ref{sec:min_privacy}.



% There are various distinct ways to minimize datasets. When different subsets of the data compete to provide the same information, minimization algorithms make an arbitrary choice, introducing multiplicity. As depicted in Figure \ref{fig:multiplicity}, the maximum overlap of retained data between any two runs is a mere 25.51\%, indicating a 74.49\% difference in their resulting minimized datasets. While this multiplicity doesn't severely affect the utility of the dataset, it will significantly impact real-world outcomes, for instance, decisions on whether an individual's data is minimized or not. Current research on multiplicity in ML~\citep{black2022model,ganesh2023impact} primarily centers on the implications and challenges of model multiplicity. Multiplicity at the dataset level, and more specifically due to data minimization, is poised to further amplify these trends. We defer the discussion of future work on addressing these concerns to Section \ref{sec:discussion}.



\subsection{Visualizing Minimized Datasets}
\label{sec:viz}

We will now visualize the minimized dataset and highlight some emergent characteristics. We start with the bank dataset, minimized to 75\% sparsity with the evolutionary algorithm, and visualized in Figure \ref{fig:visualize}(a). It is intriguing to note that individualization trends naturally emerge from optimization, i.e., no single feature is heavily favoured over others, as illustrated by their distribution in Figure \ref{fig:visualize}(b). This individualized behaviour is a significant characteristic of data minimization and will play a crucial role in our privacy risks assessment (see Section \ref{sec:privacy_leackage}).  %emphasizing our decision to create a framework capable of performing individualized minimization.

Next, we turn our attention to minimized images in the handwritten digits dataset. Figure \ref{fig:visualize}(c) illustrates the behaviour of the evolutionary algorithm at 50\% sparsity. In these images, the individualization trends are more interpretable. For instance, when minimizing an image of the digit `1' the central vertical line is preserved, while for '0' it's the outside curves that are retained.
% since it contains the essential elements of the digit. 
% Similarly, the curves of `0' are also retained in the minimized image. The imputed images are even more fascinating. 
Notice however that despite minimizing half of the pixels, a significant portion of the image can be reconstructed using statistics learned from the public data, providing a strong indication of privacy risks.

\begin{figure}[tb!]
    \centering
    \begin{subfigure}[b]{0.29\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/compressed_bank_evolutionary_25.pdf}
         \caption{Compressed View of the Bank Dataset at 75\% Sparsity}
         \label{subfig:compressed}

         \includegraphics[width=\textwidth,height=0.62\textwidth]{images/histogram_bank_evolutionary_25.pdf}
         \caption{Feature Distribution of the Bank Dataset at 75\% Sparsity}
         \label{subfig:histogram}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/digits_visualize.pdf}
         \caption{Examples of Minimized Images \\(Handwritten Digits at 50\% Sparsity)}
         \label{subfig:digitsviz}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=1.28\textwidth]{images/20news_visualize.pdf}
         \caption{Examples of Minimized Text \\(20 Newsgroups at 25\% Sparsity)}
         \label{subfig:20newsviz}
    \end{subfigure}
    
    \caption{Visualizing minimized datasets across modalities, highlighting emergent individualized minimization and misalignment with privacy. \textbf{(a)} A compressed visualization of the minimized dataset shows emergent individualization, with no features or complete data points favoured over others. \textbf{(b)} Distribution of features retained in the minimized dataset, further highlighting the individualized nature of minimization. \textbf{(c)} Imputed images after minimization show the risks of data reconstruction despite minimization, thus emphasizing the lack of alignment between minimization and privacy. \textbf{(d)} Trends of minimizing stop words before personal identifiers further prove our claim of the misalignment between the current definition of minimization and the expectation of privacy.}
    \label{fig:visualize}
\end{figure}

Similar trends are observed in minimized text from the 20 newsgroups dataset, under modelling target utility algorithm at 25\% sparsity, in Figure \ref{fig:visualize}(d). When minimizing text, the algorithm focuses on eliminating stop words and other connectors that do not significantly alter the text's meaning. Interestingly, the algorithm retains various names, some of which may be relevant to the task (e.g., hockey player names in the news post about hockey) and others that could potentially compromise individual privacy (e.g., names of individuals who responded to an email regarding astrocytoma treatment). These examples highlight that a minimized dataset does not equate to enhanced privacy. %Next, we delve deeper into this misalignment through a detailed set of evaluations and even explore some potential remedies.

==> sections/archived_to_shorten/sec_formalizing_data_minimization_archived.tex <==
This section presents a mathematical interpretation of data minimization. Successively, we discuss its privacy implications and define various threat models to quantify real-world privacy risks.

\subsection{Data Minimization as Optimization}

Consider a dataset $D$ consisting of $n$ datapoints $(\bm{x}_i, y_i)$, with $i \in [n]$, drawn i.i.d.~from an unknown distribution. Therein, $\bm{x}_i \in \cX$ is a $p$-dimensional feature vector and $y_i \in \cY$ is the output label. 
For example, consider a loan approval task, where features $\bm{x}_i$ may describe an individual's characteristics, including their age, income, race, job, military history, and medical history, and label $y_i$ describes whether the individual will be able to repay the requested loan. 
The goal is to learn a predictor $f_\theta : \cX \to \cY$, with real-valued parameters $\theta$ that minimizes the empirical risk function (i.e., ERM):
\begin{align}
\label{eq:erm}
\optimal{\theta} \,= \argmin_\theta\; J(\theta; \bX, \bY) \quad \quad
\textrm{where} \quad J(\theta; \bX, \bY) = 
\frac{1}{n} \sum_{i=1}^n \ell(f_\theta(\bm{x}_i), y_i).
\end{align}
Here $\ell: \cY \times \cY \to \RR_+$ is a non-negative \emph{loss function} that measures the model quality, and $\bX$ and $\bY$ are used to denote, respectively, the $(n\times p)$-dimensional matrix of all features and the $n$-dimensional vector of all labels in $D$. While we use ERM as our learning objective here, the formulation can easily be extended to more complex utility functions.

The goal of \emph{data minimization} can be modelled as minimizing the size of the dataset $D$ by removing entries from the feature vectors $\bm{x}_i$ (\hlblue{data relevance}) while also retaining similar performance as it would have on the complete dataset (\hlgreen{purpose}). This objective can be formalized in the following bi-level optimization: 
\begin{subequations}
\label{eq:dm_goal}
    \begin{align}
        \minimize_{\bm{B} \in \{\bot, 1\}^{n \times p}} \;\;
            & \mhlblue{\| \bm{B} \|_1}
            % \label{eq:data_relevance}\\
        \quad \quad
        \textsl{s.t.}:\;\; 
            % &
            J(\mhlgreen{\hat{\theta}}; \bX, \bY) 
            - J(\optimal{\theta}; \bX, \bY)  \leq \alpha
            \label{eq:fidelity_archived}\\
        % \textrm{where} \;\;
            & \mhlgreen{\hat{\theta} = 
                \argmin_\theta \frac{1}{n} \sum_{i=1}^n 
                \ell\left(f_\theta( \mhlblue{\bm{x}_i \odot \bm{B}_i}), y_i\right)}
                \label{eq:purpose_limitation_archived}
    \end{align}
\end{subequations}
where $\bm{B}$ is an $n \times p$ binary matrix, which we call the \emph{minimization matrix} (visualized in Figure~\ref{fig:datamin}), taking values in the set $\{\bot, 1\}$, and the $\ell_1$-norm of $\bm{B}$, i.e., $\| \bm{B} \|_1$, is simply the count of $1$ in the minimization matrix. Here, $\bot$ represents the concealment or removal of a value, i.e., $\forall v \in \R: v \times \bot = \bot$, and $\alpha \geq 0$ is a parameter which bounds the permitted drop in model quality due to data minimization. While we define the misalignment between the two models as the loss' difference on the original dataset (\eqref{eq:fidelity}), this can be generalized to other measures of quality drop. %, such as privacy, fairness, or robustness. 

%  To address this, we will formalize data minimization as binary decisions on data collection made for each value in the dataset, as illustrated in Figure~\ref{fig:dm_abstract}.

The minimized input feature set $\bX'$ is defined as the element-wise product of the original feature set $\bX$ and the minimization matrix $\bm{B}$, i.e., $\bX' = \bX \odot \bm{B}$. 
Note that, data minimization produces a data feature set in the space $\cX \cup \{\bot\}$. While some learning algorithms are capable of handling missing values ($\bot$) in the dataset, in most cases one would be required to fill these values with data imputation, such as using average statistics or more advanced techniques. A discussion of imputation methods is delegated to Section \ref{sec:experiment_setup}.

The optimization problem in \eqref{eq:dm_goal} defines an operational method to remove entries from the feature set $\bX$ in a \emph{individualized} manner,
% (\eqref{eq:data_relevance})
while adhering to pre-specified accuracy requirements on the original dataset (\eqref{eq:fidelity}), for the final model trained on the minimized dataset (\eqref{eq:purpose_limitation}). While this formulation captures the legal formulation of data minimization, it is however intractable to solve in practice. We delegate a discussion of tractable approximate algorithmic alternatives to Section \ref{sec:algorithms} and discuss the privacy implications of this data minimization process next. 

% \nando{Need to mention that we can generalize the utility metric.}

% \nando{We need now a discussion on each of the equations above and this part on the bottom needs to be reorganized. }

% The misalignment is defined such that even though our model is trained on the minimized dataset with missing values, it should perform well on the full dataset, i.e., the inference behaviour remains unchanged.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Privacy Leakage}
\label{sec:threat_models}
% \nando{Refer back to the figure.}

We now consider a range of threat models that reflect real-world privacy risks and allow us to evaluate the extent of information leakage under various objectives and degrees of access available to the adversary. 
To do so, we introduce three threat models (Figure \ref{fig:framework}), each designed to measure a specific inference attack. The first two threats focus on \emph{data breaches}, i.e., situations in which the adversary has access to the minimized dataset. In this setting, we want to quantify the amount of information in the original dataset that we can safeguard by performing data minimization. The third threat focuses on \emph{information leakage} through the trained model, without direct access to the training data.

\emph{Note that the expectation of data privacy from minimization in various data protection regulations is primarily focused on the events of a data breach} (attacks happening inside the ``wall'' in Figure \ref{fig:framework}). This is different from the conventional settings of data privacy studied in the machine learning literature~\citep{dwork2006differential,rigaki2023survey}. Nonetheless, we also examine how data minimization privacy promise may hold in the event of information leakage due to ML inference (outside the "wall" in Figure \ref{fig:framework}). We will now define these threat models in detail.


\subsubsection{Data Breaches}

Within the confines of the ``wall'' in Figure \ref{fig:framework}, we will study the fundamental threats of a data breach. Specifically, we will focus on two distinct adversarial objectives, (i)~reconstructing the minimized data to get back the original dataset, and (ii)~re-identifying individuals from partial information in the minimized dataset.

\noindent\textbf{Reconstruction Risk (RCR).}
Real-world datasets often exhibit underlying associations between various features. Thus, even when particular information is minimized from the dataset, it can still be reconstructed from the remaining data~\citep{garfinkel2019understanding}. Reconstruction attacks (sometimes studied under attribute inference or model inversion) thus aim to recover missing information from a target dataset, often using aggregate statistics about the overall dataset distribution.

Given the minimized dataset $\bX'$, the attacker's goal is to generate their optimal reconstruction $\bX^R$ of the original set of features $\bX$. The Reconstruction Risk (RCR) can be evaluated by measuring the similarity between the original features $\bm{x}_i \in \bX$ and the reconstructed features $\bm{x}_i^R \in \bX^R$, computed using a gaussian kernel with $\sigma=1$~\citep{srebro2007good} as:
\begin{align}
    \textrm{RCR} = \frac{1}{n} \sum\limits_{i=1}^{n} e^{-|| \bm{x}_i - \bm{x}_i^R ||_2}.
\end{align}
As required, the reconstruction risk metric can also be adjusted further to prioritize the reconstruction of certain features over others by introducing appropriate weights to the similarity measurement.
%Adjustments to this metric can also be considered to prioritize the reconstruction of specific features.

\noindent\textbf{Re-identification Risk (RIR).}
% One of the central concerns in a data breach is the re-identification of individuals even in the presence of only partial or anonymized features. Re-identification attacks rely on an auxiliary dataset(s) $\bX^A$ to obtain public information about an individual, which can be matched with the minimized dataset to identify them~\citep{henriksen2016re}.
% 
% The effectiveness of the re-identification attack can be evaluated through the \emph{mean reciprocal rank (MRR)} scores~\citep{radev2002evaluating}, which assesses the quality of the rankings provided by an attacker. Specifically, for each data point $\bm{x}_i^A \in \bX^A$, the adversary generates a ranking of all data points in the minimized dataset $\bX'$ based on their likelihood of being the same corresponding individual. The re-identification risk (RIR) can be quantified as the average MRR scores, where a score of $1$ is assigned to the correct match and a score of $0$ is assigned otherwise:
% \begin{align}
%     \textrm{RIR} = \frac{1}{n} \sum\limits_{i=1}^{n} \frac{1}{\textrm{index}(i, \textrm{rank}(\bm{x}_i^A, \bX'))}.
% \end{align}
% Therein, $\textrm{rank}(\bm{x}_i^A, \bX')$ represents the ranking of data points as predicted by the adversary, and $\textrm{index}(e, A)$ returns the (1-based) index of some element $e$ in the array $A$. For evaluations, we assume a one-to-one mapping between auxiliary and minimized datasets, i.e., the $i^{th}$ data point in both datasets corresponds to the same individual. 
Data breaches often lead to re-identification of individuals using partial or anonymized data matched with an auxiliary dataset $\bX^A$. The success of these re-identification attacks can be measured by the mean reciprocal rank (MRR) scores. For each data point $\bm{x}_i^A$ in $\bX^A$, the adversary ranks data points in the minimized dataset $\bX'$ based on the likelihood of matching identities. The Re-identification Risk (RIR) is calculated as the average MRR score, assigning a score of $1$ for a correct match and $0$ otherwise, defined by the formula:
\begin{align}
     \textrm{RIR} = \frac{1}{n} \sum\limits_{i=1}^{n} \frac{1}{\textrm{index}(i, \textrm{rank}(\bm{x}_i^A, \bX'))}.
\end{align}
In this, $\textrm{rank}(\bm{x}_i^A, \bX')$ is the adversary's predicted ranking, and $\textrm{index}(e, A)$ gives the index of element $e$ in array $A$. It assumes a one-to-one match between auxiliary and minimized datasets.


\subsubsection{Information Leakage}

Next, we will shift our focus to threat models outside the ``wall'', specifically addressing inference attacks on the trained model without direct access to the minimized dataset. 
% Here, the focus is only on the privacy leakage from the dataset, i.e., we will not be discussing any model extraction attacks.

% \nando{Intro paragraph that specifies that now we are outside the wall.}
\noindent\textbf{Membership Inference Risk (MIR).}
Membership inference attacks~\cite{shokri2017membership} aim to discern if an individual's data was in the dataset before minimization, focusing on an attacker accessing the model $\hat{\theta}$ trained on this minimized dataset. In these attacks, the adversary calculates a likelihood score $L(\bm{x}_q)$ for each query $\bm{x}_q$, representing its probability of being in the original dataset $\bX$ using the model $\hat{\theta}$. The score is given by $L(\bm{x}_q) = \Pr\left[\bm{x}_q \in \bX \, \vert \, \hat{\theta}\right]$. Using these scores for both original dataset $\bX$ and non-members $\bX_{nm}$, binary membership predictions can be made at any threshold $t$, denoted as $\mathbbm{1}_{L(\bm{x}_q) \geq t}$. The overall Membership Inference Risk (MIR) is assessed as the area under the curve (AUC) of true positive rates ($\overrightarrow{\mathrm{tpr}}$) and false positive rates ($\overrightarrow{\mathrm{fpr}}$) across various thresholds:
\begin{align}
    \textrm{MIR} = \textrm{AUC}(\overrightarrow{\mathrm{tpr}}, \overrightarrow{\mathrm{fpr}})
\end{align}

% \begin{mdframed}
%     Our work focuses on three main objectives: \emph{maintaining utility}, \emph{preserving privacy}, and \emph{ensuring computational efficiency}. We strive to strike a balance between dataset utility and safeguarding against potential privacy breaches, while recognizing the importance of computational efficiency in practical applications. We aim to develop a framework that can be easily adapted and deployed by data holders to perform minimization.
% \end{mdframed}





% \subsubsection{Data Imputation}
% Sometimes, prior to releasing the data, the data holder may find it necessary to impute missing values in the minimized dataset. This is particularly relevant when the dataset release is expected to be complete and devoid of any missing entries, as required to train many ML algorithms.

% Imputation involves filling in the missing values of the minimized features $x_i' \in \cX'$ with estimated or imputed values to get the features $x_i'' \in \cX''$. It should be noted that the imputed dataset will have less information compared to the minimized dataset, because it no longer contains information about the specific set of feature values that were minimized. In our paper, we employ a simple imputation method that assumes an underlying multivariate gaussian distribution between all features in the dataset and imputes missing values using statistical measures like mean and covariance. While this method is rudimentary, for the purposes of our study, this provides a suitable framework to demonstrate the effects of imputation on the minimized dataset.

% \subsubsection{Preserving Utility}
% In a supervised setting, in the context of data minimization, the preservation of utility can be quantified through the minimization of the empirical risk associated with training a model on the minimized dataset $\cD' = \{x_i \cdot \cB_i, y_i\}^n_{i=1}$. For a given loss function $\ell(\cdot)$, the objective is to find the optimal parameter values $\theta^*$ that minimize the empirical risk. This can be expressed as:

% $$ \theta^* = \text{argmin}_{\theta} \sum^n_{i=1}  \ell\bigg(f_{\theta}(x_i \cdot B_i), y_i\bigg) $$

% Here, $f_{\theta}$ denotes the model with parameters $\theta$. By minimizing this empirical risk, we aim to ensure that the minimized dataset retains its utility during training.




==> sections/sec_defenses.tex <==
In the previous section, we saw that data minimization may not always guarantee privacy. In the following, we now present some simple yet effective adjustments to the minimization problem to align better with privacy and demonstrate the feasibility of a more comprehensive minimization objective, managing both utility and privacy.

\subsection{Feature-Level Privacy Scores}
To counteract the two distinct data breach risks, i.e., re-identification and reconstruction, we propose a simple augmentation to the minimization objective. Given the output of a minimization algorithm $\bm{B}^a = [\optimal{\bm{B}}]_{\bot \rightarrow 0}$, we define privacy scores $\bm{V}$, such that the score matrix $\bm{C}_{ij} = \bm{B}^a_{ij} + \beta\bm{V}_{ij}$ determines the indices that should be retained or removed. For simplicity, we will only define feature-level privacy scores, which are not personalized, i.e., $\bm{V}_{ij} = \bm{V}_{qj},\; \forall i, q \in [n], j \in [p]$.
Here, $\beta$ serves as a hyperparameter to tune the emphasis on privacy. Ultimately, we minimize values with the lowest $\bm{C}_{ij}$ scores to achieve the target sparsity. We now present the privacy scores for the re-identification and reconstruction attacks, respectively.

% For this paper, Note that we will only use simple feature-level privacy scores for our experiments, which are not personalized, i.e., $\bm{V}_{ij} = \bm{V}_{qj}\, \forall i, q, j$. 

\begin{itemize}[leftmargin=*, parsep=0pt, itemsep=0pt, topsep=2pt]
    \item \textbf{Privacy Scores to Reduce Re-identification.} In re-identification attacks, the risk arises from disclosing \emph{unique} features (e.g., phone number, SSN) rather than non-unique features (e.g., gender, race), as they make it easier to identify individuals. Following this rationale, we propose using the negative of the number of unique values for a feature as its privacy score. Minimizing distinctive features can increase the difficulty of re-identification.
    \item \textbf{Privacy Scores to Reduce Reconstruction.} In reconstruction attacks, the risk stems from features that exhibit a high correlation with other features, which can be exploited by adversaries to deduce missing values. Thus, to mitigate reconstruction risks, we propose using the negative of the average correlation of each feature with every other feature as a measure of its independence and thus its privacy score.
\end{itemize}

\noindent The privacy scores $\bm{V}$ are normalized within the range $[0, 1]$ before being combined with the minimization matrix.

% For example, considering a cancer patient database, if the outputs of data minimization process reveal some unique attributes like phone number, zip codes, then the adversary (e.g., insurance company) can identify well these patients from some public/axulirary data. 

% Different data minimization methods in Section \ref{sec:algorithms} focus only on utility of the learning models without any attention to the information leakage. In this subsection, we introduce a general defense framework against the inference attacks in data minimization problem. We assume that the data minimization process procedues a utility score matrix $\cU \in R^{n\times d}$, where each entry $\cU_{i,j}$ indicates the utility of feature $X_{ij}$. The higher  the value of $\cU_{i,j}$ is, the better the learning model $\hat{\btheta}$ will be if it is retained during minimization process. Our defense mechanism relies on constructing a privacy matrix score $\cP \in {n\times d}$, where $\cP_{i,j}$ represents for the amount of information leakage if  feature $\bm{x}_{ij}$ is revealed. $\cP$ is constructed differently for reconstruction and reidentification attack.

% In re-identification attack, the risks comes from publishing so-called \emph{unique} features of individuals. For example, considering a cancer patient database, if the outputs of data minimization process reveal some unique attributes like phone number, zip codes, then the adversary (e.g., insurance company) can identify well these patients from some public/axulirary data. In contrast, if the output of data minimization process releasing  less unique attributes like gender, races,... the adversay find it more difficult to identify such cancer patient since many individuals sharing the same gender, races. Based on this motivation, we propose the following  privacy scores $\cP$ against the reidentification attack:

% $$ \cP_{ij} = - | \text{Dom}(\bm{x}^j)|,$$
% where $\text{Dom}(a)$ denotes the domain of feature attribute $a$.

% \paragraph{Privacy scores for reconstruction attack}  In reconstruction attacks, the risks comes from releasing the features that have high correlation with other features. In fact, upon releasing these features, the adversary with knowledge from the underlying data distributon $P(\bm{x})$ can infer the missing features. To defend such attack, we propose the following privacy scores $\cP$:

% $$\cP_{i,j} =- \sum_{h\neq j} | \text{Corr}(\bm{x}_j, \bm{x}_h)|,$$

% where $\text{Corr}(a,b)$ compute the Pearson correlation between two vector $a$ and $b$.

\smallskip\noindent\textbf{Evaluating Privacy Score Modifications.}
%We will now evaluate the proposed modifications with privacy scores and their impact on the minimized datasets. 
For a given level of sparsity, it can be expected that incorporating privacy scores will decrease data breach risks, but potentially reduce accuracy. The critical issue is whether we can attain a more favourable trade-off between privacy and utility, regardless of the sparsity. We present the results in Figure \ref{fig:reid_recon_defense} for the handwritten digits dataset, varying the hyperparameter $\beta$. Results for other datasets are detailed in Appendix \ref{sec:app_defense}.

At $\beta=1.5$, integrating privacy scores enhances the privacy-utility trade-off, cutting the re-identification risk by over 50\% while maintaining the same accuracy. The impact on reconstruction risk is less dramatic, but improvements are evident. Increasing the focus on privacy to $\beta=3$ results in a less optimal trade-off, yet still better than at $\beta=0$. %The ideal privacy hyperparameter likely falls between these two points for this dataset. 
This notable effect of a basic feature-level privacy score underscores the necessity of directly addressing privacy in the minimization process, instead of relying on its incidental emergence.

% \begin{figure*}
%     \centering
%     \footnotesize
%     % \input{figure_scripts/fig_reidentification_defense}
%     % \input{figure_scripts/fig_reconstruction_defense}
%     \input{figure_scripts/fig_defenses}
%     % \input{figure_scripts/fig_algorithms_legend_defense}
%     \caption{\textbf{(Left)} Re-identification and reconstruction risks on the handwritten digits dataset, using feature-level privacy scores. The best trade-offs can be seen at $\beta=1.5$, highlighting the importance of considering privacy during minimization. \textbf{(Right)} Membership inference risks under DP-SGD in the lower-level problem, showing minor yet consistent improvements in the privacy-utility trade-off.}
% 	\label{fig:reid_recon_defense}
% \end{figure*}

% \subsection{Information Leakage Risks and DP-SGD}

% Finally, we analyze privacy-centric modifications in data minimization to counter membership inference. 
% An effective mitigation can be obtained by introducing a differentially private learning algorithm, DP-SGD~\citep{abadi2016deep}, into the lower-level program of the bi-level optimization in \eqref{eq:dm_goal}. We test its compatibility with data minimization by re-evaluating membership inference in this new setting. Note, we do not introduce DP-SGD into utility calculation, i.e., once the data is minimized, the rest of the pipeline outside the ``wall'' remains unchanged.

% \smallskip\noindent\textbf{Evaluating DP-SGD Modifications.} 
% By incorporating DP-SGD into the minimization optimization without altering other components, we want to assess the compatibility between these two methods. 
% The results, collected in Figure \ref{fig:reid_recon_defense}, clearly demonstrate a reduction in membership inference risks at the same accuracy threshold, with prominent improvements for methods that were more susceptible to information leakage, such as modelling target utility algorithm.
% DP-SGD is indeed compatible with minimization, reinforcing the benefits of considering privacy during minimization.

==> sections/sec_introduction_archived.tex <==
As data-driven systems and machine learning (ML) applications continue to proliferate, they introduce new privacy risks~\citep{nasr2019comprehensive,thomas2022framework,wairimu2022modelling}, necessitating robust data protection. Among these risks stands the fundamental concern of data breach, which involves unauthorized access, disclosure, or acquisition of sensitive information, posing a threat to individuals' privacy. Several international data protection frameworks, including the European General Data Protection Regulation (GDPR), %~\footnote{\href{https://gdpr-info.eu/}{gdpr-info.eu/}} 
the California Privacy Rights Act (CPRA), %~\footnote{\href{https://cppa.ca.gov/}{cppa.ca.gov/}} 
and the Brazilian General Data Protection Law (LGPD), %~\footnote{\href{https://lgpd-brazil.info/}{lgpd-brazil.info/}} 
have consequently adopted the principle of \emph{data minimization} as a cornerstone to address these potential privacy risks~\citep{biegaRevivingPurposeLimitation2021}.

At its core, the data minimization principle requires organizations to \emph{collect, process, and retain only personal data that is adequate, relevant, and limited to what is necessary for specified objectives} (see Table \ref{tab:legal} for further details). It's grounded in the expectation that not all collected data is essential for the objective, in this case training an ML model~\citep{goldsteen2021data,paul2021deep,sorscher2022beyond,shanmugam2022learning}, and instead contributes to a heightened risk of information leakage. In essence, this principle aims to reduce the amount of data collected, processed, and retained, to minimize the potential for misuse, unauthorized access, or data breaches. 
Despite its legal significance and endorsement by various global data protection regulations, the data minimization principle lacks an appropriate mathematical representation, one that can be applied effectively to real-world ML applications. In particular, the current discourse on data minimization practices often overlooks two crucial aspects {\bf (1)} the individualized nature of minimization (e.g., information that is unimportant for an individual may be critical for another) and {\bf (2)} its intrinsic link to data privacy. 

To overcome these limitations, this paper introduces a formal framework that recasts the data minimization principle in ML as an optimization problem while being faithful to its legal and practical aspects. We further show how to leverage existing algorithms from optimization literature to solve this problem. % Our choice of algorithms reflects the principle's multifaceted nature, capturing both its focus on privacy and the need for data utility. 
The paper conducts an extensive evaluation of these algorithms and explores several key characteristics of minimized datasets, such as emergent individualized minimization during optimization and compatibility with real-world privacy metrics. We seek to answer a critical question: \emph{``Do current data minimization requirements in various regulations genuinely meet privacy expectations in legal frameworks?''} Our evaluations reveal that the answer is, unfortunately, no. While being an implicit intention \red{\st{in its legal interpretation}}, the requirements of data minimization are not aligned with data privacy and thus \red{\st{are not enough to} may not} provide the expected privacy protection. 

Finally, to address these shortcomings, we propose simple yet effective modifications to data minimization algorithms that enhance their privacy-preserving capabilities, leading to far better privacy-utility trade-offs under minimization. Through these comprehensive analyses, the paper hopes to demonstrate that incorporating data minimization with appropriate modifications into ML systems not only satisfies the legal requirements but can also reduce the privacy risks of potential data breaches while retaining high accuracy.
In summary, this paper makes the following contributions:
\begin{enumerate}[leftmargin=*, parsep=0pt, itemsep=0pt, topsep=2pt]
\item It examines various data protection regulations from around the world and provides the first formalization of data minimization as an optimization problem that \red{\st{is in line with the legal frameworks} faithfully incorporates the individualized nature of minimization}.
\item It implements three different classes of optimization algorithms for solving the data minimization problem in ML and introduces several threat models to empirically quantify privacy leakage within the context of data minimization.
\item Through extensive evaluations, it assesses the limitations and shortcomings of current regulatory requirements of data minimization in meeting the implicit privacy expectations.
\item Finally, it proposes simple yet effective modifications to the data minimization algorithms and demonstrates that attention to privacy during minimization can provide better trade-offs between user privacy and downstream utility.
\end{enumerate}

These contributions aim to bridge the gap between the regulatory and technical domains, offering a robust solution to the data minimization challenge faced by ML practitioners. The proposed framework provides a solid groundwork for future research and a practical guide for developing privacy-preserving ML systems in compliance with the legal requirements of data minimization.

% \noindent\textbf{Personalization in data minimization.} 
% Traditional methods for structured data preprocessing, such as feature selection~\citep{}, data sampling~\citep{}, and active learning~\citep{}, have been adapted to align with data minimization goals~\citep{}. Nevertheless, these adaptations rarely account for the inherently individualized nature of data minimization---what may be essential data for one individual could be redundant for another.

% \noindent\textbf{Data minimization and privacy.}
% While reducing the amount of collected personal data can mitigate privacy risks, data minimization's potential for privacy preservation extends beyond mere dataset reduction. Given its privacy expectations from various data protection regulations, it is important to understand the extent to which, data minimization aligns with real-world privacy risks. Unfortunately, current resarch predominantly focuses on reducing the raw dataset size as measure of minimization quality, disregarding its concrete effects on privacy.



==> sections/sec_neurips_checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract and introduction list our contribution to formalizing the mathematical definition of data minimization, implementing various algorithms to operationalize data minimization, and studying the alignment between the expectation and reality of data privacy through minimization. We cover all these points in our main paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: We discuss the assumptions made in our work in \S \ref{sec:formalization} and further discuss the limitations of our setting in \S \ref{sec:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not make any theoretical claims in the main paper. However, we do make theoretical claims in the appendix, along with complete proofs, in \S \ref{sec:app_baseline}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Details of the datasets used are provided in \S \ref{sec:experiment_setup}, while details of all the algorithms present in the paper are provided in \S \ref{sec:app_algorithms}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release our code with the submission, however, we do plan to make our code open source after the paper is published.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All experiment details required to reproduce the results are present in \S \ref{sec:experiment_setup} and \$ \ref{sec:app_algorithms}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We address variability in data minimization algorithms separately in \S \ref{sec:multiplicity}. However, not all experiments are reported with error bars across multiple runs.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not contain details of the exact computing setup used. However, the experiments were all performed using a single GPU, and can be easily replicated under limited resources.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work relies on publicly available datasets, and does not create any application with potential harms. Instead, we attempt to operationalize the data minimization principle, which can help improve data privacy for individuals.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our work can help improve the privacy of data collected in various ML pipelines, discussed at various points in the paper. We also discuss potential negative impact of our work in \S \ref{sec:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: There is no release of high risk data or models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All datasets used in the paper are publicly available datasets that can be used for research purposes. They are all properly cited throughout the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new assets are introduced in the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing experiments or research with human subjects is done in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing experiments or research with human subjects is done in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> tables/tab_multiplicity.tex <==
\begin{table}[hbtp!]
    \centering
    \scriptsize
    \begin{tabular}{cccccc}
        \toprule
         & Run 1 & Run 2 & Run 3 & Run 4 & Run 5 \\
         \midrule
         Run 1 & 1. & 0.504 & 0.499 & 0.499 & 0.501 \\
         Run 2 & 0.504 & 1. & 0.503 & 0.505 & 0.505 \\
         Run 3 & 0.499 & 0.503 & 1. & 0.502 & 0.503 \\
         Run 4 & 0.499 & 0.505 & 0.502 & 1. & 0.508 \\
         Run 5 & 0.501 & 0.505 & 0.503 & 0.508 & 1. \\
         \midrule
         Accuracy & 90.94\% & 91.33\% & 91.08\% & 91.01\% & 91.01\% \\
         \midrule
         Reid Risk & 0.65 & 0.68 & 0.65 & 0.70 & 0.71 \\
         \midrule
         Recon Risk & 0.51 & 0.51 & 0.51 & 0.51 & 0.51 \\
        \bottomrule
    \end{tabular}
    \caption{Caption.}
    \label{tab:multiplicity}
\end{table}
